Ordered Decompositional DAG Kernels Enhancements

In this paper, we show how the Ordered Decomposition DAGs (ODD) kernel framework, a framework that allows the definition of graph kernels from tree kernels, allows to easily define new state-of-the-art graph kernels. Here we consider a fast graph kernel based on the Subtree kernel (ST), and we propose various enhancements to increase its expressiveness. The proposed DAG kernel has the same worst-case complexity as the one based on ST, but an improved expressivity due to an augmented set of features. Moreover, we propose a novel weighting scheme for the features, which can be applied to other kernels of the ODD framework. These improvements allow the proposed kernels to improve on the classification performances of the ST-based kernel for several real-world datasets, reaching state-of-the-art performances.

==> Hash2.tex <==

\section{Two graph kernels based on the framework} \label{sec:frameworkinstances}

Various instances of the proposed framework can be obtained from the kernels described in Section~\ref{sec:kernelsfortrees}. 
However, a naive application of such kernels may lead, on most datasets, to graph kernels not competitive from the computational point of view. 
%  to demanding graph kernels from the computational point of view. 
This section, instead, focuses on obtaining fast graph kernels. Specifically, two instances of the framework are presented in the following: 
% having the main goal to obtain fast kernels. 
% For this reason, 
Section~\ref{sec:hash} focuses on the graph kernel based on the ST Kernel and show how to optimize its computation. 
Section~\ref{sec:noveltk} introduces a novel tree kernel, which is more expressive than ST. 

\subsection{A graph kernel based on the Subtree Kernel} \label{sec:hash}

In the previous section we discussed how the $BigDAG$, and consequently the $Big^2 DAG$, can improve the speed of the kernel matrix computation. 
If the tree kernel $K_T$ in eq.~\eqref{eq:bigdag} is the \textit{subtree kernel}, the $BigDAG$ yields an explicit (and compact) representation of the feature space of the kernel: by construction each node $u$ is associated to the unique proper subtree $T(u)$ rooted at $u$. Such subtree is uniquely associated to a feature and $f_u$ is the frequency of $T(u)$ in all the ODDs related to the input graph. 
By definition of the \textit{subtree kernel}, only matching identical subtrees contribute to the kernel, that is $ C(u_1,u_2) \neq 0 \Leftrightarrow T(u_1) = T(u_2)$. Exploiting this property leads to an efficient implementation. 
In fact, if $T(u_1) = T(u_2)$, we recall from Section~\ref{sec:kernelsfortrees} that $C(u_1, u_2)=\lambda^{|T(u_1)|}$ and eq.~(\ref{eq:big2dag}) can be computed with a single scan of the $Big^{2}DAG$ built from $G_i$ and $G_j$: 
\begin{equation}\label{eq:bigbigdagsubtree}
  \begin{array}{rl}
K_{Big^{2}DAG}(G_i,G_j)=&\displaystyle \!\!\!\!\!\!\!\!\!\!\!\sum_{u_1,u_2\in V(Big^{2}DAG)}\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\! F_{u_1}[i] * F_{u_2}[j] * C(u_1,u_2)\\ 
=& \displaystyle\!\!\!\!\!\!\sum_{u\in V(Big^{2}DAG)}\!\!\!\!\!\!\!\!\! F_{u}[i] * F_{u}[j] * \lambda^{|u|}. 
  \end{array}
\end{equation}
% 
% Since, as mentioned above, each $T(u)$ corresponds to a feature and the weight of the feature is determined by its frequency in the input graphs and the parameter of the kernel $\lambda$, then eq.~\eqref{eq:bigbigdagsubtree} becomes  
% \begin{equation}
%  \label{eq:hashimplementation}
%   \sum_{u\in V(Big^{2}DAG)}\!\!\!\!\!\!\!\!\! F_{u}[i]*F_{u}[j] C(u,u) = \sum_{u\in V(Big^{2}DAG)}\!\!\!\!\!\!\!\!\! F_{u}[i]*F_{u}[j]*\lambda * \delta(T(u))  
% \end{equation}
% 
% 
% Note that, scanning the $Big^{2}DAG$ built only on the graphs 
% 
As eq.~\ref{eq:bigbigdagsubtree} shows, the information needed to compute the kernel, for each feature $f$ and graph $G$, is: {\it i)} a representation of the proper subtree $f$; {\it ii)} the frequency of $f$ in $G$; {\it iii)} the value $\lambda^{|f|}$. 

We now discuss a more compact representation for proper subtrees than the $Big^2DAG$ which keeps all relevant information for computing the kernel.  
% Since, as we will show in the following, proper subtrees do not need to be represented explicitly, it turns out that the $Big^{2}DAG$ stores explicitly more information than necessary, for example the edges between nodes. 
% In order to look for a more compact representation and r
Recalling that the evaluation of a kernel function corresponds to a dot product in a feature space induced by the kernel, i.e. $K(G_i,G_j)=\langle \phi(G_i) ,\phi(G_j)\rangle$, we consider the explicit feature space representation $\phi(G)$ of a graph $G$, as induced by the kernel in eq.~\ref{eq:bigbigdagsubtree}: let us assume a mapping $\hash()$ from proper subtrees to indices of the vector $\phi(G_i)$ is available, if the value of the element of index $\hash(u)$ is $\phi_{\hash(u)}(G_i)=F_u[i]\lambda^\frac{|u|}{2}$ then 
\begin{equation}
 \sum_{u\in V(Big^{2}DAG)} \!\!\!\!\!\!\!\!\!F_{u}[i] * F_{u}[j] * \lambda^{|u|} = \!\!\!\!\!\!\sum_{u\in V(Big^{2}DAG)}\!\!\!\!\!\!\!\!\!\! \phi_{\hash(u)}(G_i) \phi_{\hash(u)}(G_j). % = \langle \phi(G_i) ,\phi(G_j)\rangle,  
  \label{eq:dagtofeaturespace}
\end{equation}
Since the last term in eq.~\eqref{eq:dagtofeaturespace} corresponds to evaluating only the non-zero elements of the feature space representation of $G_i$ and $G_j$, we can express eq.~\eqref{eq:dagtofeaturespace} as $\langle \phi(G_i) ,\phi(G_j)\rangle$ by setting $\phi_s(G)=0$ for all $s$ such that $\nexists u\in V(G). \hash(u)=s$. 
% 
% 
% Notice that the $Big^{2}DAG$ stores explicitly more information than necessary, for example the edges between the nodes. 

We propose a hash-based implementation of the $\phi(G)$ in eq.~\eqref{eq:dagtofeaturespace}. 
% 
% Not surprisingly, we can do that when the $Big^2DAG$ constitutes an explicit representation of the \textit{subtree kernel} feature space.
% In that case, each node $u$ of the $Big^2DAG$ represents a specific feature (tree) occurring at least once in the dataset, i.e. $u$ is the
% root of a (limited) tree visit of some vertex of a graph of the dataset. Associated to $u$ is the frequency vector $F_u[\cdot]$ reporting
% for each graph of the dataset how frequent the feature is, and
% the size of the tree rooted in $u$ to be used in conjunction with the $\lambda$ parameter.
% This information is sufficient to compute the kernel.
% Our proposal is to use an hash table to efficiently store such information. 
% The frequency values and the sizes are updated incrementally during the generation of the tree visits. Specifically, 
% Each vertex in $u\in Big^{2}DAG$ has associated a single feature appearing in $G_i$ or $G_j$, i.e. the proper subtree $T(u)$. 
The function $\hash(u)$ returning the unique id of the feature/subtree $T(u)$ is the one in \definizione{\ref{def:leq}}. Notice that, by using such $\hash()$ function to encode any DAG vertex $u$, the size of each id, and consequently the time to compute it, is bounded by $\rho(u)$ and it is independent from the number of descendants of $u$. 
If the vertices are processed in inverse topological order, each feature is guaranteed to get a unique id. 
Notice that, since the tree kernel is ST, the number of features corresponds to the number of nodes in the $BigDAG$. 
% 
% Each vertex $u\in Big^{2}DAG$, the key of the hash is a unique id associated to each tuple. Such id is the one returned by the function $\hash()$ in \definizione~\ref{def:leq}. Notice that, by using an hash function to encode any DAG vertex $\node$, the size of each id is bounded by a constant which, in practice, can be considered independent from the number of descendants of $\node$. 
% Each vertex $u$ is mapped, via the hash function, into a (sparse) vector $F_u[\cdot]$ with as many elements as the number of graphs having the proper subtree rooted at $u$ as feature; each element of the vector $F_u[i] = \lambda^{\frac{|u|}{2}} f_u$ represents the frequency of the corresponding feature in the graph $G_i$, say $f_u$, multiplied by $\lambda^{\frac{|u|}{2}}$. 
% \begin{equation}\label{eq:kerneltrick}
% 	\begin{array}{cccl}
% 	x_1,x_2 \in \mathbb{R}^D 				& \stackrel{\phi}{\longrightarrow} & \phi(x_1),\phi(x_2) \in \mathbb{R}^N &\,\,\,\,\,\,N \gg D\\
% 	\downarrow k	&															&	\downarrow \left\langle \cdot ,\cdot\right\rangle &\\
% 	      				k(x_1,x_2)												&    = & \left\langle \phi(x_1),\phi(x_2) \right\rangle &  
% 	\end{array}
% 	\end{equation}
%where $D_u=\lambda^{|u|}$ and $F_u[\cdot]$ is the 
%(sparse) vector of frequencies of the feature in each graph of the dataset. %and $ID_u$ is a unique id associated to each tuple. The id of a feature is created according to \definizione~\ref{def:leq}. 
%The frequency values and the sizes are updated incrementally during the generation of the tree visits. 
% 
% The mapping is created by using as access key for $u$ the string $L(u)\left(ID_{ch_1[u]},\ldots,ID_{ch_{outdeg(u)}[u]}\right)$. Of course, if $outdeg(u) = 0$, the key will only be constituted by the associated label $L(u)$, while if 
% \mbox{$outdeg(u) > 0$} the key will also include the ids of the children of $u$. 

We finally show that $\phi(G)$ can be computed directly from the input graph without constructing first the $Big^{2}DAG$. 
\begin{algorithm}[t]
\begin{algorithmic}[1]
    \scriptsize
    \STATE {\bfseries Input:} a graph $G$, $h$ (maximum depth of the visit)
    \FOR{{\bfseries each $\node\in V(G)$}}
	\STATE generate $DD_G^{\node,h}$ as described in Section~\ref{sec:odd} 
	\FOR{{\bfseries $u \in $ post-order-visit($DD_G^{\node,h}$)}}
	  \STATE $X_{u}[0]=\kappa(L(u))$
	  \STATE $S_{u}[0]=1$
    	  \IF{$X_u[0]$ is a new feature}
	    \STATE $\phi_{X_u[0]}=\lambda^{\frac{1}{2}}$
	  \ELSE
	    \STATE $\phi_{X_u[0]}=\phi_{X_u[0]} + \lambda^{\frac{1}{2}}$
	  \ENDIF
	  \IF{$u$ is not a leaf}
	    \FOR{{\bfseries $1\leq i\leq \max_{\node\in\subtreerootedat{u}}\depth(\node)-\depth(u)$}}
	      \STATE sort the children of $u$ 
	      \STATE {\bfseries compute-st-features} //see macro below 
	    \ENDFOR
	  \ENDIF
	\ENDFOR
    \ENDFOR
    \STATE {\bfseries Output:} $\phi$, the set of features of $G$
\end{algorithmic}
\begin{center}
\vspace{-0.2cm}
 *****
\vspace{-0.25cm}
\end{center}
\scriptsize
{\bfseries compute-st-features}
\begin{algorithmic}[1]
  \scriptsize
  \STATE $X_{u}[i]=\kappa\Big(L(u)\Big\lceil X_{ch_u[1]}[i-1] \#X_{ch_u[2]}[i-1]\ldots \#X_{ch_{u}[\rho(u)]}[i-1]\Big\rfloor\Big)$
  \STATE $S_u[i] = 1 + \displaystyle\sum_{j=1}^{\rho(u)}S_{ch_u[j]}[i-1]$
  \IF{$X_u[i]$ is a new feature}
    \STATE $\phi_{X_u[i]} = \lambda^{\frac{S_u[i]}{2}}$
  \ELSE
    \STATE $\phi_{X_u[i]} = \phi_{X_u[i]} + \lambda^{\frac{S_u[i]}{2}}$ %// add the subtree encoded by $X_u[i]$ as a feature.
  \ENDIF
\end{algorithmic}
\caption{An algorithm for computing the feature space representation of a graph $G$ according to the kernel $ST_h$. \label{alg:kernelsth}}
\end{algorithm}
The process is detailed in Alg.~\ref{alg:kernelsth}, in which the sparse representation of the feature space of a graph $G$, induced by the ST kernel with visits limited to depth $h$, is computed and represented via a hash map. 
Given a node of the graph, first the $DD_G^{\node,h}$ is constructed. %Note that $DD_G^{\node,h}$ has at most $h\rho$ nodes. 
The vector $X[]$ represents the encodings, according to \definizione{\ref{def:leq}}, of the subtrees resulting from the limited visits.  Specifically $X_u[d]$ is the encoding of the proper subtree rooted at $u$ and obtained from a breadth-first visit limited to $d$ levels. The vector $S[]$ represents the size of the subtrees encoded by the corresponding element of $X[]$. Finally, $\phi$ stores the weights of the extracted features. 
% Statistics concerning the feature size and frequency in each graph are incrementally and efficiently collected. 
% : when a feature of a graph $G_i$ is encountered, its id is looked up in the hash table, if it is not already present, then a new $F_u[\cdot]$ vector is inserted, otherwise the $F_u[i]$ element is updated accordingly. 
% 
% If all the visits up to depth $h$ must be generated, it is sufficient to perform only the visit at depth $h$ and for each vertex $u$ at level $k\leq h$ all the required $h-k+1$ features can be generated by using the features already generated for the children of $u$. 
% The process is detailed in Alg.~\ref{alg:kernelsth}. 
% The algorithm, for each node $\node$ of the graph, starts by building the {\it Decompositional DAG} starting from $\node$ whose depth of the visit is limited by $h$. 
% The vector $X[]$ represent the encoding of the subtrees of resulting from the limited visits. Specifically $X_u[d]$ represents the encoding, according to \definizione~\ref{def:leq}, of the subtree resulting from a breadth-first visit limited to $d$ steps. The vector $S[]$ represents the size subtrees encodded by the corresponding element of $X[]$. Finally, $\phi$ stores the weights of the extracted features. 
% Let $\subtreerootedat{\node}$ be the proper subtree of $T$ rooted at $\node$. 
The fact that in line $4$ the visit is post-order and that the variable $i$ in line $9$ of Alg.~\ref{alg:kernelsth} ranges from $1$ to $\max_{\node \in\subtreerootedat{u}}\depth(\node)-\depth(u)$, ensures that the $X_{ch_u[j]}[i-1]$ values of the children nodes of $u$ have been properly computed before being first accessed. 
Lines $5$-$11$ compute the encoding of the subtree composed by the single node $u$, obtained from the visit limited to $0$ levels, and add the corresponding element to $\phi$. If $u$ is not a leaf node, all subtrees obtained from limited visits up to $(\max_{\node \in\subtreerootedat{u}}\depth(\node)-\depth(u))\leq h$ levels, i.e. the visits termined at level $h$ or when a leaf node is encountered, are generated. The ordering of children nodes in line $14$ is the one of \definizione{\ref{def:leq}}. The macro \textbf{compute-st-features} in line $15$ executes the code in the bottom part of Alg.~\ref{alg:kernelsth}, which computes the encoding of the subtree resulting from the visit limited to $i$ levels and add the corresponding entry to $\phi$.  

Since the number of nodes of the DAG generated in line $3$ of Alg.~\ref{alg:kernelsth} is at most $H$, the complexity of the algorithm is $O(|V_G|H h\rho\log \rho)$. 
Evaluating the kernel between two graphs $G_1$ and $G_2$ then reduces to look for matching entries in the hash tables returned by Alg.~\ref{alg:kernelsth}. If we consider $H$ constant, the complexity of a kernel evaluation then is $|V_G|\log |V_G|$, where the term $\log |V_G|$ accounts for the worst case complexity for looking up a key in a hash table. 

% \begin{algorithm}[t]
% \begin{algorithmic}[1]
%     \scriptsize
%     \STATE {\bfseries Input:} a graph $G$, $h$ (maximum depth of the visit)
%     \FOR{{\bfseries each $\node\in V(G)$}}
% 	\STATE generate $DD_G^{\node,h}$ as described in Section~\ref{sec:odd} 
% 	\FOR{{\bfseries $u \in $ post-order-visit($DD_G^{\node,h}$)}}
% 	  \STATE $X_{u}[0]=\kappa(L(u))$
% 	  \STATE $S_{u}[0]=1$
%     	  \IF{$X_u[0]$ is a new feature}
% 	    \STATE $\phi_{X_u[0]}=\lambda^{\frac{1}{2}}$
% 	  \ELSE
% 	    \STATE $\phi_{X_u[0]}=\phi_{X_u[0]} + \lambda^{\frac{1}{2}}$
% 	  \ENDIF
% 	  \IF{$u$ is not a leaf}
% 	    \FOR{{\bfseries $1\leq i\leq \max_{\node\in\subtreerootedat{u}}\depth(\node)-\depth(u)$}}
% 	      \STATE sort the children of $u$ 
% 	      \STATE {\bfseries compute-st-features} //see macro below 
% 	    \ENDFOR
% 	  \ENDIF
% 	\ENDFOR
%     \ENDFOR
%     \STATE {\bfseries Output:} $\phi$, the set of features of $G$
% \end{algorithmic}
% \begin{center}
%  *****
% \end{center}
% \scriptsize
% {\bfseries compute-st-features}
% \begin{algorithmic}[1]
%   \scriptsize
%   \STATE $X_{u}[i]=\kappa\Big(L(u)\Big\lceil X_{ch_u[1]}[i-1] \#X_{ch_u[2]}[i-1]\ldots \#X_{ch_{u}[\rho(u)]}[i-1]\Big\rfloor\Big)$
%   \STATE $S_u[i] = 1 + \displaystyle\sum_{j=1}^{\rho(u)}S_{ch_u[j]}[i-1]$
%   \IF{$X_u[i]$ is a new feature}
%     \STATE $\phi_{X_u[i]} = \lambda^{\frac{S_u[i]}{2}}$
%   \ELSE
%     \STATE $\phi_{X_u[i]} = \phi_{X_u[i]} + \lambda^{\frac{S_u[i]}{2}}$ %// add the subtree encoded by $X_u[i]$ as a feature.
%   \ENDIF
% \end{algorithmic}
% \caption{An algorithm for computing the feature space representation of a graph $G$ according to the kernel $ST_h$. \label{alg:kernelsth}}
% \end{algorithm}

Alg.~\ref{alg:kernelsth} is applied to a single graph. However, an equivalent of the construction of the $Big^2DAG$ (Section~\ref{sec:bigbigdag}) can be obtained by a simple merge operation between the hash tables resulting from the application of Alg.~\ref{alg:kernelsth} to a set of graphs. 

% 
% [TOGLIERE IL PARAGRAFO SUCCESSIVO????????]
% As a final remark on the requirement for $\kappa(\cdot)$ to be a perfect hash function, it must be considered that in real-world datasets, the number of features is relatively small compared to the space of different (non perfect) hash codes, so the probability that two features are assigned to the same hash value is very small and depends on the complexity of the selected hash function. In addition to that, if an SVM/SVR is used, only the features occurring in the support graphs must be considered, further reducing the probability of a collision for the hash function. 
% 
% 
% \subsection{Encoding}
% 
% For our purposes, if we have to compute the kernel value between two graphs, we only need to know how many features the two graphs have in common and the size of the shared features, since this 
% information is used as the exponent of the $\lambda$ parameter in the kernel formula.
% So we do not need to keep an explicit representation of the structure corresponding to a given feature as long as we are able to code the feature in a unique way\footnote{Actually, features that are structurally different, but which cannot be discriminated by the used kernel can get identical code. For example a diamond shape graph and the tree obtained by a breadth-first visit of the same graph, as a whole, constitute equivalent features from the kernel point of view.}, e.g. by using a function that returns an identifier (e.g., a numerical value) given the structural representation of the feature in input. If we are able to define such function, then we can compare 
% the features present into two graphs by comparing their identifiers.  
% Let us elaborate on how such a function can be defined.
% Let consider an hash function $\kappa(\cdot)$ which given an alphanumeric string in input returns an integer value. Let for the moment assume that $\kappa(\cdot)$ is {\it perfect}, i.e. no repeating hash values 
% will arise from different alphanumeric strings in input. Then, given a vertex $\node$, we can assign 
% the following alphanumeric string $\sigma(\node)$ to it:
% \[\sigma(\node)=L(\node)\cdot \left(\prod_{i=1}^{outdeg(v)}\kappa(\sigma(ch_{i}[\node]))\right)\]
% where '$\cdot$' is the concatenation operator\footnote{Here we assume that the concatenation operator inserts between the two concatenated strings a special character non belonging to the alphabet used to generate the strings, so to 
% avoid to generate the same string starting from different input strings, e.g. concatenation of label "a1" with hash value "1" would otherwise lead to the same string obtained by concatenating
% label "a" with hash value "11". } and '$\prod$' represents the application of
% '$\cdot$' to an indexed sequence of arguments; moreover, the order adopted for the children $ch_{i}[\node]$ of $\node$
% is the same order induced by the hash function $\kappa(\cdot)$, i.e., $\node_1$ comes before $\node_2$ if $\kappa(\sigma(\node_1))<\kappa(\sigma(\node_2))$.
% Notice that the above function is well defined since if $\node$ is a leaf, then the alphanumeric string associated to it is given by $L(\node)$; moreover,
% strings associated to leaf nodes are sorted by the $\kappa(\cdot)$ function, which assigns different numerical values to different labels; in turn, such order 
% can be exploited to apply the $\sigma(\cdot)$ function to internal nodes that only have leaf nodes as children and recursively to other internal nodes.
% 
% It should be noticed that:
% \begin{itemize}
% \item $\sigma(\node)$ can efficiently be generated from $L(\node)$ and the strings generated for its children;
% \item  the size of each string is bounded by a constant which in practice can be considered independent from the number of descendants of $\node$;
% \item no explicit extended representation of the features is generated. 
% \end{itemize} 
% Thus, any feature can be identified by the value returned by $\kappa(\cdot)$ applied to the string obtained via $\sigma(\cdot)$, and stored into an
% hash table in association with additional information, such as feature size and how frequent that feature occurs into any of the training graphs.
% Actually, we can construct the whole feature space representation directly from the tree-visits of the graphs (one starting from each node) in the training set. In fact, if we insert in the table all the nodes
%  belonging to each tree, starting from the leaves up to the roots, we are sure that all the graph features are inserted into the table in an efficient and well defined way. Statistics
%  concerning feature size and frequency for each graph can be incrementally and efficiently collected as well. Specifically, for each different alphanumeric string $\sigma(\node)$ (where $\node$ is a node belonging to one of the
%  training graph $g_i$) 
%  the corresponding entry in  such  hash table is the following tuple:
%  
%  \begin{center}
%  (key=$\tau(\sigma(\node))$, $size_{visit}(\sigma(\node))$, $\#(\sigma(\node) ,g_1)$,\ldots, $\#(\sigma(\node),g_n)$)\\
%  \end{center}
%  
%  \noindent where, $size_{visit}(\sigma(\node))$ is equal to the number of nodes which have been visited to generate $\sigma(\node)$, and  $\#(\sigma(\node) ,g_i)$ is equal
%  to the number of times $\sigma(\node)$ has been generated when visiting nodes in the training graph $g_i$. It can be observed that $size_{visit}(\sigma(\node))=1+\sum_{i=1}^{outdeg(v)}size_{visit}(\sigma(ch_{i}[\node]))$,
%  and that the hash table will contain all the information concerning the training set: the representation of a graph $g_i$ in the feature space is obtained by projecting all the tuples on $\#(\sigma(\node) ,g_i)$. Moreover,
%  the kernel value between graphs $g_i$ and $g_j$ can be computed as 
%  \[K(g_i,g_j)=\sum_{f\in hash-table}  \lambda^{size_{visit}(f)}  \#(f,g_i)\#(f,g_j).\]
%  Finally, after training with an SVM, the optimal weight vector can be obtained by collapsing all the contributions of the support graphs for each feature $f$, 
%  i.e. 
%  \[w^*_f =  \lambda^{\frac{size_{visit}(f)}{2}} \sum_{i \in SG} y_i \alpha^*_i \#(f,g_i),\]
% \noindent where $SG$ is the set of support graphs, $y_i$ is the target value for $g_i$, and $\alpha^*_i$ is the optimal value for the dual variable associated to $g_i$.
% 
% Thus, after training, the model can be represented by an hash table with the following entries:
% 
% \begin{center}
%  (key=$\tau(f)$, $w^*_f$)\\
%  \end{center}
%  
%  \noindent which drastically reduces the storage occupancy.
%  Notice that, given a graph $\tilde{g}$ for which the score with respect to the model has to be computed, the contribution of each feature occurring in  $\tilde{g}$ can be 
%  computed by generating the corresponding alphanumeric string $f$ via $\sigma(\cdot)$, and then looking for $\tau(f)$ into the model hash table for 
%  checking if there is a match. In case of match, the corresponding $w^*_f$ is used to update the score\footnote{If $score$ is the partial value of the score computed till the matching feature $f$ is considered, the updated
%  value for the score becomes \mbox{$score\ \leftarrow\ score+ \lambda^{\frac{size_{visit}(f)}{2}}w^*_f$}. In order to avoid to recompute $size_{visit}(f)$ for features in $\tilde{g}$, it is more convenient to store into the model hash table the weight \mbox{$\hat{w}^*_f=\lambda^{\frac{size_{visit}(f)}{2}}w^*_f$} and update the current score according to \mbox{$score\ \leftarrow\ score+ \hat{w}^*_f$}.}. Thus the score computation can be performed in time and space which is linear with 
%  respect to the number of  nodes generated by the tree-visits of $\tilde{g}$.
%  
% The above approach leads to practical computational improvements with respect to an approach where the features are represented explicitly since the feature space is constructed directly from the graphs
% with no need to define an order between nodes being such order induced by the hash function $\kappa(\cdot)$.
% 
% If the \textit{subtree kernel} is used, the method we propose yields an explicit (and compact) feature space representation of the kernel; this fact leads to a very efficient implementation.
% As mentioned above, the $Big^{2}DAG$ is an explicit representation of the feature space of the \textit{subtree kernel} described in Section~\ref{sec:kernelsfortrees}. In fact, we can notice that the frequency associated to each node in $BigDag(G_i)$ is the frequency of the proper subtree rooted at that node in all the ODDs related to the graph $G_i$.
% If the \textit{subtree kernel} is used, there is a match only between identical subtrees, that is $ C(u_1,u_2) \neq 0 \iff T(u_1) = T(u_2) $, and eq.~(\ref{eq:big2dag}) can be rewritten as:
% \begin{equation}\label{eq:bigbigdagsubtree}
%  K_{Big^{2}DAG}(G_i,G_j)=\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\sum_{u\in V(Big^{2}DAG)}\!\!\!\!\!\!\!\!\!\!\!\!\!\! F_{u}[i]*F_{u}[j] C(u,u)
% \end{equation}
% 
% Exploiting eq.~\eqref{eq:bigbigdagsubtree} leads to a very efficient implementation. In fact, the whole kernel matrix can be computed with a single scan of the $Big^{2}DAG$ nodes. 
%h
%While new features are introduced when the \textit{subtree kernel} is employed and the visits are limited, all DAGs generated by visits of depth $j>h$ are lost (see Figure~\ref{fig:dd_with_h}).


==> bigdagconstruction.tex <==

\begin{figure}
\centering
\begin{tikzpicture}[auto,thick,scale=.5]
   \tikzstyle{graph}=[scale=1.0,minimum size=12pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
%		\node (s) [graph] {s} [->]  
%					child {
%            node (b) [graph] {b}
%        	};
%         \node (e) [graph] at (0:2){e}   
%         		child { node (d) [graph] {d}};		
%    ;    	
%    \draw
%    (s) to (e)
%    (b) to (d)
%    (b) to (e)
%    ;
  \small
   \tikzstyle{node}=[minimum size=12pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
        \node [node] {\textbf{s}} [->] %[->, ultra thick]
                child {
                    node [node] {\textbf{e}}[] 
                    child {node (d2)[node, xshift=0.35cm]{\textbf{d}}[]}
                }
                child {
                    node (b2) [node]{\textbf{b}}[]
                }
				;
         \draw [->]
         (b2) to (d2)
        ;
        \node (e) [node,xshift=2cm,yshift=0.0cm] {e}
        		child[->] {
            			node (s) [node] {s}
            			}
						child[->]{
									node (b) [node] {b}
									}
	   				child[->] {
            			node (d) [node] {d}
            			}
        ;
	 			\draw [red,->,line width=5pt] (6,-1.6)--(8,-1.6);
        \node [node,xshift=4.1cm,yshift=-1.0cm] {b}
        		child[->] {
            			node [node] {s}
            			}
						child[->]{
									node [node] {e}
									}
	   				child[->] {
            			node [node] {d}
            			}
        ;    
        \node [node,xshift=6.5cm, yshift=-0.2cm] {\textbf{d}} [->] 
                child {
                    node [node] {\textbf{b}}[] 
                    child {node (d2)[node, xshift=0.35cm]{\textbf{s}}[]}
                }
                child {
                    node (e2) [node]{\textbf{e}}[]
                }
				;
         \draw [->]
         (e2) to (d2)
        ;    
        %\node [black,yshift=-0.4cm,xshift=7.0cm] {b)};
\end{tikzpicture}
%\begin{tikzpicture}[scale=0.7]
%   	\tikzstyle{every node}=[scale=0.7,minimum size=18pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
%    \node (s) [xshift=1cm, yshift=0cm] {s}
%     child[->] {
%            node (b) {b}}
%	child[->]{
%	node (e) {e}
%		child[->] { node (d) {d}}
%        };
%        
%    \draw [->]
%    (b) to (d)
%    ;
%%    \node (e) {e}
%%        child[->] {
%%            node (s) {s}
%%            	}
%%	child[->]{
%%	node (b) {b}}
%%	   child[->] {
%%            node (d) {d}
%%            	}
%%        ;       
%%    \node (e) [xshift=0cm] {b}[->]
%%        child {
%%            node (s) {s}[]
%%            	}
%%	child[->]{
%%	node (b) {e}}
%%	   child[->] {
%%            node (d) {d}
%%            	}
%%        ;        
%%    \node (s) [xshift=0cm] {d}
%%     child[->] {
%%            node (b) {e}}
%%	child[->]{
%%	node (e) {b}
%%		child[->] { node (d) {s}}
%%        };
%%        
%%    \draw [->]
%%    (b) to (d)
%%    ;
%\end{tikzpicture}
\caption{Example of creation of an Annotated DAG from two ODDs. \label{fig:bigdag}}
\end{figure}


==> conclusions.tex <==

\section{Conclusions} \label{sec:conclusions}

We have proposed a framework for graph kernels based on the decomposition of a graph into a multiset of unordered DAGs. 
By extending the definition of convolution tree kernels to DAGs and by defining an ordering of the nodes of the DAGs, we favored the application of a vast class of tree kernels to graph data. 
A technique for speeding up the kernel computation for a large category of DAG kernels have been described and its effectiveness proved both from the theoretical and the practical point of view. 
Our analysis focused on two kernels of the framework, one of which is based on a novel tree kernel, and discussed specific optimizations. Their  classification performances on five benchmark datasets show that they are able to reach optimal or competitive results on practically all the datasets considered. 
Experimental results on efficiency show that, in practice, they are competitive, if not faster than state-of-the-art graph kernels. 
% Moreover, we experimentally showed that, considering both the accuracy and the average time needed to classify a test example, our kernels has better trade off between these two goals than the other state of the art kernels considered. 


==> dag_kernel.tex <==

\subsection{Tree-based kernels for ordered DAGs and graphs} 
\label{sec:treekernelsfordags}

Here we define a family of kernels for ordered DAGs based on tree-kernels. 
The basic idea is to project sub-DAGs to a tree space and then apply a tree kernel on the projections. 

Let a tree visit be a function $T(\node)$ that, given a node $\node$ of a $ODD^{\node_{i}}_{G}$, returns the tree resulting from the visit of the DAG starting from $\node$. 
Figure~\ref{fig:treevisit} gives an example of tree visits. The trees resulting from the visit starting in node \textbf{s} are identical for the DAGs in Figure~\ref{fig:treevisit}-a and Figure~\ref{fig:treevisit}-b even if the DAGs are not isomorphic. However, the DAGs in Figure~\ref{fig:treevisit}-a and Figure~\ref{fig:treevisit}-b can be discriminated if we consider the multiset of trees returned by the tree visits starting in all nodes of the DAGs: one tree is produced by the visit starting in node \textbf{d} of the DAG in Figure~\ref{fig:treevisit}-a and two trees are generated by the two visits starting in the nodes labelled with \textbf{d} in Figure~\ref{fig:treevisit}-b. 
Moreover, note that the set of tree visits would be different even if the nodes labelled with \textbf{d} were not leaves. 
The concept of tree visit is used in the following 
\begin{theorem} \label{teo:visits}
	Given the ordering $\dot{<}$ in \definizione{\ref{def:leq}}, $\neg(\node_i \dot{<} \node_j) \wedge \neg(\node_j \dot{<} \node_i)$ if and only if 
	 $T(\node_i)$ and $T(\node_j)$, obtained as visits of the sub-DAGs rooted at $\node_i$ and $\node_j$, are identical.
\end{theorem}
\begin{proof}
 If $\neg(\node_i \dot{<} \node_j) \wedge \neg(\node_j \dot{<} \node_i)$ then $\hash(\node_i)=\hash(\node_j)$. Recalling that $\kappa()$, the function on which $\hash()$ is based on, is a perfect hash function, we prove the thesis by induction. If $\node_i, \node_j$ are leaf nodes, then $\hash(\node_i)=\hash(\node_j)\Leftrightarrow L(\node_i)=L(\node_j)$. If $\node_i, \node_j$ are not leaf nodes, then $\forall l. 1\leq l\leq \rho(\node_i)$~ $T(ch_{\node_i}[l])$ is identical to $T(ch_{\node_j}[l])$ for inductive hypothesis, and then it must be $L(\node_i)=L(\node_j)$ since $\hash(\node_i)=\hash(\node_j)$; therefore $T(\node_i)$ is identical to $T(\node_j)$. 
  Now we show that if $T(\node_i)$ is identical to $T(\node_j)$, then $\hash(\node_i)=\hash(\node_j)$ by induction. The base case has already been proved by the equality $\hash(\node_i)=\hash(\node_j)\Leftrightarrow L(\node_i)=L(\node_j)$. By inductive hypothesis $\hash(ch_{\node_i}[m])=\hash(ch_{\node_j}[m])$ for each child $m$ of  $\node_i$ and $\node_j$. Then $\hash(\node_i)=\hash(\node_j)$ and $\neg(\node_i \dot{<} \node_j) \wedge \neg(\node_j \dot{<} \node_i)$. 
%  We prove the thesis by induction. If $\node_i, \node_j$ are leaf nodes, then $L(\node_i)=L(\node_j)$ for \Lemma~\ref{lemmaeq}. If $\node_i, \node_j$ are not leaf nodes, then $L(\node_i)=L(\node_j)$, $\rho(\node_i)=\rho(\node_j)$ for \Lemma~\ref{lemmaeq} and $\forall 1\leq l\leq \rho(\node_i)$ $ch_l[\node_i]$ is identical to $ch_l[\node_j]$ for inductive hypothesis; therefore $\node_i$ is identical to $\node_j$. 
\end{proof}
%  The basic idea is to use tree-visits to project subdags to a tree space and then apply tree kernels on the visits. 
%The basic idea is to consider, given a tree-kernel $K_T$, the feature space ${\cal F}_{K_T}$ induced by $K_T$ and then to project the DAG into ${\cal F}_{K_T}$ by means of the tree . More formally,
%given a DAG $D$ and $v\in V_D$, let $I_{\phi_i}(v)$ be $1$ if feature $\phi_i\in {\cal F}_{K_T}$ is seen rooted in $v$ and $0$ otherwise; here ``rooted in $v$''
%means that if we consider $tree(v)$, i.e. the tree generated by a visit of $D$ starting from $v$ and following the direction 
%of the edges, 
%the root of feature $\phi_i$ coincides with the root of $tree(v)$. Then, we can represent $D$ as  
%${\bf h}(D)\in \mathbb{N}^{|{\cal F}_{K_T}|}$, where  ${\bf h}_{\phi_i}(D)=\sum_{v\in V_D}I_{\phi_i}(v)$, and
% Finally define the DAG kernel $K_{K_T}(D_1,D_2)={\bf h}(D_1)\cdot {\bf h}(D_2)$.
\begin{figure}
\centering
\begin{tikzpicture}[auto,thick,scale=.5]
   \tikzstyle{node}=[minimum size=12pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
  \small
	 \draw [red,->,line width=5pt] (-14.8,-1.5)--(-12.6,-1.5);
 	 \draw [red,->,line width=5pt] (-14.8,-6.0)--(-12.6,-6.0);
    \node [node, xshift=-8.4cm] {\textbf{s}} [->] 
                child {
                    node [node] {\textbf{b}}[] 
                    child {node (d2)[node, xshift=0.35cm]{\textbf{d}}[]}
                }
                child {
                    node (b2) [node]{\textbf{e}}[]
                };
         \draw [->]
         (b2) to (d2);
 	 \node [yshift=-0.8cm, xshift=-9.3cm] {a)};
       \node [node, xshift=-8.4cm, yshift=-2.3cm] {\textbf{s}} [->] 
                child {
                    node [node] {\textbf{b}}[] 
                    child {node (d2)[node, xshift=0.0cm]{\textbf{d}}[]}
                }
                child {
                    node (b2) [node]{\textbf{e}}[]
                    child {node (d3)[node, xshift=0.0cm]{\textbf{d}}[]}
                };
        ;     
     	 \node [yshift=-3.1cm, xshift=-9.3cm] {b)};  
     	    \node [node, xshift=-5cm] {\textbf{s}} [->] 
                child {
                    node [node] {\textbf{b}}[] 
                    child {node (d2)[node, xshift=0.0cm]{\textbf{d}}[]}
                }
                child {
                    node (b2) [node]{\textbf{e}}[]
                    child {node (d3)[node, xshift=0.0cm]{\textbf{d}}[]}
                };
	  ;
           \node [node, xshift=-3.8cm] {\textbf{e}} [->]
           child {node (d2)[node, xshift=0.0cm]{\textbf{d}}[]};
           \node [node, xshift=-3.0cm] {\textbf{b}} [->]
           child {node (d2)[node, xshift=0.0cm]{\textbf{d}}[]};
           \node [node, xshift=-2.2cm] {\textbf{d}};          
     	    \node [node, xshift=-5cm, yshift=-2.3cm] {\textbf{s}} [->] 
                child {
                    node [node] {\textbf{b}}[] 
                    child {node (d2)[node, xshift=0.0cm]{\textbf{d}}[]}
                }
                child {
                    node (b2) [node]{\textbf{e}}[]
                    child {node (d3)[node, xshift=0.0cm]{\textbf{d}}[]}
                };
	  ;
           \node [node, xshift=-3.8cm, yshift=-2.3cm] {\textbf{e}} [->]
           child {node (d2)[node, xshift=0.0cm]{\textbf{d}}[]};
           \node [node, xshift=-3.0cm, yshift=-2.3cm] {\textbf{b}} [->]
           child {node (d2)[node, xshift=0.0cm]{\textbf{d}}[]};
           \node [node, xshift=-2.2cm, yshift=-2.3cm] {\textbf{d}};
           \node [node, xshift=-1.4cm, yshift=-2.3cm] {\textbf{d}};          
\end{tikzpicture}
\caption{Two DAGs (left) and their associated tree visits $T()$ starting from each node.\label{fig:treevisit}}
\end{figure}
 If we consider the tree kernels defined in Section~\ref{sec:kernelsfortrees}, then we can write
\begin{equation}
 \label{eq:dagkernel}
	KDAG_{K_T}(D_1,D_2)=\sum_{\substack{\node_1\in V_{D_1}\\\node_2\in V_{D_2}}}C(root(T(\node_1)),root(T(\node_2))), 
\end{equation}
where $root()$ is a function returning the root node of a tree, $T()$ are tree-visits 
% as defined in Section~\ref{sec:orderingdagvertices} 
and the  $C()$ function is the one related to the corresponding tree kernel $K_T$. A list of $C()$ functions can be found in Section~\ref{sec:kernelsfortrees}. 
Theorem~\ref{teo:visits} ensures that the mapping in feature space of each tree visit is well defined since the swapping of any two non comparable children of a node does not change the resulting tree visit. This, in turn, ensures that: 
\begin{itemize}
  \item $C(root(T(ch_{\node_1}[i])),root(T(ch_{\node_2}[j])))= C(ch_{root(T(\node_1))}[i],ch_{root(T(\node_2))}[j])$, for every $1\leq i\leq \rho(\node_1), 1\leq j\leq \rho(\node_2)$, which allows us to use the algorithms described in \cite{Collins2002, Moschitti2006a}, thus significantly reducing the computational burden;
  \item $C()$ remains a valid local kernel.
\end{itemize}
Given two isomorphic DAGs $DD_{G_1}^{\node_i}$ and $DD_{G_2}^{\node_j}$, by applying Theorem~\ref{teo:dagisomorfi} and Theorem~\ref{teo:visits} it can be concluded that $DD_{G_1}^{\node_i}$ and $DD_{G_2}^{\node_j}$ yield the same set of tree visits and thus have the same representation in feature space for each tree kernel. 
 Finally, the kernel of eq.~\eqref{eq:dagkernel} is positive semidefinite since it is an instance of convolution kernel framework \cite{Haussler1999}, where the relation $R$ is defined on $X_1 \times \ldots \times X_{|V|} \times ODD$, with $X_1 \times \ldots \times X_{|V|}$ being the set of tree-visits obtained from $ODD$. 
The feature space, i.e. the set of features associated with the kernels of eq.~\eqref{eq:dagkernel}, coincides with the one of the tree kernel $K_T$. 
However, note that a DAG with a ``diamond'' shape, such as the DAG in Figure~\ref{fig:treevisit}-a, has a different representation with respect to the DAG of Figure~\ref{fig:treevisit}-b: while the non-zero features are the same, the feature related to the leaf node \textbf{d} occurs once in Figure~\ref{fig:treevisit}-a, while it occurs twice in Figure~\ref{fig:treevisit}-b. 
After introducing the kernels used in this paper, we can now motivate why the ordering in Section~\ref{sec:orderingdagvertices} has been employed. %discuss how different orderings would not have allowed us to define a positive semidefinite kernel. 
We recall that the requirements for the ordering are to be efficiently computable and to  ensure that the swapping of non comparable nodes does not affect the feature space representation of the DAG. 
 More ``standard'' orderings would not meet both constraints. For example, a total order between DAG vertices would require an algorithm with GI-complete computational complexity \cite{JGT:JGT3190010410}. On the contrary, simple partial orderings, such as the one based on reachability of the nodes, would not allow us to consistently order structurally different sub-DAGs. This makes impossible to have a consistent mapping in feature space for any kernel whose features are tree structures, which basically includes the vast majority of tree kernels.

On the basis of eq.~\eqref{eq:dagkernel}, given a tree-kernel $K_T$, we can define a kernel $K_{K_T}$ between two graphs $G_1$ and $G_2$ as follows: 
\begin{equation} \label{eq:convolutiondagkernel}
K_{K_T}(G_1,G_2) = \sum_{\substack{D_1 \in ODD(G_1) \\D_2 \in ODD(G_2)}} KDAG_{K_T}(D_1,D_2)
\end{equation}
where $ODD(G)$ is the multiset $\{ODD_{G}^{\node_{i}} |  \node_{i} \in V_{G} \}$, $KDAG$ is defined according to eq.~\eqref{eq:dagkernel} and depends on a kernel for trees $K_T$. In the following, we refer to this class of kernels as $ODD$ kernels. 
As we noted in Section~\ref{sec:odd}, self-loops are ignored during the decomposition from graph to multiset of DAGs. However, information about self-loops can be incorporated into node labels. For example, let $*\notin \cal{A}$ be a symbol not appearing in any node label. Then, the label of any node with a self-loop can be concatenated with $*$ in order to distinguish it from a node with the same label but without self-loop. 
%It is trivial to recognize that the above kernel is PD.
%remembering to the reader that $ODD_{v_{i}}^{G}$ is the  Ordered Decompositional DAG that we obtain from the graph $G$ fixing the root at the vertex $v_{i}$ (with $v_{i} \in V_{G}$).  $ODDs(G)$ is a multiset, in which an element can appear more than one time.

\nuovo{Note that, given a DAG $ODD^{\node_{i}}_{G_1}$, the total number of nodes of all the tree visits, i.e. $\sum_{\node\in ODD^{\node_{i}}_{G_1}}|T(\node)|$, can be exponential with respect to $|V_{G_1}|$. However, such observation does not imply that the complexity of \eqref{eq:convolutiondagkernel} can be exponential since tree visits need not to be explicitly computed to evaluate the kernel function. 
Let us use a cache to store $C()$ values as described in \cite{Moschitti2006a}. The number of different tree visits obtained from $ODD^{\node_{i}}_{G_1}$ is at most $|V_{G_1}|$. Thus, when evaluating \eqref{eq:convolutiondagkernel} for two graphs $G_1$ and $G_2$, the number of values to be stored in the cache is at most $|V_{G_1}| |V_{G_2}|$. The number of times $C()$ is called is bounded by the total number of edges of $ODD(G_1)$ and $ODD(G_2)$. }{Rev 2 major issue 1}
Let $Q(n)$ denote the worst-case complexity of the tree kernel $K_T$, where $n=\max_{\substack{D_1 \in ODD(G_1) \\D_2 \in ODD(G_2)}} \{|V_{D_1}|,|V_{D_2}|\},$ then the kernel of eq.~\eqref{eq:convolutiondagkernel}
%\begin{flushleft}
%
%\end{flushleft}
 has time complexity $O(|V_{G_1}||V_{G_2}|\cdot Q(n))$. Thus, in the worst case where $n=\max \{ |V_{G_1}|,|V_{G_2}|\}$, using ST, SST, and PT as
tree-kernels, leads to a time complexity of  $O(n^3\log n)$, $O(n^4)$ and $O(\rho^3 n^4)$, respectively. 

% As we will see in Section~\ref{sec:relatedwork}, such complexities are not competitive with state of the art graph kernels, thus in 
In Sections~\ref{sec:bigdag}-\ref{sec:h} we show how the computation of $K_{K_T}(G_1,G_2)$ can be optimized. 


==> discussion.tex <==

\subsection{Feature spaces comparison of some graph kernels} \label{sec:discussion}

% The generally good results of the $ODD-ST_h$ kernel reported in Section~\ref{sec:exps} may be attributed to the fact that it has associated a large feature space, which improves its  adaptability to different datasets. 
A way to get insights on the difference between graph kernels is to analyze what types of inputs they are able to discriminate. 
While this is not a sufficient requirement for successfully solving a learning task, it becomes necessary, for example, in a classification problem when two graphs, with the same representation in feature space, have different target classes. 
Specifically %, which types of non isomorphic graphs have the same representation in feature space, i.e. 
we are going to present some cases in which $\phi(G_1)=\phi(G_2)$ when $G_1$ is not isomorphic to $G_2$. 
The analysis focuses on gBoost, the Fast Subtree and the proposed $ODD-ST_h$ and \nuovotk~kernels.  
Since gBoost extracts only a set of informative subgraphs, it is sufficient to consider $G_1=\{g\} \cup \{g_1\}$ and $G_2=\{g\} \cup \{g_2\}$, where $g$ is an informative subgraph and $g_1$, $g_2$ are not. Clearly $\phi(G_1)=\phi(G_2)=\phi(g)$. 

When considering the Fast Subtree Kernel, it can be observed that, in order for two graphs
to get the same representation in feature space, they need to have the same number of vertices and the same
statistics on the out-degree of vertices. In addition, $K_{ODD-ST_h}$ also requires the same distribution on the
length of all the pairwise shortest paths. This is not the case for the Fast Subtree Kernel. Figure~\ref{fig:graphbad4fs} shows an example of two graphs having the same feature space representation. Note that $K_{ODD-ST_h}$ is able to discriminate those two graphs: the left one has a shorter path of length $4$, while the longest one for the graph on the right has length $3$. This implies that there are at least two different tree visits and consequently two different features for both $ODD-ST_h$ and $ODD-$\nuovotk: the proper subtrees whose root correspond to the root of the tree visits.  

\begin{figure}[ht]\centering
  \centering
  \begin{tikzpicture}[scale=0.310]
    \tikzstyle{node}=[minimum size=15pt, inner sep=0pt, outer sep=0pt, circle, text=black, very thick]
    \node (s) [draw, node]{};
    \node (sr) [draw, node, xshift=4.0cm]{};
    \node (l1)[draw, node, xshift=-0.8cm, below=0.3cm of s]{};
    \node (r1)[draw, node, xshift=0.8cm, below=0.3cm of s]{};
    \node (l2)[draw, node, below=0.5cm of l1]{};
    \node (r2)[draw, node, below=0.5cm of r1]{};
    \node (l3)[draw, node, below=0.5cm of l2]{};
    \node (r3)[draw, node, below=0.5cm of r2]{};
    \node (srl1)[draw, node, xshift=-0.8cm, below=0.3cm of sr]{};
    \node (srr1)[draw, node, xshift=0.8cm, below=0.3cm of sr]{};
    \node (srl2)[draw, node, below=0.5cm of srl1]{};
    \node (srr2)[draw, node, below=0.5cm of srr1]{};
    \node (srl3)[draw, node, below=0.5cm of srl2]{};
    \node (srr3)[draw, node, below=0.5cm of srr2]{};
    \draw [-] (s) to (l1); \draw [-] (s) to (r1);
    \draw [-] (l1) to (l2); \draw [-] (r1) to (r2);
    \draw [-] (l2) to (l3); \draw [-] (r2) to (r3);
    \draw [-] (l1) to (r3); \draw [-] (r1) to (l3);
    \draw [-] (sr) to (srl1); \draw [-] (sr) to (srr1);
    \draw [-] (srl1) to (srl2); \draw [-] (srr1) to (srr2);
    \draw [-] (srl2) to (srl3); \draw [-] (srr2) to (srr3);
    \draw [bend right=65, -] (srl1) to (srl3); \draw [bend left=65, -] (srr1) to (srr3);
  \end{tikzpicture}
  \caption{An example of two different graphs having the same representation in feature space according to the Fast Subtree kernel. All the nodes have the same label.\label{fig:graphbad4fs}}
\end{figure}
% 
% \begin{figure}[ht]\centering
% 	\includegraphics[width=0.4\columnwidth]{figs/example_fst}
% 	\caption{An example of two different graphs having the same representation in feature space according to the Fast Subtree kernel. All the nodes have the same label.\label{fig:graphbad4fsold}}
% \end{figure}

% \begin{figure}[ht]\centering
% 	\includegraphics[width=0.8\columnwidth]{figs/example_odd}
% 	\caption{An example of two different graphs having the same representation in feature space according to the ODD kernels. All the nodes have the same label except the black one.\label{fig:graphbad4oddOLD}}
% \end{figure}

Let us turn our attention to the ODD-ST$_h$ and ODD-\nuovotk~kernels. Clearly, two graphs differing just in self-loops, yield identical multisets of DAGs. However, the information about the presence of self-loops could be transferred into the representation of the corresponding node, for example by adding a field to the representation of the label. A less trivial example of non-injective mapping for the ODD-ST kernel is shown in Figure~\ref{fig:graphbad4odd}. Since the set of DAGs generated from the graphs in the figure are identical, the feature spaces related to the ODD-\nuovotk~kernel are identical as well. 

\begin{figure}[ht]\centering
  \begin{tikzpicture}[scale=0.45]
    \tikzstyle{node}=[minimum size=13pt, inner sep=0pt, outer sep=0pt, circle, text=black, very thick]
    \node (s) [draw, node, xshift=5.3cm]{};
    \foreach \s in {1,...,11} {
      \node (a\s) [draw, node, yshift=-1.05cm, xshift={24 * \s}] {};
      \draw [-] (s) to (a\s); 
    }
    \foreach \n in {2,...,11} {
      \pgfmathsetmacro{\m}{\n - 1};
      \draw [-] (a\n) to (a\m);
    }
   \node (a6) [draw, node, ball color=black, yshift=-1.05cm, xshift={24 * 6}] {};
   \node (sb) [draw, node, below=1.7cm of s]{};
    \foreach \s in {1,...,11} {
      \node (as\s) [draw, node, yshift=-3.3cm, xshift={24 * \s}] {};
      \draw [-] (sb) to (as\s); 
    }
    \foreach \n in {2,...,11} {
      \pgfmathsetmacro{\m}{\n - 1};
      \draw [-] (as\n) to (as\m);
    }
    \node (a5) [draw, node, ball color=black, yshift=-3.3cm, xshift={24 * 5}] {};
  \end{tikzpicture}
  \caption{An example of two different graphs having the same representation in feature space according to the $ODD-ST_h$ and $ODD-$\nuovotk kernels. All the nodes have the same label.\label{fig:graphbad4odd}}
\end{figure}

% The two DAGs in Figure~\ref{fig:graphbad4sth} have identical representation in feature space. However, we haven't been able to find a pair of different graphs generating only one of those DAGs. 
% The only non-injective mapping for any of our proposed kernels, that we are able to find occurs when one of the two graphs have at least one self-loop. However, the information about the presence of self-loops could be transferred into the representation of the corresponding node, for example by adding a field to the representation of the label.
% \begin{figure}[ht]
% \centering
% \begin{tikzpicture}[auto,thick,scale=.5]
%    \tikzstyle{node}=[minimum size=12pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
%   \small
%     \node [node] {\textbf{s}} [->] 
%     child {
%      node [node, xshift=-0.3cm] {\textbf{s}} [->] %[->, ultra thick] -8.4cm
%                 child {
%                     node [node] {\textbf{b}}[] 
% 		    child {node [node, xshift=0cm]{\textbf{d}}[]}
%                     child {node (d2)[node, xshift=-0.01cm]{\textbf{d}}[]}
%                 }
%                 child {
%                     node (b2) [node]{\textbf{e}}[]
%                 }
%   }
%   child {
%        node [node, xshift=0.3cm] {\textbf{s}} [->] %[->, ultra thick] -5.4cm
%                 child {
%                     node [node] {\textbf{b}}[] 
%                     child {node (d3)[node, xshift=0.0cm]{\textbf{d}}[]}
%                 }
%                 child {
%                     node (b3) [node]{\textbf{e}}[]
%                     child {node (d4)[node, xshift=0.0cm]{\textbf{d}}[]}
%                 }
% }
% ;
%   \draw [->]
%          (b2) to (d2)
%         ;
%     \node [node, xshift=4cm] {\textbf{s}} [->] 
%   child {
%        node [node, xshift=-0.3cm] {\textbf{s}} [->] %[->, ultra thick] -5.4cm
%                 child {
%                     node [node] {\textbf{b}}[] 
% 		    child {node [node, xshift=-0.1cm]{\textbf{d}}[]}
%                     child {node (dd3)[node, xshift=-0.1cm]{\textbf{d}}[]}
%                 }
%                 child {
%                     node (bb3) [node]{\textbf{e}}[]
%                     child {node (dd4)[node, xshift=0.0cm]{\textbf{d}}[]}
%                 }
% }
%     child {
%      node [node, xshift=0.3cm] {\textbf{s}} [->] %[->, ultra thick] -8.4cm
%                 child {
%                     node [node] {\textbf{b}}[] 
%                     child {node (dd2)[node, xshift=0.35cm]{\textbf{d}}[]}
%                 }
%                 child {
%                     node (bb2) [node]{\textbf{e}}[]
%                 }
%   }
% ;
%   \draw [->]
%          (bb2) to (dd2)
%         ;
% \end{tikzpicture}
% 	\caption{Two different ordered DAGs having the same representation in feature space according to the $K_{ODD-ST_h}$ kernel.\label{fig:graphbad4sth}}
% \end{figure}

% Let us now turn our attention to the efficiency of the proposed $ODD-ST_h$ kernel.
% In Section~\ref{sec:bigdag} we have proposed a technique for speeding up the kernel computation by compactly representing the ODDs by means of an Annotated DAG (BigDAG). The complexity of the DAG kernels, for example the one of $K_{ODD-ST}$ and $K_{ODD-ST_{h}}$, depends on the number of nodes of the BigDAG. 
% In order to evaluate the actual complexities we have computed, for the $K_{ODD-ST_{h}}$ kernel, the number of nodes in each BigDAG on the NCI1 dataset. 
% The obtained figures are plotted in Figure~\ref{fig:dagnodes} as a function of the nodes of the graphs. We have also plotted the polynomial function interpolating these points. In order to have a comparison with the values of the bounds discussed in Section~\ref{sec:bigdag}, the functions $n^\frac{3}{2}$ and $n^2$ are plotted as well. 
% The number of nodes inserted in the BigDAG %for the dataset for $K_{ST_{h}}$ 
% are for the vast majority of points under the curve $n^{1.5}$. The size of the BigDAG tends to an asymptotic value with the number of nodes contained in the input graphs (see Section~\ref{sec:h}). In this case, the ``actual'' complexity of the kernel is proportional (via $H$) to $n\log n$. 
% Similar results are obtained for the other datasets. 
% Figure~\ref{fig:tempinci1} reports the time needed to compute the kernel matrix, as a function of $h$, for the $K_{ODD-ST_{h}}$ and the FS kernels on NCI1 and CAS. 
% %Computation times are divided into the components \textit{preprocessing} and \textit{kernel computation}. %The preprocessing phase includes all steps needed for the generation of the $Big^{2}DAG$. The kernel computation
% %includes the computation of the kernel matrices varying the $\lambda$ parameter. 
% Given that the available implementations of the two kernels are in different programming languages, the plots of the FS kernel were added just for a qualitative comparison. 
% Notice that, as $h$ increases, the time required for computing the kernel matrix seems to increase almost linearly. 
% This can be explained with the fact that smaller graphs do not allow too deep visits, so the
% increase in complexity due to the increase of the depth visit is compensated by the smaller number 
% of graphs where visits of that depth can be actually performed. 

% Let us now turn our attention the computational time required by the gBoost, the Fast Subtree and the $K_{ST_{h}}$ kernel. The following comparison is a qualitative one, since the algorithms are implemented in different languages and have been executed on different, although comparable, machines. Figure~\ref{tab:tempinci1} reports the time required for the computation of the kernel matrix for gBoost, the Fast Subtree and $K_{ST_{h}}$ for different values of the parameter $h$. 
% 
% \begin{figure*}[ht]
% 	\includegraphics[width=1.0\columnwidth]{figs/tempinci1.pdf}
% 	%\includegraphics[width=1.0\columnwidth]{figs/nodesNCIall_h6.pdf}
% 	\caption{Time in seconds required for the computation of the kernel matrix for NCI1 and CAS.\label{fig:confrontotempi}}
% \end{figure*}

%The complexity of the Shortest Path kernel is $O(n^4)$ and the complexity of the Fast Subtree kernel is $O(mh)$, where $m$ is the number of edges of the graph and $h$ is the maximum number of levels of a breadth-first visit of the graph (see \cite{Shervashidze2009a} for details). 

% Table~\ref{tab:timeresults} gives an idea of the time needed to compute the $K_{ST_{h}}$ kernel.
% All the times reported in tables, figures and in the following paragraphs refers to executions in a PC with two Quad-Core AMD Opteron(tm) 2378 Processors and 64GB of RAM.
% 
% Computation times are divided into the components \textit{preprocessing} and \textit{kernel computation}. The preprocessing phase includes all steps needed for the generation of the $Big^{2}DAG$. The kernel computation
% includes the computation of the kernel matrices varying the $\lambda$ parameter.
% 
% In order to compare our performance with the other methods with attention to fairness, we calculated the total (average) time needed to train a single round of k-fold cross validation with the optimal parameters (reported in table~\ref{tab:results}) for each method.
% Indeed, when applying cross validation, kernel methods has to compute the kernel matrix only once for each parameter configuration, and the only thing that needs to be repeated is the SVM algorithm. On the contrary, gBoost needs to repeat his whole execution for each different fold, because the model it generates is based on the frequency of subgraphs in the training set.
%  We performed this experiment on the biggest dataset we employed, namely CAS. $K_{ST_{h}}$ kernel took $561$ seconds to compute the kernel matrix and $2.4$ seconds for the SVM to converge. FS kernel took $113$ seconds for the computation of the kernel matrix, and $4.2$ seconds for the training of the SVM. GBoost took approximately $4000$ seconds.

% \begin{figure}[ht]
% 	\includegraphics[width=1.0\columnwidth]{figs/nodesNCIall-eps-converted-to.pdf}
% 	\caption{Number of nodes inserted into the BigDAG as a function of the nodes of the graphs. The plots refer to NCI1 with limitation to the depth of the visits ($h=6$).\label{fig:dagnodes}}
% \end{figure}
% 
% \begin{figure}[ht]
% 	\includegraphics[width=1.0\columnwidth]{figs/tempinci1.pdf}
% 	\caption{Time needed to compute the kernel matrix, as a function of $h$, for the $K_{ODD-ST_{h}}$ and the FS kernels on NCI1 and CAS datasets.\label{fig:tempinci1}}
% \end{figure}


==> experiments.tex <==

\section{Experimental results} \label{sec:exps}

While eq.~\eqref{eq:convolutiondagkernel} can be instantiated with any tree kernel, in order to reduce the time required for the experimentation, only the kernels in Section~\ref{sec:frameworkinstances}, the subtree kernel with visits of limited depth, i.e. $K_{ODD-ST_h}$, and the kernel $K_{ODD-\nuovotk}$,  are considered in the following. 
The reason for such choice lies in the fact that previous sections heavily focused on $K_{ODD-ST_h}$ and $K_{ODD-\nuovotk}$, especially from the computational point of view. 

% {\color{red}

%  Typically, learning algorithms depend on a set of parameters, that in the following we will refer with $\theta$. For the assessment of the predictive performance of an algorithm, we need a way to estimate the optimal values for such parameters.
 
% Then, using only the best parameters for each of the K folds, we classify the remaining examples (the test set for the particular iteration of K-fold).
% When assessing the quality of the results the word significant will be used referring to the  statistical test referred as 
% The $10 \times 10$-CV statistical test proposed in \cite{Bouckaert2004} has been used for assessing the significance of the results.
%with confidence level 95\%TODO: a t-test [21]
% 
%  Typically, learning algorithms depend on a set of parameters, usually referred to as $\theta$. For the assessment of the predictive performance of an algorithm, we need a way to estimate the optimal values for such parameters.
%   We will present two types of experiments that adopt different parameter selection procedures, in order to assess in the more unbiased way the predictive performances of the proposed methods, and to compare the performance with other algorithms present in literature.
% The first experiments are performed in K-fold cross validation~\cite{Mitchell:1997:ML}, with K=10.
% %, since this is a widely adopted technique for the assessment of the performances of learning algorithms over finite datasets.
% 
% We compute the cross validation values over a grid of parameters $\theta$, and chose the parameters that minimize the CV error to be our best parameters estimates.
% This evaluation method allows us to compare the performance of the proposed algorithms with other previously published results, where for different reasons we were not able to recompute the experiments. 
% 
% When the cross validation is used for model selection (i.e. for parameter selection), as in our case, it is known that the results can be overly optimistic \cite{Cawley2007,Tibshirani}. Even if the effect applies to all learning algorithms, so the comparison should be fair, we decided to use also another parameter selection method, that more closely reflects the performance expected from the algorithm on unseen data.
% The second type of experiments adopt a technique commonly referred to as \textit{nested} k-fold cross validation. For each fold of the K-fold cross validation, we performed another \textit{inner} K-fold cross validation, in which we select the best parameters for that particular fold. Then, using only the best parameters for each fo the K folds, we classify the remaining examples (the test set for the particular iteration of K-fold).
% With this second approach, the parameters are optimized, for each fold, on the training dataset only, similarly to the approach adopted in \cite{NIPS2009_0533}.
% 
% When assessing the quality of the results the word significant will be used referring to the  statistical test referred as $10 \times 10$-CV proposed in \cite{Bouckaert2004}.
%with confidence level 95\%TODO: a t-test [21]

\subsection{Dataset Description} \label{sec:datasetdescription}

The experimentation has been performed on five datasets: %Mutag~\cite{Debnath1991}, 
CAS\footnote{http://www.cheminformatics.org/datasets/bursi}, CPDB~\cite{Helma2004}, AIDS~\cite{Weislow1989}, NCI1~\cite{springerlink:10.1007/s10115-007-0103-5} and GDD~\cite{dobson2003}. 
All datasets involve chemical compounds and represent binary classification problems. In all data sets nodes are labelled and there are no self-loops. 
%%Mutag, 
CAS, CPDB are dataset of mutagenic compounds whose target class represents whether or not they have a mutagenic effect. %the bacterium Salmonella typhimurium. 
NCI1 is a balanced subset of a dataset of chemical compounds screened for activity against non small cell lung cancer.  
AIDS is an antiviral screen dataset. 
%and ovarian cancer cell lines, respectively (Wale and Karypis, 2006, and http://pubchem.ncbi.nlm. nih.gov).  

 The GDD dataset comprises X-ray crystal structures of proteins. Each protein is represented by a graph, in which the nodes are amino acids and two nodes are connected by an edge if they are less than $6^\circ$  Angstroms apart. The examples are divided into enzymes and non-enzymes classes on the basis of Enzyme Commission number, annotations in the Protein Data Bank and Medline abstracts \cite{dobson2003}. 

Table~\ref{tab:datasets} summarizes the statistics of the datasets. 
% 
% 
% Mutag, CAS, CPDB are mutagenicity datasets, while AIDS and NCI1 are, respectively, antiviral and anti-cancer screen datasets.  
\begin{table}
%\vspace{0.1in}
\center
% % \caption{Statistics of MUTAG, CAS, CPDB, AIDS, NCI1 and GDD datasets: number of graphs, percentage of positive examples, average number of atoms, average number of edges.\label{tab:datasets}}
\caption{Statistics of CAS, CPDB, AIDS, NCI1 and GDD datasets: number of graphs, percentage of positive examples, average number of atoms, average number of edges.\label{tab:datasets}}
\begin{tabular}{|l|c|c|c|c|}
\hline
Dataset	&	graphs	& 	pos(\%)	&	avg atoms	& avg edges \\
\hline
%Mutag	&	$188$	&	$66.48$	&	$45.1$		& $47.1$ 	\\
CAS	&	$4337$	&	$55.36$	&	$29.9$		& $30.9$	\\
CPDB	&	$684$	&	$49.85$	&	$14.1$		& $14.6$	\\
AIDS	&	$1503$	&	$28.07$	&	$58.9$		& $61.4$	\\
NCI1	&	$4110$	&	$50.04$	&	$29.87$		& $32.3$	\\
GDD	&	$1178$	&	$58.65$	&	$284.31$	& $2862.63$	\\		
\hline
\end{tabular}
\end{table}

\subsection{Results} \label{sec:results}
This section is divided into two parts: in the first one we report experiments testing the effectiveness of the proposed kernels with respect to state-of-the-art competing approaches; in the second part we compare the same techniques with respect to their efficiency. 


\subsubsection{Efficacy evaluation}
We compare the predictive abilities of the kernels in Section~\ref{sec:frameworkinstances} with the Fast Subtree Kernel (FS), the Neighborhood Subgraph Pairwise Distance Kernel (NSPDK). %% and gBoost. 
% % In addition, results from the following algorithms, when available, are provided from~\cite{Saigo2009} and~\cite{Shervashidze2009a}: Gaston, Correlated Pattern Mining (CPM), MOLFEA, Marginalized Graph Kernel (MGK) and SVM with frequent pattern mining (freqSVM).  
The proposed kernel, as each of the kernel functions in the following, was employed together with a Support Vector Machine. %s 

%%In the following, we present two types of experiments that adopt different parameter selection procedures.
%  in order to compare the performance with other algorithms present in literature \cite{NIPS2009_0533,Costa2010,Saigo2008}, and to assess in the most unbiased way the predictive performances of the proposed methods.
% %   The first experiments are performed in K-fold cross validation, with K=10. We selected the best parameters a posteriori.
% % This evaluation method allows us to compare the performance of the proposed algorithms with other previously published results. 
% % It is known that when the cross validation is used for model selection (i.e. for parameter selection), as in our case, results can be overly optimistic \cite{Cawley2007,Tibshirani}. %more closely 
% % The second type of experiments adopts 
The kernels are evaluated on the datasets via a technique commonly referred to as \textit{nested} k-fold cross validation. For each fold of the K-fold cross validation, we performed another \textit{inner} K-fold cross validation, in which we select the best parameters for that particular fold. 
With this %second 
approach, the parameters are optimized, for each fold, on the training dataset only, similarly to the approach adopted in \cite{NIPS2009_0533}. 
% % In order to reduce the total time required for performing the experiments, we restricted to the four best performing kernels in the first set of experiments. 
%This experimental setting should reflect more closely the performance expected from the algorithm on unseen data.

% For the sake of comparison with the above mentioned results, the accuracy of each algorithm was measured by selecting a posteriori the best parameters among the average of $10$ repetitions of a $10-$fold cross validation.   
For all the experiments, the values of the parameters of the ODD-ST$_{h}$ and \nuovotk~kernels have been restricted to: $\lambda=\{0.1, 0.2, \ldots, 2.0\}$, $h=\{1, 2, \ldots, 10\}$. 
The parameter selection procedure for the Fast Subtree Kernel replicates the one described in~\cite{Shervashidze2009a}, i.e. only the parameter $h=\{1, 2, \ldots, 10\}$ is optimized. 
% % gBoost has many parameters, but following the parameter selection process exposed in~\cite{Saigo2009}, only $\mu$ (that controls training accuracy) has been optimized among the values $\{0.01, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6\}$. %, while other parameters of the method (minimum pattern size and minimum support) have been fixed. For more details please refer to~\cite{Saigo2009}.
% % For the parameters of the other methods, see to the corresponding papers. 
% The accuracy reported for each algorithm/kernel is computed as the average of $10$ repetitions 
All the experiments have been repeated $10$ times using different splits for the cross validation, and the average results (with standard deviation) are reported.

% % Table~\ref{tab:results} reports the average accuracy and the ranking obtained by the considered methods on the six datasets for the first set of experiments. 
% % \begin{table}
% % \centering
% %   \begin{tabular}{|l|c|c|c|c|c|c|}
% % \hline
% % $Kernel$ 		& Mutag   	& CAS 		& CPDB 		& AIDS 		& NCI1  	& GDD \\
% % \hline
% % %			& Acc		& Acc		& Acc 		& Acc		& Acc		& Acc \\
% % Gaston 			& -   		& 79.0 (6) 	& -  		& -  		& -  		& - \\
% % MOLFEA 			& -   		&  -  		& -  		& 78.5 (6) 	&  -   		& - \\
% % CPM 			& -   		& 80.1 (5)	& 76.0 (8)	& 83.2 (3)	&  -   		& - \\
% % MGK 			& 80.8 (6)	& 77.1 (8)	& 76.5 (7)	& 76.2 (8)	&  -   		& - \\
% % freqSVM 		& 80.8 (6)	& 77.3 (7)	& 77.8 (5)	& 78.2 (7)	&  -   		& - \\
% % gBoost 			& 85.2 (5)	& 82.5 (3)	& 78.8 (3) 	& 80.2 (4)	&  70.8 (5)   	&  - \\
% % %ST_param_learning	& 0.856	– 	& 0.8399 –	& 0.766	–	& 0.8256 –	& – – 		\\%& – – \\
% % FS			& $89.54$ (2) 	& $81.12$ (4) 	& $76.72$ (6)	& $78.45$ (5)	& \underline{$86.12$}  (1)	& \underline{$79.63$} (1) \\
% % 	& \tiny{\raisebox{0.2cm}{($\pm 0.99$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.17$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.96$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.67$)}}&  \tiny{\raisebox{0.2cm}{($\pm 0.21$)}} & \tiny{\raisebox{0.2cm}{($\pm 0.27$)}} \\
% % % 			& \tiny{(c=100,h=1)}& \tiny{(c=0.1,h=3)}& \tiny{(c=0.1,h=2)}& \tiny{(c=0.01,h=9)}&  \tiny{(c=0.01,h=8)} & \tiny{(c=0.1,h=1)} \\
% % NSPDK			& $88.61$ (4) 	& $84.35$ (2)	& $78.12$	(4)  	& $83.96$ (2) 	& $84.98$ (3)	& $76.09$ (4) \\
% %  			& \tiny{\raisebox{0.2cm}{($\pm 0.60$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.12$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.71$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.42$)}}&  \tiny{\raisebox{0.2cm}{($\pm 0.16$)}} & \tiny{\raisebox{0.2cm}{($\pm 0.35$)}} \\
% % % 			&(h=2,\ $\lambda$=0.5,\ c=1000) & & & & & \\
% % % $DDK_{ST_h}$		& 0.898 (2) 	& 0.844 (2)	& 0.794	 (2)  	& \underline{0.838} (1) 	& 0.839 (4)	& 0.776 (3) \\
% % % 			& \tiny{(c=10,h=1, $\lambda$ =1.8)}& \tiny{(c=10,h=3, $\lambda$ =1.6)}& \tiny{(c=10,h=2,$\lambda$=1.6)}& \tiny{(c=10,h=7,$\lambda$=1.8)}&  \tiny{(c=1000,h=4,$\lambda$=1)} & \tiny{(c=10,h=1,$\lambda$=1.4)} \\
% % $ODD-{ST_h}$		& $89.28$ (3) 	&  $83.97$(3)	& \underline{$79.62$}	 (1)  	& $83.6$(3) 	& $82.71$ (4)	& $77.92$(3) \\
% % 		& \tiny{\raisebox{0.2cm}{($\pm 0.74$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.21$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.59$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.34$)}}&  \tiny{\raisebox{0.2cm}{($\pm 0.20$)}} & \tiny{\raisebox{0.2cm}{($\pm 0.20$)}} \\
% % $ODD-{ST_+}$		& \underline{$89.92$} (1) 	& \underline{$84.40$} (1)	& $79.47$	 (2)  	& \underline{$83.99$} (1) 	& $85.46$ (2)	& $78.37$ (2) \\
% % & \tiny{\raisebox{0.2cm}{($\pm 0.18$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.91$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.18$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.52$)}}&  \tiny{\raisebox{0.2cm}{($\pm 0.45$)}} & \tiny{\raisebox{0.2cm}{($\pm 0.21$)}} \\
% % \hline
% % \end{tabular}
% % \normalsize
% %  \caption{Average accuracy results (when available) $\pm$ standard deviation in 10-fold cross validation for Gaston, MOLFEA, Correlated Pattern Mining, Marginalized Graph Kernel, SVM with Frequent Mining, gBoost, the Fast Subtree, the Neighborhood Subgraph Pairwise Distance, the $K_{ODD-ST_h}$ and the $K_{ODD-\nuovotk}$ kernels obtained on MUTAG, CAS, CPDB, AIDS, NCI1 and GDD datasets. The rank of the kernel is reported between brackets. \label{tab:results}}
% % \end{table}
\begin{table*}
\centering
 \caption{Average accuracy results $\pm$ standard deviation in nested 10-fold cross validation for the Fast Subtree, the Neighborhood Subgraph Pairwise Distance, the $K_{ODD-ST_h}$ and the $K_{ODD-\nuovotk}$ kernels obtained on MUTAG, CAS, CPDB, AIDS, NCI1 and GDD datasets. The rank of the kernel is reported between brackets. \label{tab:nestedkfoldresults}}
  \begin{tabular}{|l|c|c|c|c|c|c|}
\hline
$Kernel$ 		&  CAS 		& CPDB 		& AIDS 		& NCI1  	& GDD & Avg. Rank\\
\hline
FS			& $81.05$ {\tiny $\pm 0.21$} (4) 	& $73.37$ {\tiny $\pm 0.84$} (4)	& $75.35$ {\tiny $\pm 0.78$} (4)	& \underline{$84.79$} {\tiny $\pm 0.32$} (1)	& \underline{$76.29$} {\tiny $\pm 1.22$} (1) & ($2.8$) \\
NSPDK			& $83.6$~~ {\tiny $\pm 0.34$} (2)	& $76.99$ {\tiny $\pm 1.15$}	(1)  	& \underline{$82.71$} {\tiny $\pm 0.66$} (1) 	& $83.45$ {\tiny $\pm 0.43$} (3)	& $74.09$ {\tiny $\pm 0.91$} (4) & ($2.2$)\\
$ODD-{ST_h}$		& $83.34$ {\tiny $\pm 0.31$} (3)	& $76.44$ {\tiny $\pm 0.62$}	 (2)  	& $81.51$ {\tiny $\pm 0.74$} (3) 	& $82.10$ {\tiny $\pm 0.42$} (4)	& $75.27$ {\tiny $\pm 0.68$} (3) & ($3$)\\
$ODD-{ST_+}$		& \underline{$83.90$} {\tiny $\pm 0.33$} (1)	& $76.3$~ {\tiny $\pm 0.23$} (3)  	& $82.06$ {\tiny $\pm 0.70$} (2) 	& $84.60$ {\tiny $\pm 0.47$} (2)	& $75.33$ {\tiny $\pm 0.81$} (2) & ($2$)\\
\hline
\end{tabular}
% % \begin{table*}
% % \centering
% %  \caption{Average accuracy results $\pm$ standard deviation in nested 10-fold cross validation for the Fast Subtree, the Neighborhood Subgraph Pairwise Distance, the $K_{ODD-ST_h}$ and the $K_{ODD-\nuovotk}$ kernels obtained on MUTAG, CAS, CPDB, AIDS, NCI1 and GDD datasets. The rank of the kernel is reported between brackets. \label{tab:nestedkfoldresults}}
% %   \begin{tabular}{|l|c|c|c|c|c|c|}
% % \hline
% % $Kernel$ 		& Mutag   	& CAS 		& CPDB 		& AIDS 		& NCI1  	& GDD \\
% % \hline
% % FS			& $83.53$ {\tiny $\pm 2.5$}~ (3) 	& $81.13$ {\tiny $\pm 0.21$} (4) 	& $73.37$ {\tiny $\pm 0.84$} (4)	& $75.35$ {\tiny $\pm 0.78$} (4)	& \underline{$84.79$} {\tiny $\pm 0.32$} (1)	& \underline{$76.29$} {\tiny $\pm 1.22$} (1) \\
% % NSPDK			& \underline{$84.53$} {\tiny $\pm 1.33$} (1) 	& $83.58$ {\tiny $\pm 0.37$} (2)	& $75.23$ {\tiny $\pm 1.77$}	(3)  	& $81.94$ {\tiny $\pm 0.41$} (2) 	& $83.45$ {\tiny $\pm 0.43$} (3)	& $74.09$ {\tiny $\pm 0.91$} (4) \\
% % $ODD-{ST_h}$		& $83.82$ {\tiny $\pm 1.71$} (2) 	&  $83.34$ {\tiny $\pm 0.31$} (3)	& \underline{$76.87$} {\tiny $\pm 1.64$}	 (1)  	& $81.93$ {\tiny $\pm 0.72$} (3) 	& $82.10$ {\tiny $\pm 0.42$} (4)	& $75.27$ {\tiny $\pm 0.68$} (3) \\
% % $ODD-{ST_+}$		& $83.44$ {\tiny $\pm 2.13$} (4) 	& \underline{$83.90$} {\tiny $\pm 0.33$} (1)	& $75.66$ {\tiny $\pm 1.33$} (2)  	& \underline{$82.33$} {\tiny $\pm 0.85$} (1) 	& $84.60$ {\tiny $\pm 0.47$} (2)	& $75.33$ {\tiny $\pm 0.81$} (2) \\
% % \hline
% % \end{tabular}
% %   \begin{tabular}{|l|c|c|c|c|c|c|}
% % \hline
% % $Kernel$ 		& Mutag   	& CAS 		& CPDB 		& AIDS 		& NCI1  	& GDD \\
% % \hline
% % FS			& $83.53$ (3) 	& $81.13$ (4) 	& $73.37$ (4)	& $75.35$ (4)	& \underline{$84.79$}  (1)	& \underline{$76.29$} (1) \\
% % 			& \tiny{\raisebox{0.2cm}{($\pm 2.5$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.21$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.84$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.78$)}}&  \tiny{\raisebox{0.2cm}{($\pm 0.32$)}} & \tiny{\raisebox{0.2cm}{($\pm 1.22$)}} \\
% % NSPDK			& \underline{$84.53$} (1) 	& $83.58$ (2)	& $75.23$	(3)  	& $81.94$ (2) 	& $83.45$ (3)	& $74.09$ (4) \\
% % 			& \tiny{\raisebox{0.2cm}{($\pm 1.33$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.37$)}}& \tiny{\raisebox{0.2cm}{($\pm 1.77$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.41$)}}&  \tiny{\raisebox{0.2cm}{($\pm 0.43$)}} & \tiny{\raisebox{0.2cm}{($\pm 0.91$)}} \\
% % $ODD-{ST_h}$		& $83.82$ (2) 	&  $83.34$(3)	& \underline{$76.87$}	 (1)  	& $81.93$(3) 	& $82.10$ (4)	& $75.27$(3) \\
% % 			& \tiny{\raisebox{0.2cm}{($\pm 1.71$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.31$)}}& \tiny{\raisebox{0.2cm}{($\pm 1.64$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.72$)}}&  \tiny{\raisebox{0.2cm}{($\pm 0.42$)}} & \tiny{\raisebox{0.2cm}{($\pm 0.68$)}} \\
% % $ODD-{ST_+}$		& $83.44$ (4) 	& \underline{$83.90$} (1)	& $75.66$	 (2)  	& \underline{$82.33$} (1) 	& $84.60$ (2)	& $75.33$ (2) \\
% % 			& \tiny{\raisebox{0.2cm}{($\pm 2.13$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.33$)}}& \tiny{\raisebox{0.2cm}{($\pm 1.33$)}}& \tiny{\raisebox{0.2cm}{($\pm 0.85$)}}&  \tiny{\raisebox{0.2cm}{($\pm 0.47$)}} & \tiny{\raisebox{0.2cm}{($\pm 0.81$)}} \\
% % \hline
% % \end{tabular}
\normalsize
% \caption{ST+\label{tab:stplus}}
\end{table*}
% {\color{red}
% % According to the experimental results, gBoost tends to have a low ranking on most datasets, i.e. third, fourth and the fifth on three datasets. 
% % On the contrary, the Fast Subtree, while placing first on two datasets, has a lower ranking, i.e. second, fourth, fifth and sixth, on the other datasets. Its average ranking is $3.16$.  
% % Incidentally, $3.16$ is exactly the average ranking of NSPDK kernel as well.
% % % Thus, $3.16$ the best average ranking of competing kernels is .
% % Thus, $3.16$ is the average ranking to compare to our proposed kernels.
% %  $K_{ODD-\nuovotk}$ has best accuracy in three out of six datasets. On the remaining datasets it places in second  position. 
% % Notice that $ODD-{\nuovotk}$ almost always increases its accuracy with respect to $ODD-{ST_h}$ (the only exception being the CPDB dataset). The average rankings of $K_{ODD-\nuovotk}$ and $ODD-{ST_h} $are $1.5$ and $2.83$, respectively. 
% % % [SIGNIFICATIVITA']
% % These generally good results may be attributed to the fact that $K_{ODD-ST_h}$and $K_{ODD-\nuovotk}$ have associated a large feature space, which makes them more adaptable to different tasks. 
% % 
% % As stated at the beginning of this section, when the cross validation is used for model selection (i.e. for parameter selection), as in our case, it is known that the results can be overly optimistic \cite{Cawley2007,Tibshirani}. 
% % In the following, we will present and discuss a second type of experiments performed with the technique commonly referred as \textit{nested} 10-fold cross validation.
Table~\ref{tab:nestedkfoldresults} reports the average accuracy results obtained with this method for parameter selection. 
% % Note that in this case, there is no single setting of best parameters for each kernel/dataset, since different parameters are selected for each fold of each dataset.
% % The values in accuracy for all the datasets are lower with respect to the results in 10-fold cross validation reported in Table~\ref{tab:results}. However, the relative ranking of the kernels for each dataset is similar. The only dataset in which there is a difference is MUTAG.  We argue that this happens because the dataset is small, and the parameter selection procedure in this case is not reliable. It is evident looking at the high standard deviation presented by all the tested kernels on this dataset.
Note that $K_{ODD-\nuovotk}$ performs well on all datasets as the average rank on all datasets is $1.6$ compared to $2.8$ of the other kernels. 
These generally good results may be attributed to the fact that $K_{ODD-ST_h}$and $K_{ODD-\nuovotk}$ has associated a large feature space, which makes it more adaptable to different tasks. 

In order to better understand the differences in the performances of the various kernels, we analyzed the statistical significance among the accuracy results.
%  for the \textit{nested} 10-fold cross validation.
We assessed the significance using the $10 \times 10$-CV statistical test proposed in \cite{Bouckaert2004} with confidence level 95\%. %: a t-test [21]
% % As expected, on small datasets (MUTAG and CPDB) the difference between the various kernels is not statistically significant.
As expected, on the small CPDB dataset, the difference between the various kernels is not statistically significant.
%More interestingly, in other datasets the difference in performance is significant. 
In the AIDS and CAS datasets, NSPDK, $K_{ODD-ST_h}$ and $K_{ODD-{ST+}}$ perform significantly better than FS.
In the NCI1 dataset, FS and $K_{ODD-{ST+}}$ performs significantly better than NSPDK that, in turn, performs better than $K_{ODD-ST_h}$.
In the GDD dataset, FS, $K_{ODD-ST_h}$ and $K_{ODD-{ST+}}$ perform significantly better than NSPDK.
Let us analyze the significativity results, $K_{ODD-{ST+}}$ never performs significantly worse than the other kernels, while $K_{ODD-ST_h}$ performs significantly worse than competitors in only one dataset: NCI1. $K_{ODD-{ST+}}$ is significantly more accurate than FS on the AIDS and CAS datasets; it performs significantly better than NSPDK on NCI1 and GDD and it is more accurate than $K_{ODD-ST_h}$ on NCI1. 

\subsubsection{Efficiency evaluation}
In this section, we assess the efficiency of the proposed $K_{ODD-ST_h}$ and $K_{ODD-\nuovotk}$ kernels.
%  are compared with the NSPDK and FS kernel. 
In Section~\ref{sec:bigdag} we have proposed a technique for speeding up the kernel computation by compactly representing the ODDs by means of an Annotated DAG (BigDAG). The complexity of the DAG kernels, for example the ones described in Section~\ref{sec:frameworkinstances}, depends on the number of nodes of the BigDAG. 
In order to compare the bound on the number of nodes in eq.~\eqref{eq:bigdagnodes} and how it affects the complexity of the kernel, we have computed the number of nodes in each BigDAG as a function of the number of nodes of each graph. 
% In order to evaluate the actual complexities we have computed, for the $K_{ODD-ST_{h}}$ kernel, the number of nodes in each BigDAG on the NCI1 dataset. %%%%
\begin{figure}[ht]
	\centering
% 	\includegraphics[width=0.80\columnwidth]{figs/nodesNCIall-eps-converted-to.pdf}
	\includegraphics[width=0.80\columnwidth]{plots/bigDAG_NCI1_unlimited.pdf}
	\caption{Number of nodes inserted into each BigDAG as a function of the total nodes of the graphs in the NCI1 dataset. \label{fig:dagnodes}}
% 	The plots refer to NCI1 with limitation to the depth of the visits ($h=6$).
\end{figure}
\begin{figure}[ht]
	\centering
% 	\includegraphics[width=0.80\columnwidth]{figs/nodesNCIall-eps-converted-to.pdf}
	\includegraphics[width=0.80\columnwidth]{plots/bigDAG_CAS_unlimited.pdf}
	\caption{Number of nodes inserted into each BigDAG as a function of the total nodes of the graphs in the CAS dataset. \label{fig:dagnodescas}}
% 	The plots refer to NCI1 with limitation to the depth of the visits ($h=6$).
\end{figure}
The plots in Figure~\ref{fig:dagnodes} refer to the NCI1 dataset while the plots in Figure~\ref{fig:dagnodescas} refer to the CAS dataset. 
We have also plotted the polynomial function interpolating these points: such function is $n^{1.3691}$ for NCI1 and $n^{1.3652}$ fo CAS. In order to have a comparison with the values of the bounds discussed in Section~\ref{sec:bigdag}, the functions $n^\frac{3}{2}$ and $n^2$ are plotted as well. 
The points of the plot, i.e. the numbers of nodes inserted in the BigDAG are, for the vast majority, under the curve $n^{1.5}$ for both datasets.  
The size of the BigDAG tends to an asymptotic value which depends on the outdegree of the nodes and the size of the longest cycle (see Section~\ref{sec:h}). In this case, the ``actual'' complexity of the kernel is proportional (via $H$) to $n\log n$. 
Similar results are obtained for the other datasets. The interpolating functions are: %$n^{1.2774}$ for MUTAG, 
$n^{1.3001}$ for CPDB, $n^{1.2571}$ for AIDS and $n^{1.672}$ for GDD. 

Figure~\ref{fig:tempinci1} and Figure~\ref{fig:tempicas} report the time needed to compute the kernel matrix, as a function of $h$, for the
% $K_{\text{ODD-ST}_{h}}$ and the FS
$K_{\text{ODD-ST}_{h}}$, $K_{\text{ODD-\nuovotk}}$, NSPDK and the FS kernels on NCI1 and CAS, respectively. 
All the experiments are performed on a PC with two Quad-Core AMD Opteron(tm) 2378 Processors and 64GB of RAM. 
%Computation times are divided into the components \textit{preprocessing} and \textit{kernel computation}. %The preprocessing phase includes all steps needed for the generation of the $Big^{2}DAG$. The kernel computation
%includes the computation of the kernel matrices varying the $\lambda$ parameter. 
Given that the available implementations of the two kernels are in different programming languages \nuovo{(FS in Matlab and the others in C++)}{Rev 3, chapter 7 commento 3}, the plots of the FS kernel were added just for a qualitative comparison.  
Notice that, as $h$ increases, the time required for computing the kernel matrix seems to increase almost linearly for FS and $ST_h$. 
This can be explained with the fact that smaller graphs do not allow too deep visits, so the increase in complexity due to the increase of the depth visit is compensated by the smaller number of graphs where visits of that depth can be actually performed. 
\begin{figure}[ht]
	\centering
	\includegraphics[width=0.80\columnwidth]{figs/times_journal_NCI1.pdf}
	\caption{Time needed to compute the kernel matrix, as a function of $h$, for the $K_{\text{ODD-ST}_{h}}$, $K_{\text{ODD-\nuovotk}_{h}}$, the NSPDK and the FS kernels on NCI1.\label{fig:tempinci1}}
\end{figure}
\begin{figure}[ht]
	\centering
	\includegraphics[width=0.80\columnwidth]{figs/times_journal_CAS.pdf}
	\caption{Time needed to compute the kernel matrix, as a function of $h$, for the $K_{\text{ODD-ST}_{h}}$, $K_{\text{ODD-\nuovotk}_{h}}$, the NSPDK and the FS kernels on CAS dataset.\label{fig:tempicas}}
\end{figure}
% Table~\ref{tab:tempi} reports the average computational time for a single fold with the optimal parameters on the four largest datasets: CAS, AIDS, NCI1, GDD. The parameters influencing the speed of the kernel are reported between brackets. 
% \begin{table*}
%   \centering
%  \begin{tabular}{|l|l|l|l|l|}
%   \hline
%   Kernel	& CAS 			&  AIDS 		& NCI1			& GDD	\\
%   \hline
%   FS		& $77$ (h=$3$)		&  $30$ (h=$9$) 	& $246$ (h=$8$) 	& $405$	(h=$1$) \\
%   NSPDK		& $24$ (h=$2$,d=$6$)	&  $217$ (h=$8$,d=$6$)	&$192$ 	(h=$5$,d=$4$)	& $395$	(h=$2$,d=$6$)\\
%   ODD-ST$_h$ 	& $18$ (h=$3$)		&  $56$ (h=$7$)		& $44$	(h=$4$)		& $29$ (h=$1$) \\
%   ODD-\nuovotk	& $32$ (h=$4$)		&  $111$ (h=$8$)	&$205$ 	(h=$1$)		& $199$ (h=$1$)\\
%   \hline
%  \end{tabular}
%    \caption{Average seconds required for computing the kernel matrix on CAS, AIDS, NCI1 and GDD dataset with the optimal parameters. The parameters influencing the speed of the kernel are reported between brackets.\label{tab:tempi}}
% \end{table*}
%
% Such data are combined with the one from Table~\ref{tab:results} to obtain Figure~\ref{fig:ranking}: on the x-axis the $K_{\text{ODD-ST}_{h}}$, $K_{\text{ODD-\nuovotk}}$, NSPDK and the FS kernels are ranked with respect to the classification accuracies reported in Table~\ref{tab:results}. Given the kernel parameters yielding the best accuracy values, on the y-axis the same kernels are ranked with respect to the average time needed to classify a novel example after the learning phase. 
% The purpose of Figure~\ref{fig:ranking} is to combine the estimate of prediction accuracy with the speed for classifying novel examples. 
% We used rankings instead of the actual values in order to be able to harmonize results from different datasets. 
% Note that the $K_{\text{ODD-ST}_{h}}$ kernel values tend to be on the lower left corner, thus having best accuracy and speed. 




Finally, in Table~\ref{tab:tempi} we report the average computational time for a single fold with the optimal parameters on the four largest datasets: CAS, AIDS, NCI1, GDD. The parameters influencing the speed of the kernel are reported between brackets. 
\subsection{Discussion}
If we compare the kernels both from the accuracy and the efficiency point of view by looking at %Table~\ref{tab:results},
 Table~\ref{tab:nestedkfoldresults} and Table~\ref{tab:tempi} together, it can be noticed that $K_{ODD-{ST_{+}}}$ reaches the best predictive performances on the considered datasets, while it  does not demand more computational resources than NSPDK.
On the other hand, if the computational burden is an issue, $K_{ODD-{ST_{h}}}$ is able to reach comparable accuracies as NSPDK (except for the NCI1 dataset) and FS kernel,
%  state of the art results 
while being the most efficient among the considered kernels.

The above considerations suggest that the proposed framework is flexible enough to allow the definition of graph kernels suitable for different scenarios.
%On the other hand, NSPDK performs significantly worse than $ODDK_{ST+}$ in GDD and NCI1, and worse than $K_{ODD-ST_h}$ in GDD.
%FS performs worse than $K_{ODD-ST_h}$ and $ODDK_{ST+}$ in CAS and AIDS datasets. 
% 
% According to the experimental results, gBoost tends to have a low ranking on most datasets, i.e. third, fourth and the fifth on three datasets. 
% On the contrary, the Fast Subtree, while placing first on two datasets, has a lower ranking, i.e.second, fourth, fifth and sixth, on the other datasets. Its average ranking is $3.16$.  
% By a curious coincidence, $3.16$ is exactly the average ranking of NSPDK kernel as well.
% Thus, the best average ranking of competing kernels is $3.16$.
%  $K_{ODD-\nuovotk}$ has best accuracy in three out of six datasets. On the remaining datasets it places in second  position. 
% Notice that $K_{ODD-\nuovotk}$ almost always increases its accuracy with respect to the one of $K_{ODD-ST_h}$ (the only exception being the CPDB dataset). The average rankings of $K_{ODD-\nuovotk}$ and $K_{ODD-ST_h}$are $1.5$ and $2.83$, respectively. 
% % [SIGNIFICATIVITA']
% These generally good results may be attributed to the fact that $K_{ODD-ST_h}$and $K_{ODD-\nuovotk}$ have associated a large feature space, which makes them more adaptable to different tasks. 
% 
% As stated in the beginning of this section, when the cross validation is used for model selection (i.e. for parameter selection), as in our case, it is known that the results can be overly optimistic \cite{Cawley2007,Tibshirani}. 
% In the following, we will present and discuss a second type of experiments performed with the technique commonly referred as \textit{nested} 10-fold cross validation.
% Table~\ref{tab:nestedkfoldresults} reports the accuracy results with this method for parameter selection. Note that in this case, there is not a single setting of best parameters for each kernel/dataset, since different parameters are selected for each fold of each dataset.
% The overall accuracy of the methods are lower with respect to the results in 10-fold cross validation reported in Table~\ref{tab:results} . However, the relative positioning of the kernels for each dataset is similar. The only dataset in which there is a difference in  the ranking of the kernels between the two different evaluation methods is MUTAG.  We argue that this happens because the dataset is small, and the parameter selection procedure in this case is not reliable.
% 
% In order to better understand the differences in the performances of the various kernels, we analyzed the statistical significance among the accuracy results for the \textit{nested} 10-fold cross validation.
% We assessed the significance using the $10 \times 10$-CV statistical test proposed in \cite{Bouckaert2004} with confidence level 95\%. %: a t-test [21]
% 
% As expected, on small datasets (MUTAG and CPDB) the difference between the various kernels is not statistically significant.
% More interestingly, in other datasets the difference in performance is significant. 
% In the AIDS and CAS datasets, NSPDK, $K_{ODD-ST_h}$ and $ODDK_{ST+}$ perform significantly better than FS.
% In the NCI1 dataset, FS and $ODDK_{ST+}$ performs significantly better than NSPDK that, in turn, performs better than $K_{ODD-ST_h}$.
% In the GDD dataset, FS, $K_{ODD-ST_h}$ and $ODDK_{ST+}$ perform significantly better than NSPDK.
% 
% Analyzing the significativity results, $ODDK_{ST+}$ never performs significantly worse respect the other kernels, while $K_{ODD-ST_h}$ performs significantly worse than competitors in only one dataset: NCI1.
%On the other hand, NSPDK performs significantly worse than $ODDK_{ST+}$ in GDD and NCI1, and worse than $K_{ODD-ST_h}$ in GDD.
%FS performs worse than $K_{ODD-ST_h}$ and $ODDK_{ST+}$ in CAS and AIDS datasets. 
% }

%According to the experimental results, gBoost tends to have a low ranking on most datasets, i.e. third, fourth and the fifth on three datasets. 
%On the contrary, the Fast Subtree, while placing first on two datasets, has a lower ranking, i.e. fourth, fifth, sixth and seventh, on the other datasets. Its averagre ranking is $4$.  
%The best average ranking of competing kernels is the one of the NSPDK: $3.083$.
% ODD-\nuovotk has best accuracy in four out of six datasets. On the remaining datasets it places in second and third position. 
%Notice that ODD-\nuovotk always increases its accuracy with respect to the one of ODD-ST$_h$. The average rankings of ODD-\nuovotk and ODD-ST$_h$ are $1.583$ and $2.5$, respectively. 
% [SIGNIFICATIVITA']
%These generally good results may be attributed to the fact that ODD-ST$_h$ and ODD-\nuovotk have associated a large feature space, which makes them more adaptable to different tasks. 
%--------------------------
% In order to compare our performance with the other methods with attention to fairness, we calculated the total (average) time needed to train a single round of k-fold cross validation with the optimal parameters (reported in table~\ref{tab:results}) for each method.
% Indeed, when applying cross validation, kernel methods has to compute the kernel matrix only once for each parameter configuration, and the only thing that needs to be repeated is the SVM algorithm. On the contrary, gBoost needs to repeat his whole execution for each different fold, because the model it generates is based on the frequency of subgraphs in the training set.
%  We performed this experiment on the biggest dataset we employed, namely CAS. $K_{ST_{h}}$ kernel took $561$ seconds to compute the kernel matrix and $2.4$ seconds for the SVM to converge. FS kernel took $113$ seconds for the computation of the kernel matrix, and $4.2$ seconds for the training of the SVM. GBoost took approximately $4000$ seconds.

% This generally good results may be attributed to the fact that $ODD-ST_h$ has associated a large feature space, which makes it more adaptable to different datasets. 
% 
% %On the MUTAG dataset the proposed kernel performs better than the Fast Subtree kernel, while it is not significantly worse than the Shortest path kernel. On NCI1 and NCI109 it outperforms all other kernels. 
% %Notice that overall $K_{ST_{h}}$ gets the best rank among all the tested kernels.  
% 
% In sections~\ref{sec:bigdag} we have proposed a technique for speeding up the kernel computation by compactly representing the ODDs by means of an Annotated DAG (BigDAG). The complexity of the DAG kernels, and thus of $K_{ST}$ and $K_{ST_{h}}$, depends on the number of nodes of the BigDAG. 
% %In fact the idea behind the limited version of the kernels is to reduce the number of nodes in the BigDAG that is being generated.
% In order to evaluate the actual complexities, on the NCI1 dataset, we have computed the actual number of nodes generated for each BigDAG, with a limit on the depth of the visits. 
% The obtained figures are plotted in Figure~\ref{fig:dagnodes} as a function of the nodes of the graphs. We have also plotted the exponential function interpolating these points. In order to have a comparison with the values of the bounds discussed in Section~\ref{sec:bigdag}, the functions $n^\frac{3}{2}$, $n^2$ are plotted as well. 
% The number of nodes inserted in the BigDAG for the dataset for $K_{ST_{h}}$ are for the vast majority of points under the curve $n^{1.5}$. The size of the BigDAG tends to an asymptotic value with the number of nodes contained in the input graphs (see Section~\ref{sec:h}). In this case, the ``actual'' complexity of the kernel is proportional (via $H$) to $n\log n$. 
% %be significantly lower than $n^2$ and this is true for almost all the points also with respect to $n^\frac{3}{2}$. This means that the ``actual'' time complexity of $K_{ST}$ for the  considered dataset can be considered proportional to  $n^{3/2}\log n$. 
% Similar results are obtained for the other datasets. 
% %The number of nodes inserted in the BigDAG for the dataset in the non-limited version of the kernel tends to be significantly lower than $n^2$ and this is true for almost all the points also with respect to $n^\frac{3}{2}$. This means that the ``actual'' time complexity of $K_{ST}$ for the  considered dataset can be considered proportional to  $n^{3/2}\log n$. 
% %Basically the same behaviour is observed also for $K_{ST_{h}}$, i.e. the limited version of the kernel, where we can notice a different curve for the number of nodes in the BigDAGs. In fact, for small graphs the number of nodes inserted in the BigDAG is larger with respect to the non-limited version, however the size of the BigDAGs tends to an asymptotic value with the number of nodes contained in the input graphs (see Section~\ref{sec:h}). In this case, the ``actual'' complexity of the kernel is proportional (via $H$) to $n\log n$. 
% %i valori dei parametri migliori
% 
% % Let us now turn our attention the computational time required by the gBoost, the Fast Subtree and the $K_{ST_{h}}$ kernel. The following comparison is a qualitative one, since the algorithms are implemented in different languages and have been executed on different, although comparable, machines. Figure~\ref{tab:tempinci1} reports the time required for the computation of the kernel matrix for gBoost, the Fast Subtree and $K_{ST_{h}}$ for different values of the parameter $h$. 
% % 
% % \begin{figure*}[ht]
% % 	\includegraphics[width=1.0\columnwidth]{figs/tempinci1.pdf}
% % 	%\includegraphics[width=1.0\columnwidth]{figs/nodesNCIall_h6.pdf}
% % 	\caption{Time in seconds required for the computation of the kernel matrix for NCI1 and CAS.\label{fig:confrontotempi}}
% % \end{figure*}
% 
% %The complexity of the Shortest Path kernel is $O(n^4)$ and the complexity of the Fast Subtree kernel is $O(mh)$, where $m$ is the number of edges of the graph and $h$ is the maximum number of levels of a breadth-first visit of the graph (see \cite{Shervashidze2009a} for details). 
% 
% Table~\ref{tab:timeresults} gives an idea of the time needed to compute the $K_{ST_{h}}$ kernel.
% All the times reported in tables, figures and in the following paragraphs refers to executions in a PC with two Quad-Core AMD Opteron(tm) 2378 Processors and 64GB of RAM.
% 
% 
% Computation times are divided into the components \textit{preprocessing} and \textit{kernel computation}. The preprocessing phase includes all steps needed for the generation of the $Big^{2}DAG$. The kernel computation
% includes the computation of the kernel matrices varying the $\lambda$ parameter.
% 
% 
% %Note that we adopted the $Big^{2}DAG$ technique for our experiments. %In D\&D dataset this slowed down the computation compared to the classic pairwise kernel matrix computation method because the graphs in this dataset have high connectivity ($p$ value), which contributes to return an high $H$ value.
% %Since, in the experiments, $h$ is proportional to $n$ for the three datasets, the complexity of the Fast subtree becomes $O(n^2)$. 
% In order to compare our performance with the other methods with attention to fairness, we calculated the total (average) time needed to train a single round of k-fold cross validation with the optimal parameters (reported in table~\ref{tab:results}) for each method.
% Indeed, when applying cross validation, kernel methods has to compute the kernel matrix only once for each parameter configuration, and the only thing that needs to be repeated is the SVM algorithm. On the contrary, gBoost needs to repeat his whole execution for each different fold, because the model it generates is based on the frequency of subgraphs in the training set.
%  We performed this experiment on the biggest dataset we employed, namely CAS. $K_{ST_{h}}$ kernel took 561 seconds to compute the kernel matrix and 2.4 seconds for the SVM to converge. FS kernel took 113 seconds for the computation of the kernel matrix, and 4.2 seconds for the training of the SVM. GBoost took approximately 4000 seconds.
% 
% \begin{figure}[ht]
% %	\includegraphics[width=0.55\columnwidth]{figs/nodesMutag-eps-converted-to.pdf}
% %	\includegraphics[width=0.55\columnwidth]{figs/nodesPTC_FM-eps-converted-to.pdf}
% %	\includegraphics[width=0.55\columnwidth]{figs/nodesPTC_FR-eps-converted-to.pdf}
% %	\includegraphics[width=0.55\columnwidth]{figs/nodesPTC_MR-eps-converted-to.pdf}
% %	\includegraphics[width=0.55\columnwidth]{figs/nodesPTC_MM-eps-converted-to.pdf}
% 	\includegraphics[width=1.0\columnwidth]{figs/tempinci1.pdf}
% 	%\includegraphics[width=1.0\columnwidth]{figs/nodesNCIall_h6.pdf}
% 	\label{fig:dagnodes}
% 	\caption{Time requested for the computation of the ST-based kernel for DAGs with limited visits on NCI1 and CAS in function of $h$. The two lines show the times for each dataset. \label{tab:timeresults}}
% \end{figure}
% 
% % \begin{table*}
% % \caption{Time requested for the computation of the ST-based kernel for DAGs with limited visits on MUTAG, NCI1 and D\&D in function of $h$. The two tables show the times for the preprocessing and the kernel matrix computation steps, respectively. \label{tab:timeresults}}
% % \vspace{0.1in}
% % \center
% % \begin{tabular}{|l|c|c|c|}
% % \hline
% % \multicolumn{4}{|c|}{Preprocessing} \\
% % \hline
% % $h$  & CAS \\
% % \hline
% % 9 & 4.46'  \\
% % 8 & 3.68' \\
% % 7 &2.95'  \\
% % 6 & 2.31'\\
% % 5 & 1.63'\\
% % 4 & 1.03' \\
% % 3 &37'' \\
% % 2 &21''\\
% % 1 & 14 '' \\
% % \hline
% % \end{tabular}
% % \begin{tabular}{|l|c|c|c|}
% % \hline
% % \multicolumn{4}{|c|}{Kernel Computation} \\
% % \hline
% % $h$  & CAS \\
% % \hline
% % 9 & 11.76''  \\
% % 8 & 11.76'  \\
% % 7 &11.35' \\
% % 6 &10.98' \\
% % 5 & 10.25' \\
% % 4 & 8.31' \\
% % 3 & 6.41' \\
% % 2 & 3.46'\\
% % 1 &1.68' \\
% % \hline
% % \end{tabular}
% % % \begin{tabular}{|l|c|c|c|}
% % % \hline
% % % \multicolumn{4}{|c|}{Preprocessing} \\
% % % \hline
% % % $h$  & MUTAG & NCI1 & D\&D \\
% % % \hline
% % % 10 & 11'' & 14' & --\\
% % % 9 & 10'' &12'  & -- \\
% % % 8 & 10'' &10'& -- \\
% % % 7 &8'' & 8' & 96.6' \\
% % % 6 &6''& 6.5'& 66.4'\\
% % % 5 &4''& 5.8'& 38.4'\\
% % % 4 &2''& 5.4' &22.5' \\
% % % 3 &2''& 3.1' & 12.5' \\
% % % 2 &1''& 2' & 6.5'\\
% % % 1 &
% % % \hline
% % % \end{tabular}
% % % \begin{tabular}{|l|c|c|c|}
% % % \hline
% % % \multicolumn{4}{|c|}{Kernel Computation} \\
% % % \hline
% % % $h$  & MUTAG & NCI1 & D\&D \\
% % % \hline
% % % 10 & 1'' & 10' & -- \\
% % % 9 & 1'' &10' & -- \\
% % % 8 & 1'' & 10' & -- \\
% % % 7 &1''& 10' & 6.3' \\
% % % 6 &1''& 9.5' & 5.6' \\
% % % 5 &1''& 8.4' & 5.6' \\
% % % 4 &1''&8.4' &4.4' \\
% % % 3 &$<$1''& 4.6'&3' \\
% % % 2 &$<$1''& 2.5' & 33'' \\
% % % \hline
% % % \end{tabular}
% % \end{table*}
% 
% 
% 
% %Notice that the kernel we used is a port of a tree kernel to work on DAGs, and is not defined to perform well on these context.
% %So we can assert that defining a DAG-specific kernel to use in our framework will give higher classification performance.
% %As previously mentioned we must take into consideration also the computational complexity of the kernels we take into consideration.
% %The fast subtree kernel has a ``more-than-quadratic'' complexity in MUTAG (where the $h$ parameter of the kernel is above $n/2$ for most graphs, see \cite{Shervashidze2009a} for the kernel formulation) and performs poorly on this dataset. The Shortest path kernel have $O(n^{4})$ complexity and placed second. ODD kernel with Partial tree kernel, in this dataset, have a complexity near $O(p^{3}n^{3})$, and performs better than other kernels.
% %
% %On NCI1 dataset the Shortest path kernel do not achieve good results, whereas the fast subtree kernel do. On this dataset the performance of ODD kernel are not distant from that of the fast subtree.
% %We should observe that ODD kernel achieve always a high accuracy level, hence it represent a significant similarity measure between graphs.
% 
% We further report the average computational time for a single fold with the optimal parameters on CAS, since it is the largest dataset. The ODD-ST$_h$ kernel took $86$ seconds to compute the kernel matrix and $2.4$ seconds for the SVM to converge; FS kernel took $282$ seconds for the computation of the kernel matrix, and $4.2$ seconds for the training of the SVM. gBoost took approximately $4000$ seconds.
% All the experiments are performed on a PC with two Quad-Core AMD Opteron(tm) 2378 Processors and 64GB of RAM. 
% 
\begin{table}
  \centering
   \caption{Average seconds required for computing the kernel matrix on CAS, AIDS, NCI1 and GDD dataset with the optimal parameters. The parameters influencing the speed of the kernel are reported between brackets.\label{tab:tempi}}
 \begin{tabular}{|l|l|l|l|l|}
  \hline
  Kernel	& CAS 			&  AIDS 		& NCI1			& GDD	\\
  \hline
  FS		& $77$ (h=$3$)		&  $30$ \hfill (h=$9$) 	& $246$ (h=$8$) 	& $405$	(h=$1$) \\
  NSPDK		& $24$ (h=$2$,		&  $217$ (h=$8$,	&$192$ 	(h=$5$,		& $395$	(h=$2$,\\
		&	\hfill d=$6$)	& \hfill d=$6$)		& \hfill d=$4$)		& \hfill d=$6$)		\\
  ODD-ST$_h$ 	& $18$ (h=$3$)		&  $56$ \hfill (h=$7$)	& $44$ \hfill (h=$4$)	& $29$ \hfill (h=$1$) \\
  ODD-\nuovotk	& $32$ (h=$4$)		&  $111$ (h=$8$)	&$205$ 	(h=$1$)		& $199$ (h=$1$)\\
  \hline
 \end{tabular}
\end{table}

% \begin{figure}[ht]
% 	\centering
% 	\includegraphics[width=0.75\columnwidth]{figs/rankings.pdf}
% 	\caption{Ranking of the $K_{\text{ODD-ST}_{h}}$, $K_{\text{ODD-\nuovotk}}$, NSPDK and the FS kernels with respect to classification accuracy on the x-axis and ranking of the average time needed to classify a test example on the y-axis.\label{fig:ranking}}
% \end{figure}


==> experimentsneurocomputing_oldresults.tex <==
\section{Experimental results}\label{sec:exps}
\subsection{\textcolor{red}{Experiments on common benchmark graph datasets}}\label{expsold}
\begin{table}[t]
%\vspace{0.1in}
\center
% % \caption{Statistics of MUTAG, CAS, CPDB, AIDS, NCI1 and GDD datasets: number of graphs, percentage of positive examples, average number of atoms, average number of edges.\label{tab:datasets}}
\begin{tabular}{|l|c|c|c|c|}
\hline
Dataset	&	graphs	& 	pos(\%)	&	avg nodes	& avg edges \\
\hline
%Mutag	&	$188$	&	$66.48$	&	$45.1$		& $47.1$ 	\\
CAS	&	$4337$	&	$55.36$	&	$29.9$		& $30.9$	\\
CPDB	&	$684$	&	$49.85$	&	$14.1$		& $14.6$	\\
AIDS	&	$1503$	&	$28.07$	&	$58.9$		& $61.4$	\\
NCI1	&	$4110$	&	$50.04$	&	$29.9$		& $32.3$	\\
NCI109 & $4127$ & $50.37$ & $29.7$ & $32.1$\\
GDD	&	$1178$	&	$58.65$	&	$284.3$	& $2862.6$	\\		
\hline
MSRC\_9 & 221 & multi-class & 40.6 & 97.9 \\
MSRC\_21& 563& multi-class & 77.5 & 198.3 \\
\hline
NCI123 & 40952 & 4.76 & 26.8 & 28.9 \\
NCI\_AIDS & 42682 & 3.52 & 45.7 & 47.7 \\
\hline
\end{tabular}
\caption{Statistics of CAS, CPDB, AIDS, NCI1 , NCI109, GDD, MSRC\_9, MSRC\_21, NCI123 and NCI\_AIDS datasets: number of graphs, percentage of positive examples, average number of atoms, average number of edges.\label{tab:datasets}}
\end{table}
The experimental assessment of the proposed approach has been performed on a total of eight datasets.  The first six datasets involve chemo and bioinformatics data: CAS\footnote{http://www.cheminformatics.org/datasets/bursi},
CPDB~\cite{Helma2004}, AIDS~\cite{Weislow1989}, NCI1, NCI109~\cite{springerlink:10.1007/s10115-007-0103-5} and GDD~\cite{dobson2003}. 
The first five datasets involve chemical compounds and represent binary classification problems. The nodes are labeled according to the atom type and the edges represent the bonds.
GDD is a dataset composed by proteins represented as graphs, where the nodes of the graphs represent amino acids and two nodes are connected by an edge if they are less than 6{\AA} apart.
\textcolor{black}{Moreover, we adopted from \cite{Birlinghoven} two real-world image datasets: MSRC9-class and MSRC21-class\footnote{\mbox{http://research.microsoft.com/en-us/projects/ObjectClassRecognition/}}. Each image is represented by its conditional Markov random field graph enriched with semantic labels, and the task is scene classification. Both the datasets are multi-class single-label classification problems.
For our experiments, we adopted a SVM classifier~\cite{Pedregosa2012}. For the multi-class problems, we adopted a  one-vs-one scheme.}
%
%For more details on the datasets, please refer to the cited papers. 
% % % % % \begin{table*}[t!]
% % % % % \centering
% % % % %   \begin{tabular}{|l|c|c|c|c|c|c|}
% % % % % \hline
% % % % % \scriptsize $Kernel$ 		& \scriptsize  CAS 		& \scriptsize CPDB 		& \scriptsize AIDS 		& \scriptsize NCI1  	& \scriptsize GDD & \scriptsize NCI109\\ %& Rank\\
% % % % % \hline
% % % % % \scriptsize FS 	&  $83.32$ (6)	&  $76.36$ (4) & $82.02$ (5)  &  $84.41$ (3) & $75.46$ (2) \vspace{-0.1cm}& {\bfseries85.02 } (1) \\ %& $(4)$  \vspace{-0.2cm}\\
% % % % %  & {\tiny $\pm 0.37$} & {\tiny $\pm 1.48$} & {\tiny $\pm 0.4$} & {\tiny $\pm 0.49$} & {\tiny $\pm 0.98$}& {\tiny $\pm 0.44$} \\
% % % % % \scriptsize NSPDK			& $83.60$ (2)	& {\bfseries 76.99}	(1)  	& {\bfseries 82.71}  (1) 	& $83.45$  (5)	& $74.09$  (6) \vspace{-0.1cm}& $84.17$ (3) \\ %& ($3.2$) \vspace{-0.2cm}\\
% % % % % & {\tiny $\pm 0.34$} &  {\tiny $\pm 1.15$}&   {\tiny $\pm 0.66$} & {\tiny $\pm 0.43$} & {\tiny $\pm 0.91$} & {\tiny $\pm 0.33$}\\
% % % % % \scriptsize ODD$_{\text{ST}_h}$		& $83.34$  (5)	& $76.44$ 	 (3)  	& $81.51$  (6) 	& $82.10$  (6)	& $75.27$  (4) \vspace{-0.1cm}& $81.91$ (6)\\ %& ($5$) \vspace{-0.2cm}\\
% % % % % & {\tiny $\pm 0.31$}  &  {\tiny $\pm 0.62$} & {\tiny $\pm 0.74$} & {\tiny $\pm 0.42$} & {\tiny $\pm 0.68$} & {\tiny $\pm 0.42$}\\
% % % % % \scriptsize ODD$_{\text{ST}_h}^{\text{\tiny{TANH}}}$		& {$83.37$}  (4)	& $76.45$ (2)  	& $82.54$  (2) 	& $84.35$  (4)	& {\bfseries 75.62}  (1) \vspace{-0.1cm}& 83.45 (4)\\%& ($2.4$) \vspace{-0.2cm}\\
% % % % % & {\tiny $\pm 0.5$} & {\tiny $\pm 1.13$} & {\tiny $\pm 0.57$} & {\tiny $\pm 0.44$} &{\tiny $\pm 1.1$}& {\tiny $\pm 0.35$} \\
% % % % % \scriptsize ODD$_{\text{ST}_+}$		&  {\bfseries 83.90}  (1)	& $76.30$  (6)  	& $82.06$  (4) 	& {\bfseries 84.97} (1)	& $75.33$  (3) \vspace{-0.1cm}& $83.08$ (5)\\%& ($3$) \vspace{-0.2cm}\\
% % % % % & {\tiny $\pm 0.33$} & {\tiny $\pm 0.23$} & {\tiny $\pm 0.70$} & {\tiny $\pm 0.47$} & {\tiny $\pm 0.81$}& {\tiny $\pm 0.49$} \\
% % % % % \scriptsize ODD$_{\text{ST}_+}^{\text{\tiny{TANH}}}$		& {$83.39$}  (3)	& $76.31$ (5)  	& $82.54$ (2) 	& $84.69$  (2)	& $74.60$ (5) \vspace{-0.1cm}& 84.33(2)\\%& ($3.2$) \vspace{-0.2cm}\\
% % % % % & {\tiny $\pm 0.34$} & {\tiny $\pm 1.72$} & {\tiny $\pm 0.90$} & {\tiny $\pm 0.34$} & {\tiny $\pm 0.68$} & {\tiny $\pm 0.27$}\\
% % % % % \hline
% % % % % \end{tabular}
% % % % %  \caption{Average accuracy results $\pm$ standard deviation in nested 10-fold cross validation for the Fast Subtree, the Neighborhood Subgraph Pairwise Distance, the $ODD_{ST_h}$ and the $ODD_{\nuovotk}$ kernels obtained on CAS, CPDB, AIDS, NCI1 and GDD datasets. The rank of the kernel is reported between brackets. \label{tab:nestedkfoldresults}}
% % % % % \end{table*}
\begin{table}[t!]
\begin{center}
\begin{tabular}{|l|c|c|c|c|}
\hline
\scriptsize $Kernel$ 		& \scriptsize  CAS 		& \scriptsize CPDB 		& \scriptsize AIDS 		& \scriptsize NCI1  \\ %& Rank\\
\hline
\scriptsize $p$-random walk & 70.16 (7) \vspace{-0.1cm}& 64.14 (8) & 73.55(8)  & -  %& $(4)$  \vspace{-0.2cm}\\
\vspace{-0.1cm}\\
 &  {\tiny $\pm 0.20$}& {\tiny $\pm 1.35$} & {\tiny$\pm 0.49$ }& {\tiny$\pm -$} \\
 \scriptsize Graphket & 68.72 (8) \vspace{-0.1cm}& 67.36 (7) & 73.98(7)  & 70.70 (7) %& $(4)$  \vspace{-0.2cm}\\
\vspace{-0.1cm}\\
 &  {\tiny $\pm 0.09$}& {\tiny $\pm 0.96$} & {\tiny$\pm 0.65$ }& {\tiny$\pm -$} \\
\scriptsize FS 	&  83.32 (6)	&  76.36 (4) & 82.02 (5)  &  84.41 (3) \vspace{-0.1cm}\\ %& $(4)$  \vspace{-0.2cm}\\
 & {\tiny $\pm 0.37$} & {\tiny $\pm 1.48$} & {\tiny $\pm 0.4$} & {\tiny $\pm 0.49$} \\
\scriptsize NSPDK			& $83.60$ (2)	& {\bfseries 76.99}	(1)  	& {\bfseries 82.71}  (1) 	&$83.45$  (5) \vspace{-0.1cm}\\ 
& {\tiny $\pm 0.34$} &  {\tiny $\pm 1.15$}&   {\tiny $\pm 0.66$} & {\tiny $\pm 0.43$} \\
\scriptsize ODD$_{\text{ST}_h}$		& $83.34$  (5)	& $76.44$ 	 (3)  	& $81.51$  (6) 	& $82.10$  (6)\vspace{-0.1cm}\\ 
& {\tiny $\pm 0.31$}  &  {\tiny $\pm 0.62$} & {\tiny $\pm 0.74$} & {\tiny $\pm 0.42$}  \\
\scriptsize ODD$_{\text{ST}_h}^{\text{\tiny{TANH}}}$		& {$83.37$}  (4)	& $76.45$ (2)  	& $82.54$  (2) 	& $84.35$  (4)	 \vspace{-0.1cm}\\
& {\tiny $\pm 0.5$} & {\tiny $\pm 1.13$} & {\tiny $\pm 0.57$} & {\tiny $\pm 0.44$} \\
\scriptsize ODD$_{\text{ST}_+}$		&  {\bfseries 83.90}  (1)	& $76.30$  (6)  	& $82.06$  (4) 	& {\bfseries 84.97} (1)\vspace{-0.1cm}\\
& {\tiny $\pm 0.33$} & {\tiny $\pm 0.23$} & {\tiny $\pm 0.70$} & {\tiny $\pm 0.47$}  \\
\scriptsize ODD$_{\text{ST}_+}^{\text{\tiny{TANH}}}$		& {$83.39$}  (3)	& $76.31$ (5)  	& $82.54$ (2) 	& $84.69$  (2)	\vspace{-0.1cm}\\
& {\tiny $\pm 0.34$} & {\tiny $\pm 1.72$} & {\tiny $\pm 0.90$} & {\tiny $\pm 0.34$}\\
\hline
\end{tabular}
\end{center}
% \vspace{1ex}
%
\begin{center}
\begin{tabular}{|l|c|c|c|c|}
\hline
\scriptsize $Kernel$  	& \scriptsize GDD & \scriptsize NCI109 & \scriptsize  MSRC\_9 		& \scriptsize MSRC\_21 \\ %& Rank\\
\hline
\scriptsize $p$-random walk & - \vspace{-0.1cm}& - & 67.01(7)  & 18.88 (8) %& $(4)$  \vspace{-0.2cm}\\
\vspace{-0.1cm}\\
 &  {\tiny $\pm -$}& {\tiny $\pm -$} & {\tiny$\pm 2.22$ }& {\tiny$\pm 1.4$} \\
\scriptsize Graphlet & 74.92 (5) \vspace{-0.1cm}& 69.27 (7) & 60.83(8)  & 19.66 (7) %& $(4)$  \vspace{-0.2cm}\\
\vspace{-0.1cm}\\
 &  {\tiny $\pm 1.40$}& {\tiny $\pm -$} & {\tiny$\pm 2.0$ }& {\tiny$\pm 0.96$} \\
\scriptsize FS & 75.46 (2) \vspace{-0.1cm}& {\bfseries85.02} (1) & 89.26 (6)  & 89.87 (6) %& $(4)$  \vspace{-0.2cm}\\
\vspace{-0.1cm}\\
 &  {\tiny $\pm 0.98$}& {\tiny $\pm 0.44$} & {\tiny$\pm 0.82$ }& {\tiny$\pm 0.71$} \\
\scriptsize NSPDK		& $74.09$  (7) \vspace{-0.1cm}& $84.17$ (3) & $89.48$ (4) & $90.24$ (3) \vspace{-0.1cm}\\ %& ($3.2$) \vspace{-0.2cm}\\
& {\tiny $\pm 0.91$} & {\tiny $\pm 0.33$} & {\tiny$\pm 1.0$ }& {\tiny$\pm 0.49$}\\
\scriptsize ODD$_{\text{ST}_h}$	& $75.27$  (4) & $81.91$ (6) & $90.80$ (3)  & $89.92$ (5) \vspace{-0.1cm}\\ %& ($5$) \vspace{-0.2cm}\\
& {\tiny $\pm 0.68$} & {\tiny $\pm 0.42$} & {\tiny $\pm 1.10$} & {\tiny$\pm 0.73$} \\
\scriptsize ODD$_{\text{ST}_h}^{\text{\tiny{TANH}}}$	& {\bfseries 75.62}  (1) \vspace{-0.1cm}& 83.45 (4)  & \textbf{93.58} (1)  & \textbf{92.13 }(1) \vspace{-0.1cm}\\%& ($2.4$) \vspace{-0.2cm}\\
 &{\tiny $\pm 1.1$}& {\tiny $\pm 0.35$} & {\tiny$\pm 1.34$} & {\tiny$\pm 0.41$}\\
\scriptsize ODD$_{\text{ST}_+}$	& $75.33$  (3) \vspace{-0.1cm}& $83.08$ (5)  & 89.33 (5) & 89.94 (4) \vspace{-0.1cm}\\%& ($3$) \vspace{-0.2cm}\\
 & {\tiny $\pm 0.81$}& {\tiny $\pm 0.49$}& {\tiny$\pm 1.2$} & {\tiny$\pm 0.80$ } \\
\scriptsize ODD$_{\text{ST}_+}^{\text{\tiny{TANH}}}$		& $74.60$ (6) \vspace{-0.1cm}& 84.33 (2) & 92.96 (2)  & 91.73 (2) \vspace{-0.1cm}\\%& ($3.2$) \vspace{-0.2cm}\\
& {\tiny $\pm 0.68$} & {\tiny $\pm 0.27$} & {\tiny$\pm 1.57$} & {\tiny$\pm 0.69$}\\
\hline
\end{tabular}
\end{center}
 \caption{Average accuracy results $\pm$ standard deviation in nested 10-fold cross validation for the Fast Subtree, the Neighborhood Subgraph Pairwise Distance, the $ODD_{ST_h}$ and the $ODD_{\nuovotk}$ kernels obtained on CAS, CPDB, AIDS, NCI1, GDD, NCI109, MSRC\_9 and MSRC\_21  datasets. The rank of the kernel is reported between brackets. \label{tab:nestedkfoldresults}}
\end{table}
%
%
We compare the predictive abilities of the $ODD_{ST_{+}}$ kernel and the two proposed variants $ODD_{\text{ST}_h}^{\text{\tiny{TANH}}}$ and $ODD_{\text{ST}_+}^{\text{\tiny{TANH}}}$ to the original $ODD_{ST_h}$ kernel~\cite{Dasan2012}, the Fast Subtree Kernel (FS)~\cite{Shervashidze2009a} and the Neighborhood Subgraph Pairwise Distance Kernel (NSPDK)~\cite{Costa2010}. 
\textcolor{red}{Moreover, we compared to the $p$-random walk kernel, that is a kernel that compares radom walks wp to length $p$ in two graphs (special case of~\citep{Kashima2003} and~\citep{Mah'e2004} ) as representative for the family of kernels based on random walks, and to the \textit{graphlet} kernel~\citep{Shervashidze2009}.
Not that the complexity of the \textit{graphlet} kernel (when applied to labeled graphs) is exponential in the size $k$ of the graphlet. We restricted to a size that can be computed efficiently, i.e. $k=3$, as in \cite{Shervashidze2011}.
}
The experiments are performed using a \textit{nested} 10-fold cross validation: for each of the 10 folds another \textit{inner} 10-fold cross validation, in which we select the best parameters for that particular fold, is performed. %\cite{NIPS2009_0533}. %aggiungere solo se c'e' abbastanza spazio! 
All the experiments have been repeated $10$ times using different splits for the cross validation, and the average results (with standard deviation) are reported. 
For all the experiments, the values of the parameters of the $ODD_{ST_h}$ and $ODD_{\nuovotk}$~kernels have been restricted to: $\lambda=\{0.1, 0.2, \ldots, 2.0\}$, $h=\{1, 2, \ldots, 10\}$. 
For the variants using \textit{tanh}, the $\sigma$ parameter is optimized (instead of $\lambda$) in the set $\{10^5, 1, \frac{1}{3}, \frac{1}{5}, \frac{1}{10}, \frac{1}{15}\}$.
%The parameter selection procedure for the Fast Subtree Kernel replicates the one described in~\cite{Shervashidze2009a}, i.e. 
For the Fast Subtree kernel the only parameter $h=\{1, 2, \ldots, 10\}$ is optimized.
For the NSPDK, the parameters $h=\{1, 2, \ldots, 8\}$ and $d=\{1, 2, \ldots, 7\}$ are optimized. 
\textcolor{red}{Finally, for the $p$-random walk kernel we selected $p=\{1, 2, \ldots, 10\}$, and for the graphlet kernel we considered only the graphlets of size $3$, as mentioned above.}
Table~\ref{tab:nestedkfoldresults} reports the average accuracies and the rankings obtained by the different kernels on the considered datasets.
Let us now focus on the six chemical datasets.
The kernels $ODD_{\text{ST}_h}^{\text{\tiny{TANH}}}$,  $ODD_{\nuovotk}$, $ODD_{\text{ST}_+}^{\text{\tiny{TANH}}}$ together have best accuracy on three out of six datasets, and the second best accuracy on the other three. 
The variant employing the hyperbolic tangent is always useful for the ST kernel, making it the best performing kernel on GDD, and is able to boost the accuracy performance of $ODD_{\nuovotk}$ on AIDS, CPDB and NCI109 datasets. 
%bisogna ipotizzare quando va bene e quando no l'uso della tangente
The generally good results of the ODD kernels, with respect to FS and NSPDK, may be attributed to the fact that they have associated a large feature space, which makes them more adaptable to different tasks. 
\textcolor{red}{Note that the execution of $p$-random walk kernel did not complete in 4 days for NCI1, NCI109 and GDD datasets, so the results are missing.}
\textcolor{black}{Let us now focus on the image datasets (MSRC\_9 and MSRC\_21).
%Table~\ref{tab:image} reports the predictive performance of the considered kernels on MSRC9 and MSRC21 datasets. 
On these datasets, the baselines FS, NSPDK, $ODD_{\text{ST}_h}$ kernels and the proposed $ODD_{\nuovotk}$ kernel show very similar performances.
On these datasets, the introduction of the hyperbolic tangent weighting scheme is very beneficial. Both $ODD_{\text{ST}_h}^{\text{\tiny{TANH}}}$ and $ODD_{\text{ST}_+}^{\text{\tiny{TANH}}}$ performs better than all the baselines, with the former being the best performing kernel on both datasets. }\\
%
\textcolor{red}{The $p$-random walk kernel and the graphlet kernel show poor performances on these datasets. We argue that this is because they are the only ones among the considered kernels that that do not consider all the neighbors of a node as a feature.
}
% On the contrary, the Fast Subtree, while placing first on two datasets, has a lower ranking, i.e. second, fourth, fifth and sixth, on the other datasets. Its average ranking is $3.16$.  
% Incidentally, $3.16$ is exactly the average ranking of NSPDK kernel as well.
% Thus, $3.16$ the best average ranking of competing kernels is .
% Thus, $3.16$ is the average ranking to compare to our proposed kernels.
%  $K_{ODD-\nuovotk}$ has best accuracy in three out of six datasets. On the remaining datasets it places in second  position. 
% Notice that $ODD-{\nuovotk}$ almost always increases its accuracy with respect to $ODD-{ST_h}$ (the only exception being the CPDB dataset). The average rankings of $K_{ODD-\nuovotk}$ and $ODD-{ST_h} $are $1.5$ and $2.83$, respectively. 
%For each fold of the K-fold cross validation, we performed another \textit{inner} K-fold cross validation, in which we select the best parameters for that particular fold.
\begin{figure}[H]
	\centering
	\includegraphics[width=0.8\columnwidth]{plots2.0/times_journal_NCI1.pdf}
	\caption{Time needed to compute the kernel matrix, as a function of $h$, for the $K_{\text{ODD-ST}_{h}}$, $K_{\text{ODD-\nuovotk}_{h}}$, the NSPDK and the FS kernels on NCI1.\label{fig:tempinci1}}
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=0.8\columnwidth]{plots2.0/times_journal_CAS.pdf}
	\caption{Time needed to compute the kernel matrix, as a function of $h$, for the $K_{\text{ODD-ST}_{h}}$, $K_{\text{ODD-\nuovotk}_{h}}$, the NSPDK and the FS kernels on CAS dataset.\label{fig:tempicas}}
\end{figure}
\textcolor{black}{Figures~\ref{fig:tempinci1} and \ref{fig:tempicas} report the computational times required by the ODD$_{ST_h}$, ODD$_{\nuovotk}$, NSPDK and the FS kernels  as a function of the parameter $h$ determining the size of the considered substructures on the NCI1 and CAS datasets, respectively.}\\
All the experiments are performed on a PC with two Quad-Core AMD Opteron(tm) 2378 Processors and 64GB of RAM. 
Given that the available implementations of the kernels are in different programming languages (FS, \textcolor{red}{$p$-random walk and graphlet} in Matlab and the others in C++), the times for the FS, \textcolor{red}{the $p$-random walk and the graphlet kernels} are reported just for a qualitative comparison. \\
The time needed to compute the kernel matrix for the ODD$_\nuovotk$ kernel increases roughly linearly with respect to the parameter $h$ for both datasets. 
As expected the constant factors are higher than the ones of the ODD$_{ST_h}$, but the ODD$_\nuovotk$ is faster than NSPDK.
\textcolor{black}{Note that we do not report the computational times for ODD$_{ST_h}^{\text{\tiny{TANH}}}$ and ODD$_\nuovotk^{\text{\tiny{TANH}}}$ since their computational requirements are basically the same as the corresponding base kernel, since only the weighing function is different and it can be computed in constant time.\\}
\begin{table}[t]
%   \footnotesize
  \centering
 \begin{tabular}{|l|c|c|c|c|}
  \hline
  Kernel	& CAS 			&  AIDS 		& NCI1			& GDD	\\
  \hline
  \textcolor{red}{Graphlet}		& $58$ 			&  $54$  		& $133$  		& $1715$	 \\
  \textcolor{red}{\scriptsize $p$-random walk} & $2d$ 			&  $2d$  		& $-$  		& $-$	 \\
  		& \scriptsize{(h=$7$)}	& \scriptsize{(h=$8$)}	& \scriptsize{(h=$-$)}	& \scriptsize{(h=$-$)} \\
  FS		& $77$ 			&  $30$  		& $246$  		& $405$	 \\
		& \scriptsize{(h=$3$)}	& \scriptsize{(h=$9$)}	& \scriptsize{(h=$8$)}	& \scriptsize{(h=$1$)} \\
  NSPDK		& $24$ 			&  $217$ 		&$192$ 	 		& $395$	\\
		& \scriptsize{(h=$2$, d=$6$)}& \scriptsize{(h=$8$,d=$6$)} & \scriptsize{(h=$5$,d=$4$)} & \scriptsize{(h=$2$,d=$6$)} \\
  ODD$_{ST_h}$ 	& $18$ 			&  $56$  		& $44$  		& $29$  \\
		& \scriptsize{(h=$3$)}	& \scriptsize{(h=$7$)}	& \scriptsize{(h=$4$)}	& \scriptsize{(h=$1$)} \\
		
		 \textcolor{red}{ ODD$_{ST_h}^{\text{\tiny{TANH}}}$ }	& $47$ 			&  $51$  		& $110$  		& $246$  \\
		& \scriptsize{(h=$5$)}	& \scriptsize{(h=$6$)}	& \scriptsize{(h=$6$)}	& \scriptsize{(h=$2$)} \\
  ODD$_{\nuovotk}$	& $32$ 			&  $111$ 		& $205$ 		& $199$ \\
		& \scriptsize{(h=$4$)}	& \scriptsize{(h=$8$)}	& \scriptsize{(h=$1$)}	& \scriptsize{(h=$1$)} \\
		\textcolor{red}{ODD$_{\nuovotk}^{\text{\tiny{TANH}}}$ }	& $179$ 			&  $61$  		& $165$  		& $541$  \\
		& \scriptsize{(h=$8$)}	& \scriptsize{(h=$5$)}	& \scriptsize{(h=$4$)}	& \scriptsize{(h=$2$)} \\
  \hline
 \end{tabular}
    \caption{Average seconds required for computing the kernel matrix on CAS, AIDS, NCI1 and GDD datasets with the optimal kernel parameters (reported between brackets). $d$ means days. \label{tab:tempi}}
\end{table}
Moreover, in Table~\ref{tab:tempi} we report the average computational time for a single fold with the optimal parameters on the four largest datasets: CAS, AIDS, NCI1, GDD. The parameters influencing the speed of the kernel are reported between brackets. \textcolor{red}{In this case, we reported the times corresponding to all the considered kernels.}
 Even when comparing the executions related to the optimal parameters, ODD$_\nuovotk$ is faster or comparable to NSPDK \textcolor{red}{and ODD$_{ST_h}$ is faster or comparable to FS}. 
% \textcolor{black}{Note that we do not report the computational times for ODD$_{ST_h}^{\text{\tiny{TANH}}}$ and ODD$_\nuovotk^{\text{\tiny{TANH}}}$ since their computational requirements are basically the same as the corresponding base kernel, since only the weighing function is different and it can be computed in constant time.\\}


% Notice that, as $h$ increases, the time required for computing the kernel matrix seems to increase almost linearly for FS and $ST_h$. 
% This can be explained with the fact that smaller graphs do not allow too deep visits, so the increase in complexity due to the increase of the depth visit is compensated by the smaller number of graphs where visits of that depth can be actually performed. 
% \begin{figure}[ht]
%   \centering
%   \begin{minipage}{.495\textwidth}
%   	\includegraphics[width=1\columnwidth]{figs/times_journal_NCI1_noylabel.pdf}
%   \end{minipage}
%   \begin{minipage}{.495\textwidth}
% 	\includegraphics[width=1\columnwidth]{figs/times_journal_CAS_noylabel.pdf}
%   \end{minipage}
% \end{figure}
%
%
\subsection{Experiments on full NCI datasets}
%
\begin{table}[t]
\centering
\textcolor{red}{
\begin{tabular}{|l|c|c|}
\hline
\scriptsize $Kernel$  	& \scriptsize NCI123 & \scriptsize NCI\_AIDS \\
\hline
\scriptsize Graphlet & 54.93 (7) \vspace{-0.1cm}& 67.74 (7)\\
 &  {\tiny $\pm 0.24$}& {\tiny $\pm 0.15$} \\
\scriptsize FS & $61.08$ (6) \vspace{-0.1cm}& 83.73 (5) \\
 &  {\tiny $\pm 0.34$}& {\tiny $\pm 0.17$} \\
\scriptsize NSPDK		& $62.45$  (3) \vspace{-0.1cm}& {\bfseries$83.80$} (3)\\
& {\tiny $\pm 0.39$} & {\tiny $\pm 0.23$} \\
\scriptsize ODD$_{\text{ST}_h}$	& $62.11$  (4) & $83.77$ (4) \\
& {\tiny $\pm 0.30$} & {\tiny $\pm 0.22$}  \\
\scriptsize ODD$_{\text{ST}_h}^{\text{\tiny{TANH}}}$	& $62.76$  (2) \vspace{-0.1cm}& 85.56 (2) \\
 &{\tiny $\pm 0.21$}& {\tiny $\pm 0.23$} \\
\scriptsize ODD$_{\text{ST}_+}$	& $61.70$  (5) \vspace{-0.1cm}& $83.36$ (6) \\
 & {\tiny $\pm 0.36$}& {\tiny $\pm 0.30$} \\
\scriptsize ODD$_{\text{ST}_+}^{\text{\tiny{TANH}}}$		& {\bfseries 63.20} (1) \vspace{-0.1cm}& {\bfseries85.64} (1)\\
& {\tiny $\pm 0.29$} & {\tiny $\pm -0.15$} \\
\hline
\end{tabular}
 \caption{Average AUC results $\pm$ standard deviation in nested 10-fold cross validation for the Graphlet, the Fast Subtree, the Neighborhood Subgraph Pairwise Distance, the $ODD_{ST_h}$, the $ODD_{\nuovotk}$
, ODD$_{\text{ST}_h}^{\text{\tiny{TANH}}}$ and $ODD_{\text{ST}_+}^{\text{\tiny{TANH}}}$	
  kernels obtained on NCI123 and NCI\_AIDS  datasets. The rank of the kernel is reported between brackets. \label{tab:nestedkfoldresultsBig}}
  }
\end{table}
%
\textcolor{red}{In this set of experiments, we analyze how the proposed kernels and the competitors scale up with bigger datasets. We considered two datasets, NCI123 and NCI\_AIDS, each one with more than $40,000$ examples (see Table~\ref{tab:datasets}).
These datasets are unbalanced, so for this set of experiments we adopted the Area under the  receiver operating characteristic curve (AUROC or AUC) as performance measure, since it is suited for unbalanced datasets.
The experimental setup in this case is different w.r.t. the one presented in Section~\ref{expsold}. Indeed, when the number of examples is big, computing the Gram matrix is unfeasible.
In this case, for each considered kernel configuration, we computed the explicit features associated to each example. With this explicit feature representation, it is possible to train a linear SVM\footnote{In our implementation we adopted \textit{Liblinear~\citep{Fan2008}}.}. Note that the computed solution is equivalent to the one that can be found by a C-SVM applied to the kernel matrix generated by the graph kernel. However, in this way it is possible to handle very big datasets in a reasonable amount of time.}

\textcolor{red}{In Table~\ref{tab:nestedkfoldresultsBig} the AUC results on the two considered datasets of the kernels for which it is possible to generate the explicit feature space representation of input examples are reported.
Figure~\ref{fig:tempinci123} reports the computational time required to perform the learning procedure for a fixed kernel. This procedure comprehends the feature generation step, and the training of the linear SVM model. We decided to report the overall times here because the rum-times of linear SVM depends on the characteristics of the kernel, and thus comparing only the feature generation part would be not fair.\\
On the considered datasets, the perofrmances of the different kernels are comparable. However, ODD$_{\text{ST}_h}^{\text{\tiny{TANH}}}$ and ODD$_{\nuovotk}^{\text{\tiny{TANH}}}$ show the highest performance on both datasets.
}
\begin{figure}[ht]
	\centering
	\textcolor{red}{
	\includegraphics[width=0.85\columnwidth]{plots2.0/times_journal_NCI123.pdf}
	\caption{Time needed to perform all the training procedure, as a function of $h$, for all the considered kernels on NCI123 dataset.\label{fig:tempinci123}}
	}
\end{figure}
\begin{table}[t]
\centering
\textcolor{red}{
\begin{tabular}{|l|c|c|}
\hline
\scriptsize $Kernel$  	& \scriptsize NCI123 & \scriptsize NCI\_AIDS \\
\hline
\scriptsize Graphlet & 698 \vspace{-0.1cm}& 1772\\
 &  {\tiny (C=0.01)}& {\tiny (C=0.001)} \\
\scriptsize FS &  261\vspace{-0.1cm}& 237 \\
 &  {\tiny (h=4,C=0.1)}& {\tiny (h=3,C=0.1)} \\
\scriptsize NSPDK \vspace{-0.1cm}& 246 &- \\
& {\tiny (h=2,d=5,C=1)} & {\tiny -} \\
\scriptsize ODD$_{\text{ST}_h}$	& 850 & $-$ (6) \\
& {\tiny (h=7,C=100)} & {\tiny $\pm 0.42$}  \\
\scriptsize ODD$_{\text{ST}_h}^{\text{\tiny{TANH}}}$	& $62.76$  (2) \vspace{-0.1cm}& 85.56 (4) \\
 &{\tiny $\pm 0.21$}& {\tiny $\pm 0.23$} \\
\scriptsize ODD$_{\text{ST}_+}$	& $61.70$  (5) \vspace{-0.1cm}& $83.09$ (5) \\
 & {\tiny $\pm 0.36$}& {\tiny $\pm 0.40$} \\
\scriptsize ODD$_{\text{ST}_+}^{\text{\tiny{TANH}}}$		& {\bfseries 63.20} (1) \vspace{-0.1cm}& - (2)\\
& {\tiny $\pm 0.29$} & {\tiny $\pm -$} \\
\hline
\end{tabular}
 \caption{Time needed to perform all the training procedure with the optimal parameter configuration (reported between brackets) for all the considered kernels on NCI123 and NCI\_AIDS datasets.\label{fig:tempinci123} \label{tab:TimesBig}}
  }
\end{table}

% \begin{table}
%   \scriptsize
%   \centering
%    \caption{Average seconds required for computing the kernel matrix on CAS, AIDS, NCI1 and GDD datasets with the optimal kernel parameters (reported between brackets). \label{tab:tempi}}
%  \begin{tabular}{|l|l|l|l|l|}
%   \hline
%   Kernel	& CAS 			&  AIDS 		& NCI1			& GDD	\\
%   \hline
%   FS		& $77$ \scriptsize{(h=$3$)}		&  $30$ \scriptsize{(h=$9$)} 	& $246$ \scriptsize{(h=$8$)} 	& $405$	\scriptsize{(h=$1$)} \\
%   NSPDK		& $24$ \scriptsize{(h=$2$, d=$6$)}	&  $217$ \scriptsize{(h=$8$,d=$6$)}	&$192$ 	\scriptsize{(h=$5$,d=$4$)} & $395$	\scriptsize{(h=$2$,d=$6$)}\\
%   ODD-ST$_h$ 	& $18$ \scriptsize{(h=$3$)}	&  $56$  \scriptsize{(h=$7$)}	& $44$ \scriptsize{(h=$4$)} & $29$ \scriptsize{(h=$1$)} \\
%   ODD-\nuovotk	& $32$ \scriptsize{(h=$4$)}	&  $111$ \scriptsize{(h=$8$)}	&$205$ 	\scriptsize{(h=$1$)}		& $199$ \scriptsize{(h=$1$)}\\
%   \hline
%  \end{tabular}
% \end{table}


==> fig.dagconstruction.tex <==

\begin{figure}
\centering
\begin{tikzpicture}[auto,thick,scale=.5]
   \tikzstyle{graph}=[scale=1.0,minimum size=12pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
		\node (s) [graph] {s}   
					child {
            node (b) [graph] {b}
        	};
         \node (e) [graph] at (0:2){e}   
         		child { node (d) [graph] {d}};		
    ;    	
    \draw
    (s) to (e)
    (b) to (d)
    (b) to (e)
    ;
  \small
	 \draw [red,->,line width=5pt] (4,-0.8)--(6,-0.8);
   \tikzstyle{node}=[minimum size=12pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
        \node [node,xshift=4.1cm, yshift=1.3cm] {\textbf{s}} [->] %[->, ultra thick]
                child {
                    node [node] {\textbf{e}}[] 
                    child {node (d2)[node, xshift=0.35cm]{\textbf{d}}[]}
                }
                child {
                    node (b2) [node]{\textbf{b}}[]
                }
				;
         \draw [->]
         (b2) to (d2)
        ;
        \node (e) [node,xshift=6.5cm,yshift=1.3cm] {e}
        		child[->] {
            			node (s) [node] {s}
            			}
						child[->]{
									node (b) [node] {b}
									}
	   				child[->] {
            			node (d) [node] {d}
            			}
        ;
        \node [node,xshift=4.1cm,yshift=-1.0cm] {b}
        		child[->] {
            			node [node] {s}
            			}
						child[->]{
									node [node] {e}
									}
	   				child[->] {
            			node [node] {d}
            			}
        ;    
        \node [node,xshift=6.5cm, yshift=-0.2cm] {\textbf{d}} [->] 
                child {
                    node [node] {\textbf{b}}[] 
                    child {node (d2)[node, xshift=0.35cm]{\textbf{s}}[]}
                }
                child {
                    node (e2) [node]{\textbf{e}}[]
                }
				;
         \draw [->]
         (e2) to (d2)
        ;    
        %\node [black,yshift=-0.4cm,xshift=7.0cm] {b)};
\end{tikzpicture}
%\begin{tikzpicture}[scale=0.7]
%   	\tikzstyle{every node}=[scale=0.7,minimum size=18pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
%    \node (s) [xshift=1cm, yshift=0cm] {s}
%     child[->] {
%            node (b) {b}}
%	child[->]{
%	node (e) {e}
%		child[->] { node (d) {d}}
%        };
%        
%    \draw [->]
%    (b) to (d)
%    ;
%%    \node (e) {e}
%%        child[->] {
%%            node (s) {s}
%%            	}
%%	child[->]{
%%	node (b) {b}}
%%	   child[->] {
%%            node (d) {d}
%%            	}
%%        ;       
%%    \node (e) [xshift=0cm] {b}[->]
%%        child {
%%            node (s) {s}[]
%%            	}
%%	child[->]{
%%	node (b) {e}}
%%	   child[->] {
%%            node (d) {d}
%%            	}
%%        ;        
%%    \node (s) [xshift=0cm] {d}
%%     child[->] {
%%            node (b) {e}}
%%	child[->]{
%%	node (e) {b}
%%		child[->] { node (d) {s}}
%%        };
%%        
%%    \draw [->]
%%    (b) to (d)
%%    ;
%\end{tikzpicture}
\caption{Example of decomposition of a graph (left) into its $4$ DDs (right). \label{fig:dagconstruction}}
\end{figure}


==> newweighting_vecchio.tex <==
\subsection{A Novel Feature Weighting Scheme} \label{sec:tanh}
\textcolor{red}{
As detailed in Section~\ref{sec:dagkernels}, the DAG kernels we considered are derived from tree kernels that count matching substructures between two input trees.
Let us focus on the ST kernel, that has a non-zero feature for each proper subtree of the considered DAG.
It is worth to pint out that if a tree appears in the feature space representation of a DAG, then all its proper subtrees will appear as well.
Let us consider the case where no feature weighting scheme is applied, i.e. each feature contributes in the same amount to the kernel value.
From a practical point of view, the value of the resulting kernel when applied to two copies of the same tree can be extremely large while the value of the kernel between two different trees is typically much smaller. This property negatively impact the model trained by the SVM, since the classification of an example would be dominated by the contribution of the most similar support example, with a behavior similar to a nearest neighbour rule.
For this reason,\cite{Collins2001} proposed to downweight the contribution of large tree fragments to the kernel.
This scheme has been implemented in our proposed Alg.\ref{fig:nuovokernelfeaturespace}.
Let $|f|$ be the number of nodes in the subtree encoded by a feature $f$. 
%, that looking at Alg.~\ref{alg:nuovokernelfeatures} can be $\subtreerootedat{\node}$ (line 3) or $t$ (line 7).
Lines 4 and 9 of Alg.\ref{fig:nuovokernelfeaturespace} show that the weight of each feature is \textcolor{red}{$w(f)=freq_G(f) \cdot \lambda^\frac{|f|}{2}$, where $freq_G(f)$ is the frequency of the feature in $G$}. Therefore the contribution to the kernel of two matching features (computed via dot product) is $freq_{G_1}(f)\cdot freq_{G_2}(f) \cdot \lambda^{|f|}$. 

In our scenario, the situation is different: big features are no longer the ones overcontributing to the kernel value, but the small ones are taken into account too much, because them can appear in multiple ODD$_G^\node$.
If a graph has several nodes with the same label, the corresponding single-node tree-feature may overcontribute to the final kernel value. 
As an example, in the CAS dataset (see Section~\ref{sec:exps}) approximately 75\% of the nodes correspond to Carbon atoms. 
Given our preprocessing, aleady with $h=1$ the percentage of such nodes in the multiset of DAGs is amplified: we will have $|V|* \rho \0.75$ of such features, a factor $\rho$ more than the real ratio of such nodes in the graph. 
By using a $\lambda>1$ it is possible to reduce the contribution of small structures. However, with this scheme we still underweight the contribution of the less frequent,  possibly interesting, small features.

More in general, there is no reason why other schemes cannot be more suited for a particular task.
\textcolor{red}{As a first step in this direction,} we propose to mitigate the contribution of \textcolor{red}{otherwise} overweighted features 
with a different definition of  
%by replacing  $\lambda^{|f|}$ with 
 $w(f)=\tanh(|f|*freq(f)*\sigma)$, 
}

}
\textcolor{blue}{
Let us start this section with a remark. If two graphs (trees) share a common subgraph (subtree) $S$, then they share also all the possible sub-graphs (sub-trees) of $S$. This is not a surprise, since the graph-subgraph relationship is transitive.
As detailed in Section~\ref{sec:dagkernels}, the DAG kernels we considered are derived from tree kernels that count matching substructures between two input trees.
The consequence of our remark is that if a tree is present in the feature space representation of a DAG, so are all the subtrees that are included in the considered tree (the type of the subtrees being defined by the specific DAG kernel).
Let us consider the case where no feature weighting scheme is applied, i.e. each feature contributes in the same amount to the kernel value.
From a practical point of view, the value of the resulting kernel when applied to two copies of the same tree can be extremely large while the value of the kernel between two different trees is typically much smaller. This property negatively impact the model trained by the SVM, since the classification of an example would be dominated by the contribution of the most similar support example, with a behavior similar to a nearest neighbour rule.
To solve this problem \cite{Collins2001} proposed to downweight the contribution of large tree fragments to the kernel, using a rationale that follows from the remark at the beginning of this section.
%
The same rule has been implemented in our proposed Alg.\ref{fig:nuovokernelfeaturespace}, where the (down)weighting function for a feature $f$ is defined as follows.}
Let $|f|$ be the number of nodes in the subtree encoded by a feature $f$. 
%, that looking at Alg.~\ref{alg:nuovokernelfeatures} can be $\subtreerootedat{\node}$ (line 3) or $t$ (line 7).
Lines 4 and 9 of Alg.\ref{fig:nuovokernelfeaturespace} show that the weight of each feature is \textcolor{red}{$w(f)=freq_G(f) \cdot \lambda^\frac{|f|}{2}$, where $freq_G(f)$ is the frequency of the feature in $G$}. Therefore the contribution to the kernel of two matching features (computed via dot product) is \textcolor{red}{$freq_{G_1}(f)\cdot freq_{G_2}(f) \cdot \lambda^{|f|}$. } %, where $freq_1(f)$ and $freq_2(f)$ are the frequencies of $f$ in $G_1$ and $G_2$, respectively.} 
% The idea is to downweight the contribution of large trees since, in order for them to match, also all of their subtrees have to match
%
% This is the usual downweighting scheme used in tree kernels to avoid that artifi overweighting the contribution of a large feature. 
% % % The parameter $\lambda$ implements a downweighting scheme to avoid of some features (large subtrees in this case, see \cite{Collins2002} for details) to be overweighted and to provide an artificially-inflated contribution to the kernel value. 
% If we consider the preprocessing described in Section~\ref{sec:background}, it turns out that a node of the graph may appear in many ODD$_G^\node$ and thus possibly overcontributing to the final kernel value

\textcolor{red}{However, there is no reason why this downweighting function should be the best one to implement.
For example, if we consider the preprocessing described in Section~\ref{sec:background}, it turns out that a node of the graph may appear in many ODD$_G^\node$. If a graph has several nodes with the same label, the corresponding single-node tree-feature (that is one of the features with higher weight) may overcontribute to the final kernel value. 
% % % % The situation is worse if everal nodes in the original graph share the same label, generating the same single-node feature.
%, i.e. two graphs are considered very similar because of these features, even if they should not be according to the target concept. In this case we speak about artificially high kernel values. 
As an example, in the CAS dataset (see Section~\ref{sec:exps}) approximately 75\% of the nodes correspond to Carbon atoms. 
Given our preprocessing, the percentage of such nodes in the multiset of DAGs is amplified (for $h>0$) and thus their contribution to the kernel evalutation will be preponderant. 
By using a $\lambda>1$ it is possible to reduce the contribution of small structures. However, with this scheme we still underweight the contribution of the less frequent,  possibly interesting, small features. }
\textcolor{red}{More in general, there is no reason why other schemes cannot be more suited for a particular task.}
\textcolor{red}{As a first step in this direction,} we propose to mitigate the contribution of \textcolor{red}{otherwise} overweighted features 
with a different definition of  
%by replacing  $\lambda^{|f|}$ with 
 $w(f)=\tanh(|f|*freq(f)*\sigma)$, 
}
% 
% In the kernel with $h=0$, the 75\% of the weight is given to the feature encoding the subtree with a single node labelled \textit{C}. With $h\geq1$, the weight is even higher. With the standard downweighting scheme it is possible to partially mitigate this situation using $\lambda>1$ values, thus assigning a higher weight to bigger, and less frequent features. However, with this scheme we underweight the contribution of the less frequent, but possibly interesting, small features, for example the feature encoding the single \textit{Nitrogen} atom.}
% 
% We propose to mitigate the preponderance of small features by replacing $\lambda^{|f|}$ with $\tanh(|f|*freq(f)*\sigma)$, 
%In order to reduce such an effect , we propose to replace the weight $\lambda^{|f|}$ with $\tanh(|f|*freq(f)*\sigma)$, 
%Following the same principle we observe that, by construction, a node of the graph may appear in multiple tree visits. 
%In order to control the contribution of the features related to such nodes, we propose to replace the weight $\lambda^{|f|}$ with $\tanh(|f|*freq(f)*\sigma)$,  
% 
% We propose a different approach, that is inspired by the sigmoidal nonlinear function used in the neurons of artificial neural networks [],
% i.e. the hyperbolic tangent \textit{tanh}.  
% The adoption of a sigmoidal function instead of the usual decay factor is justified by the fact that usually with structured data, 
% the features associated to the leaves, and in general to small features, are little informative. 
% This observation has to be considered together with another consideration, that huge features are usually not very frequent and lead to 
% overtraining (this is the reason why downweighting has been introduced in the first place). 
% Our proposal is to substitute the weighting $\lambda^{|f|}$ with a $\tanh(|f|*freq(f)*\sigma)$, 
where 
%$freq(f)$ is the frequency of the feature in the particular example and 
$\sigma$ is a parameter determining the smoothness of the sigmoid function. %We will show in Section~\ref{sec:exps} that sometimes this leads to slightly improved predictive performance.
\textcolor{red}{Note that the original weighting scheme depends nonlinearly (exponentially) on the size of the feature $|f|$ and linearly on its frequency.
The novel scheme we are proposing, on the other hand, depends nonlinearly on both $|f|$ and $freq(f)$.
%
In this way, the contribution of each feature is smoothly and non-linearly normalized in the interval $[0,1]$.}\\
\textcolor{red}{Note that the hyperbolic tangent function is almost linear around the zero, and asymptotically tends to one. This means that the contribution of frequent features is truncated, while the less frequent features are still discriminated since they fall in the linear part of the function. 
The gradient of the weight function is determined by the $\sigma$ paramter. }
% \textcolor{red}{TODO Nonlinearità nella frequenza delle features invece che nella dimensione.
% tanh è lineare intorno allo zero, quindi le feature con frequenza (pesata per la sigma) bassa continuano ad essere discriminate, ma viene troncato il contributo delle features molto frequenti che invece rischia di offuscare le altre.
%}\\
The new weighting scheme is applied to the ST kernel, obtaining a variant of the kernel proposed in \cite{Dasan2012}, and to the ST+ kernel first proposed in this paper. 


% % % % % % % % % % % % % \subsection{A Novel Feature Weighting Scheme} \label{sec:tanh}
% % % % % % % % % % % % % \textcolor{red}{
% % % % % % % % % % % % % When dealing with structured features, and more specifically with trees as considered in this paper, if a tree is present in the feature space representation of a graph, so are all the proper subtrees
% % % % % % % % % % % % % of the considered tree. This is a well-known property of kernels with structured features, and it introduces a strong dependency among features.
% % % % % % % % % % % % % For both theoretical and computational
% % % % % % % % % % % % % reasons, usually the features are downweighted according
% % % % % % % % % % % % % to their size. For historical reasons, the (down)weighting
% % % % % % % % % % % % % function for a feature f is defined as follows.}
% % % % % % % % % % % % % Let $|f|$ be the number of nodes in the subtree encoded by a feature $f$. 
% % % % % % % % % % % % % %, that looking at Alg.~\ref{alg:nuovokernelfeatures} can be $\subtreerootedat{\node}$ (line 3) or $t$ (line 7).
% % % % % % % % % % % % % Lines 3 and 8 of Alg.\ref{fig:nuovokernelfeaturespace} show that the weight of each feature is \textcolor{red}{$freq_G(f) \cdot \lambda^\frac{|f|}{2}$, where $freq_G(f)$ is the frequency of the feature in $G$}. Therefore the contribution to the kernel of two matching features (computed via dot product) is \textcolor{red}{$w(f)=freq_{G_1}(f)\cdot freq_{G_2}(f) \cdot \lambda^{|f|}$. } %, where $freq_1(f)$ and $freq_2(f)$ are the frequencies of $f$ in $G_1$ and $G_2$, respectively.} 
% % % % % % % % % % % % % % The idea is to downweight the contribution of large trees since, in order for them to match, also all of their subtrees have to match
% % % % % % % % % % % % % %
% % % % % % % % % % % % % % This is the usual downweighting scheme used in tree kernels to avoid that artifi overweighting the contribution of a large feature. 
% % % % % % % % % % % % % The parameter $\lambda$ implements a downweighting scheme to avoid of some features (large subtrees in this case, see \cite{Collins2002} for details) to be overweighted and to provide an artificially-inflated contribution to the kernel value. 
% % % % % % % % % % % % % % If we consider the preprocessing described in Section~\ref{sec:background}, it turns out that a node of the graph may appear in many ODD$_G^\node$ and thus possibly overcontributing to the final kernel value
% % % % % % % % % % % % %
% % % % % % % % % % % % % \textcolor{red}{The introduction of this downweighting function is a bias, and have some drawbacks.
% % % % % % % % % % % % %  If we consider the preprocessing described in Section~\ref{sec:background}, it turns out that a node of the graph may appear in many ODD$_G^\node$. If a graph has several nodes with the same label, the corresponding single-node tree-feature may overcontribute to the final kernel value. 
% % % % % % % % % % % % % %, i.e. two graphs are considered very similar because of these features, even if they should not be according to the target concept. In this case we speak about artificially high kernel values. 
% % % % % % % % % % % % % As an example, in the CAS dataset approximately 75\% of the nodes correspond to Carbon atoms. 
% % % % % % % % % % % % % Given our preprocessing, the percentage of such nodes in the multiset of DAGs is amplified and thus their contribution to the kernel evalutation will be preponderant. 
% % % % % % % % % % % % % By using a $\lambda>1$ is it possible to amplify the contribution of large structures. However, with this scheme we still underweight the contribution of the less frequent,  possibly interesting, small features. 
% % % % % % % % % % % % % \textcolor{red}{More in general, there is no reason why other schemes cannot be more suited for a particular task.}
% % % % % % % % % % % % % \textcolor{red}{As a first step in this direction,} we propose to mitigate the contribution of overweighted features 
% % % % % % % % % % % % % with a different definition of  
% % % % % % % % % % % % % %by replacing  $\lambda^{|f|}$ with 
% % % % % % % % % % % % %  $w(f)=\tanh(|f|*freq(f)*\sigma)$, 
% % % % % % % % % % % % % }
% % % % % % % % % % % % % % 
% % % % % % % % % % % % % % In the kernel with $h=0$, the 75\% of the weight is given to the feature encoding the subtree with a single node labelled \textit{C}. With $h\geq1$, the weight is even higher. With the standard downweighting scheme it is possible to partially mitigate this situation using $\lambda>1$ values, thus assigning a higher weight to bigger, and less frequent features. However, with this scheme we underweight the contribution of the less frequent, but possibly interesting, small features, for example the feature encoding the single \textit{Nitrogen} atom.}
% % % % % % % % % % % % % % 
% % % % % % % % % % % % % % We propose to mitigate the preponderance of small features by replacing $\lambda^{|f|}$ with $\tanh(|f|*freq(f)*\sigma)$, 
% % % % % % % % % % % % % %In order to reduce such an effect , we propose to replace the weight $\lambda^{|f|}$ with $\tanh(|f|*freq(f)*\sigma)$, 
% % % % % % % % % % % % % %Following the same principle we observe that, by construction, a node of the graph may appear in multiple tree visits. 
% % % % % % % % % % % % % %In order to control the contribution of the features related to such nodes, we propose to replace the weight $\lambda^{|f|}$ with $\tanh(|f|*freq(f)*\sigma)$,  
% % % % % % % % % % % % % % 
% % % % % % % % % % % % % % We propose a different approach, that is inspired by the sigmoidal nonlinear function used in the neurons of artificial neural networks [],
% % % % % % % % % % % % % % i.e. the hyperbolic tangent \textit{tanh}.  
% % % % % % % % % % % % % % The adoption of a sigmoidal function instead of the usual decay factor is justified by the fact that usually with structured data, 
% % % % % % % % % % % % % % the features associated to the leaves, and in general to small features, are little informative. 
% % % % % % % % % % % % % % This observation has to be considered together with another consideration, that huge features are usually not very frequent and lead to 
% % % % % % % % % % % % % % overtraining (this is the reason why downweighting has been introduced in the first place). 
% % % % % % % % % % % % % % Our proposal is to substitute the weighting $\lambda^{|f|}$ with a $\tanh(|f|*freq(f)*\sigma)$, 
% % % % % % % % % % % % % where 
% % % % % % % % % % % % % %$freq(f)$ is the frequency of the feature in the particular example and 
% % % % % % % % % % % % % $\sigma$ is a parameter determining the smoothness of the sigmoid function. %We will show in Section~\ref{sec:exps} that sometimes this leads to slightly improved predictive performance.
% % % % % % % % % % % % % \textcolor{red}{In this way, the contribution of each feature is smoothly and non-linearly normalized in the interval $[0,1]$.}
% % % % % % % % % % % % % The new weighting scheme is applied to the ST kernel, obtaining a variant of the kernel proposed in \cite{Dasan2012}, and to the ST+ kernel first proposed in this paper. 
% % % % % % % % % % % % %


==> noveltreekernel.tex <==

\subsection{A graph kernel based on a novel tree kernel} \label{sec:noveltk}

In Section~\ref{sec:hash} a graph kernel based on the ST kernel for trees has been defined. It has $|V_G|\log |V_G|$ complexity but, in practice,  it is competitive, in terms of speed, with the fastest graph kernels (see Section~\ref{sec:exps}). However, being based on the ST kernel, the associated feature space might not be expressive for certain tasks. 

The kernel we introduce in this section enlarges the feature space of the kernel in Section~\ref{sec:hash}, with a modest increase in computational burden. 

The associated tree kernel, which is a novel contribution in itself, is referred to as \nuovotk. 
The set of features related to the \nuovotk~kernel is a superset of the features of ST and a subset of the features of PT. 
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[-,thick,scale=0.485, sibling distance=4.0cm]
 	          \node []{$\node$}
		   child {node (lft) []{$\subtreelimitedrootedat{ch_{\node}[1]}{l}$}}
		   %child {node[xshift=0.1cm]{$\ldots$}}
		   child {node[xshift=0.3cm]{$\subtreelimitedrootedat{ch_{\node}[j-1]}{l}$}}
		   child {node[]{$\subtreerootedat{ch_{\node}[j]}$}}
		   child {node[xshift=-0.3cm]{$\subtreelimitedrootedat{ch_{\node}[j+1]}{l}$}}
		   %child {node[]{$\ldots$}}
		   child {node (rgt)[]{$\subtreelimitedrootedat{ch_{\node}[\rho(\node)]}{l}$}}	
		  ;
		  \node[right=0.3cm of lft, yshift=-0.15cm]{$\dots$};
		  \node[left=0.1cm of rgt, yshift=-0.15cm]{$\dots$};
  \end{tikzpicture} 
  \caption{A feature for the tree kernel \nuovotk. Given the node $\node$ and the index $j$, the feature is composed by $\node$, the proper subtree rooted at the $j$-th child and the subtrees resulting from a limited visit of $l$ levels for the other children.\label{fig:nuovotkfeature}}
\end{figure}
Figure~\ref{fig:nuovotkfeature} describes a generic novel feature introduced by \nuovotk. Notice that it depends on $\node\in T$, the index of a child $j$ and a limit $l$ on the depth of the visits. While for the ST kernel there is one feature for each $\node\in T$, \nuovotk~ associates at most $\rho(\node)h$ features for any $\node\in T$. 
Figure\ref{fig:nuovokernelfeaturespace} depicts a partial feature space representation of a tree according to \nuovotk. 
% We will refer to 
% , while Figure\ref{fig:nuovokernelfeaturespace} depicts a partial feature space representation of a tree. 
% Alg.~\ref{alg:nuovokernelfeatures} describes the procedure for building the feature space representation for a tree according to the kernel \nuovotk. In order to explain the algorithm we refer to Figure\ref{fig:nuovokernelfeaturespace}, which depicts a partial feature space representation of a tree according to \nuovotk. 
% Let $\subtreelimitedrootedat{\node~~~}{h}$ be the subtree of $T$ resulting from a breadth-first visit starting at $\node$ and limited to $h$ levels of depth. 
For each node $\node\in T$, for example the node hightlighted in Figure~\ref{fig:nuovokernelfeaturespace}-a, the algorithm inserts at most $\rho(\node)h+1$ features: 
\begin{itemize}
  \item the proper subtree rooted at $\node$, which in our example is the one in  Figure~\ref{fig:nuovokernelfeaturespace}-b; 
  \item given the $j$-th child of $\node$, the subtree composed by 
  \begin{itemize}
    \item $\node$,
    \item the proper subtree rooted at the $j$-th child of $\node$,
    \item the subtrees resulting from a visit limited to $1\leq l\leq h$ levels starting from the other children of $\node$ 
  \end{itemize} 
  is added as feature. As $l$ ranges from $0$ to $h$, the features/subtrees from  \mbox{Figure~\ref{fig:nuovokernelfeaturespace}-c} to \mbox{Figure~\ref{fig:nuovokernelfeaturespace}-e} are added.
\end{itemize}

Substituting line $15$ of Alg.~\ref{alg:kernelsth} with Alg.~\ref{alg:nuovokernelfeatures}, an algorithm for computing the features of \nuovotk~directly from a graph $G$ is obtained. 
The variables $u$, $i$ are set in Alg.~\ref{alg:kernelsth} and represent the current node of the $DD_G^\node$ and the current level of the visit, respectively.  
The features of the ST kernel are added in line $1$ by the macro {\bfseries compute-st-features}. Notice that it sets the vectors $X[]$ and $S[]$. The variables $x$ and $s$ represent the encoding of the novel features of \nuovotk~as exemplified in Figure~\ref{fig:nuovotkfeature}.  

\begin{algorithm}%[H]
\scriptsize
{\bfseries compute-\nuovotk features}
\begin{algorithmic}[1]
    \scriptsize
    \STATE {\bfseries compute-st-features} // macro defined in Alg.~\ref{alg:kernelsth}
    \FOR{{\bfseries $1\leq j\leq \rho(u)$}}
      \FOR{{\bfseries $0\leq l<i$}}
	\STATE{$(M_1,\ldots,M_{\rho(u)})$=sort$\Big(X_{ch_u[1]}[l],\ldots,X_{ch_{u}[j-1]}[l],X_{ch_{u}[j]}[i],$\linebreak
	       $~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~	X_{ch_{u}[j+1]}[l],\ldots,X_{ch_{u}[\rho(u)]}[l]\Big)$}
% 	\STATE $x=\kappa\Big(L(u)\Big[X_{ch_1[u]}[l]\ldots \#X_{ch_{j-1}[u]}[l]\#X_{ch_{j}[u]}[i]\#X_{ch_{j+1}[u]}[l]\ldots\#X_{ch_{\rho(u)}[u]}[l]\Big]\Big)$
	\STATE $x=\kappa\Big(L(u)\Big\lceil M_1\#\ldots\#M_{\rho(u)}\Big\rfloor\Big)$
	\STATE $s = 1 + S_{ch_u[j]}[i] + \displaystyle\sum_{z=1, z\neq j}^{\rho(u)}S_{ch_u[z]}[l]$
	\IF{$x$ is a new feature}
	  \STATE $\phi_{x} = \lambda^{\frac{s}{2}}$
	\ELSE
	  \STATE $\phi_{x} = \phi_{x} + \lambda^{\frac{s}{2}}$ 
	\ENDIF
      \ENDFOR
    \ENDFOR
%     \STATE {\bfseries Input:} a tree $T$, $h$ (maximum depth of the visit)
%     \FOR{{\bfseries each $\node\in T$}}
% 	\STATE $\phi_{\hash(\node)} = \phi_{\hash(\node)} + \lambda^{\frac{|\node|}{2}}$ // add the proper subtree rooted at $\node$ as a feature.
% 	\STATE \hspace{2.62cm}// If the feature is first encountered, it is assumed $\phi_{\hash(\node)}=0$
%       \FOR{{\bfseries $0\leq d\leq h$}}
% 	\FOR{{\bfseries $1\leq j\leq \rho(\node)$}}
%  	  \STATE \begin{tikzpicture}[-,thick,scale=0.485, sibling distance=3.25cm]
%  	          \node []{$\node$}
% 		   child {node (lft) []{$\subtreelimitedrootedat{ch_1[\node]}{d}$}}
% 		   child {node[xshift=0.1cm]{$\ldots$}}
% 		   child {node[xshift=0.3cm]{$\subtreelimitedrootedat{ch_{j-1}[\node]}{d}$}}
% 		   child {node[]{$\subtreerootedat{ch_j[\node]}$}}
% 		   child {node[xshift=-0.3cm]{$\subtreelimitedrootedat{ch_{j+1}[\node]}{d}$}}
% 		   child {node[]{$\ldots$}}
% 		   child {node (rgt)[]{$\subtreelimitedrootedat{ch_{\rho(\node)}[\node]}{d}$}}	
% 		  ;
% 		  \node [left=0.0cm of lft, yshift=0.3cm] {$t = $};
%  	         \end{tikzpicture} 
% 	  \STATE ~$\phi_{\hash(t)} = \phi_{\hash(t)} + \lambda^{\frac{|t|}{2}}$ // add the subtree $t$ as a feature.
%  	\ENDFOR
%      \ENDFOR
%     \ENDFOR
%     \STATE {\bfseries Output:} $\phi$, the set of features of $T$
\end{algorithmic}
\caption{A macro for computing the features of the \nuovotk~kernel. It is supposed to replace line $15$ of Alg.~\ref{alg:kernelsth}. \label{alg:nuovokernelfeatures}}
\end{algorithm}

The complexity of Alg.~\ref{alg:kernelsth} where line $15$ is substituted with Alg.~\ref{alg:nuovokernelfeatures} is $O(|V_G|H h^2\rho^2\log \rho)$. The complexity of a kernel evaluation then is $|V_G|\log |V_G|$ if we consider $H$ constant. 
% Computing the encoding $\hash(ch_{k}[\node])$ in line $8$ of Alg.~\ref{alg:nuovokernelfeatures} for any $k\neq j$ requires $d\rho$ steps. However, the same encoding does not have to be recomputed as $j$ varies in line $6$ of Alg.~\ref{alg:nuovokernelfeatures}. Therefore, the total time required for computing the encoding $\hash()$ is $\rho\sum_{d=0}^hd=O(\rho h^2)$ and thus the complexity of Alg.~\ref{alg:nuovokernelfeatures} is $O(|T|\rho h^2)$. 
% The complexity of . 

\begin{figure}%[t] %h
\centering
\begin{tikzpicture}[auto,thick,scale=.5]
\tikzstyle{node}=[minimum size=12pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
        \node (s) [node,xshift=2.0cm, yshift=1.3cm] {\textbf{s}} [->] 
                child {
                    node [node, xshift=-0.6cm] {\textbf{d}}[] 
		     child {
			node [node, xshift=-0.0cm]{\textbf{f}}[]
		    }
                }
                child {
		    node [node, ball color=yellow, text=black]{\textbf{v}}[]
  		    child {
			node [node, xshift=0.25cm]{\textbf{a}}[]
		    }
		    child {
		      node [node, ball color=yellow, text=black]{\textbf{x}}[]
		      child {
			node [node]{\textbf{d}}[]
			child {
			  node [node]{\textbf{e}}[]
			}
			child {
			  node [node]{\textbf{f}}[]
			}
		      }
		    }
                   child {
		      node (ei) [node, xshift=0cm]{\textbf{e}}[]
		      child {
			node [node, xshift=0.1cm]{\textbf{e}}[]
		      }
		      child {
			node [node, xshift=0.1cm]{\textbf{f}}[]
			child {
			  node [node]{\textbf{g}}[]
			}
		      }
		    }
		    child {
			node (eei) [node, xshift=0.2cm]{\textbf{e}}[]
			child {
			  node [node]{\textbf{g}}[]
			}
		    }
               }
		child {
		  node (b) [node, xshift=0.5cm]{\textbf{b}}[]
		};
	\node (laba) []{a)}[];%%[left=0.1cm of ei]{a)}[];%
	\draw [red,->,line width=5pt, right=1cm of laba] (7.5,-0.4)--(9.0,-0.4);
		    \node (rf1) [node, right=4cm of s, yshift=-0.5cm]{\textbf{v}}[]
  		    child {
			node [node, xshift=0.25cm]{\textbf{a}}[]
		    }
		    child {
		      node [node]{\textbf{x}}[]
		      child {
			node [node]{\textbf{d}}[]
			child {
			  node [node]{\textbf{e}}[]
			}
			child {
			  node [node]{\textbf{f}}[]
			}
		      }
		    }
                   child {
		      node (ei) [node, xshift=0cm]{\textbf{e}}[]
		      child {
			node [node, xshift=0.1cm]{\textbf{e}}[]
		      }
		      child {
			node [node, xshift=0.1cm]{\textbf{f}}[]
			child {
			  node [node]{\textbf{g}}[]
			}
		      }
		    }
		    child {
			node (eei) [node, xshift=0.2cm]{\textbf{e}}[]
			child {
			  node [node]{\textbf{g}}[]
			}
		    };
 	  \node (labb) [right=4.35cm of laba]{b)}[];
% 		    \node (rf2) [node, right=2.5cm of rf1]{\textbf{v}}[]
% 		    child {
% 		      node [node]{\textbf{x}}[]
% 		      child {
% 			node [node]{\textbf{d}}[]
% 			child {
% 			  node [node]{\textbf{e}}[]
% 			}
% 			child {
% 			  node [node]{\textbf{f}}[]
% 			}
% 		      }
% 		    }
% 		    ;
%       \node[right=3.0cm of labb]{c)}[]; %
		    \node (rf2) [node, below=2.25cm of laba, xshift=0.7cm]{\textbf{v}}[]
		    child {
		      node [node]{\textbf{x}}[]
		      child {
			node [node]{\textbf{d}}[]
			child {
			  node [node]{\textbf{e}}[]
			}
			child {
			  node [node]{\textbf{f}}[]
			}
		      }
		    }
		    ;
      \node (labc) [below=2.8cm of laba]{c)}[]; %
      \node[right=0.7cm of labc, yshift=-1.2cm]{$l=0$}[]; %
%       \node (labc) [below=2.8cm of laba]{c)}[];
      \node [right=3.6cm of labc, yshift=-1.25cm]{$l=1$}[];
      \node [right=1.6cm of labc]{d)}[];
		    \node (rf3) [node, below=3.6cm of s, xshift=1.6cm]{\textbf{v}}[]
  		    child {
			node [node, xshift=0.25cm]{\textbf{a}}[]
		    }
		    child {
		      node [node]{\textbf{x}}[]
		      child {
			node [node]{\textbf{d}}[]
			child {
			  node [node]{\textbf{e}}[]
			}
			child {
			  node [node]{\textbf{f}}[]
			}
		      }
		    }
                   child {
		      node (ei) [node, xshift=0cm]{\textbf{e}}[]
		    }
		    child {
			node (eei) [node, xshift=0.2cm]{\textbf{e}}[]
		    };
      \node[right=5.1cm of labc]{e)}[];
      \node[right=7.0cm of labc, yshift=-1.3cm]{$l=2$}[];
		    \node (rf4) [node, right=3.0cm of rf3]{\textbf{v}}[]
  		    child {
			node [node, xshift=0.25cm]{\textbf{a}}[]
		    }
		    child {
		      node [node]{\textbf{x}}[]
		      child {
			node [node]{\textbf{d}}[]
			child {
			  node [node]{\textbf{e}}[]
			}
			child {
			  node [node]{\textbf{f}}[]
			}
		      }
		    }
                   child {
		      node (ei) [node, xshift=0cm]{\textbf{e}}[]
		      child {
			node [node, xshift=0.1cm]{\textbf{e}}[]
		      }
		      child {
			node [node, xshift=0.1cm]{\textbf{f}}[]
		      }
		    }
		    child {
			node (eei) [node, xshift=0.2cm]{\textbf{e}}[]
			child {
			  node [node]{\textbf{g}}[]
			}
		    };
\end{tikzpicture}
  \caption{Feature space representation related to the kernel \nuovotk~for an example tree: a) the input tree; b) the proper subtree rooted at the node labelled as \textbf{v}; c)-e) given the child \textbf{x} of \textbf{v}, the features related to visits limited to $l$ levels. \label{fig:nuovokernelfeaturespace}}
\end{figure}


% \begin{figure}[ht]
% \centering
% \begin{tikzpicture}[auto,thick,scale=.5]
% \tikzstyle{node}=[minimum size=12pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
%         \node (s) [node,xshift=4.2cm, yshift=1.3cm] {\textbf{s}} [->] 
%                 child {
%                     node [node, xshift=-0.5cm] {\textbf{d}}[] 
%                     child {
% 		      node (ei) [node]{\textbf{e}}[]
% 		      child {
% 			node [node]{\textbf{f}}[]
% 			child {
% 			  node [node]{\textbf{e}}[]
% 			}
% 		      }
% 		      child {
% 			node [node]{\textbf{g}}[]
% 		      }
% 		    }
%                 }
%                 child {
% 		    node [node]{\textbf{a}}[]
% 		    child {
% 		      node [node]{\textbf{c}}[]
% 		      child {
% 			node [node]{\textbf{a}}[]
% 		      }
% 		      child {
% 			node [node, ball color=yellow, text=black]{\textbf{d}}[]
% 			child {
% 			  node (eei) [node]{\textbf{e}}[]
% 			}
% 			child {
% 			  node [node]{\textbf{h}}[]
% 			  child {
% 			    node [node]{\textbf{f}}[]
% 			  }
% 			  child {
% 			    node [node]{\textbf{b}}[]
% 			  }
% 			}
% 		      }
% 		    }
%                 }
% 		child {
% 		  node (b) [node, xshift=0.9cm]{\textbf{b}}[]
% 		  child {
% 		    node [node]{\textbf{a}}[]
% 		    child {
% 		      node [node]{\textbf{g}}[]
% 		    }
% 		  }
%  		  child {
% 		    node [node]{\textbf{b}}[]
% 		    child {
% 		      node (d) [node]{\textbf{d}}[]
% 		      child {
% 			node [node]{\textbf{e}}[]
% 		      }
% 		    }
% 		  }
% 		  child {
% 		    node [node]{\textbf{c}}[]
% 		  }
% 		};
% 	\node (laba) [left=0.1cm of ei]{a)}[];%
% 	\draw [red,->,line width=5pt, right=1cm of laba] (14.0,-0.4)--(15.5,-0.4);
% 	 \node (rf1) [node, right=4.25cm of s, yshift=-0.5cm]{\textbf{d}}[]
% 	  child {
% 	    node (est) [node]{\textbf{e}}[]
% 	  }
% 	  child {
% 	    node [node]{\textbf{h}}[]
% 	    child {
% 	      node [node]{\textbf{f}}[]
% 	    }
% 	    child {
% 	      node [node]{\textbf{b}}[]
% 	    }
% 	  };
% 	  \node (labb) [right=5.1cm of laba]{b)}[];
% 	  \node [node, right=1.5cm of rf1]{\textbf{s}}[]
% 	   child {
% 	    node [node]{\textbf{a}}[]
% 	    child {
% 	      node (f2) [node]{\textbf{c}}[]
% 	      child {
% 		node [node]{\textbf{a}}[]
% 	      }
% 	      child {
% 		node [node]{\textbf{d}}[]
% 		child {
% 		  node [node]{\textbf{e}}[]
% 		}
% 	      child {
% 		node [node]{\textbf{h}}[]
% 		child {
% 		    node [node]{\textbf{f}}[]
% 		}
% 		child {
% 		    node [node]{\textbf{b}}[]
% 		}
% 	      }
% 	      }
% 	    }
%            };
% 	  \node[right=1.75cm of labb]{c)}[]; %
%         \node (rf3) [node,below=1.0cm of eei] {\textbf{s}} [->] 
%                 child {
%                     node [node, xshift=-0.5cm] {\textbf{d}}[] 
% %                     child {
% % 		      node (f3) [node]{\textbf{e}}[]
% % 		      child {
% % 			node [node]{\textbf{f}}[]
% % 			child {
% % 			  node [node]{\textbf{e}}[]
% % 			}
% % 		      }
% % 		      child {
% % 			node [node]{\textbf{g}}[]
% % 		      }
% % 		    }
%                 }
%                 child {
% 		    node [node]{\textbf{a}}[]
% 		    child {
% 		      node [node]{\textbf{c}}[]
% 		      child {
% 			node [node]{\textbf{a}}[]
% 		      }
% 		      child {
% 			node [node]{\textbf{d}}[]
% 			child {
% 			  node [node]{\textbf{e}}[]
% 			}
% 			child {
% 			  node [node]{\textbf{h}}[]
% 			  child {
% 			    node [node]{\textbf{f}}[]
% 			  }
% 			  child {
% 			    node [node]{\textbf{b}}[]
% 			  }
% 			}
% 		      }
% 		    }
%                 }
% 		child {
% 		  node (b) [node, xshift=0.9cm]{\textbf{b}}[]
% % 		  child {
% % 		    node [node]{\textbf{a}}[]
% % 		    child {
% % 		      node [node]{\textbf{g}}[]
% % 		    }
% % 		  }
% %  		  child {
% % 		    node [node]{\textbf{b}}[]
% % 		    child {
% % 		      node (d) [node]{\textbf{d}}[]
% % 		      child {
% % 			node [node]{\textbf{e}}[]
% % 		      }
% % 		    }
% % 		  }
% % 		  child {
% % 		    node [node]{\textbf{c}}[]
% % 		  }
% 		};
% 	      \node (labc) [below=3cm of laba]{d)}[];
%         \node (rf4) [node,right=3.5cm of rf3] {\textbf{s}} [->] 
%                 child {
%                     node [node, xshift=-0.5cm] {\textbf{d}}[] 
%                     child {
% 		      node (ei) [node]{\textbf{e}}[]
% % 		      child {
% % 			node [node]{\textbf{f}}[]
% % 			child {
% % 			  node [node]{\textbf{e}}[]
% % 			}
% % 		      }
% % 		      child {
% % 			node [node]{\textbf{g}}[]
% % 		      }
% 		    }
%                 }
%                 child {
% 		    node [node]{\textbf{a}}[]
% 		    child {
% 		      node [node]{\textbf{c}}[]
% 		      child {
% 			node [node]{\textbf{a}}[]
% 		      }
% 		      child {
% 			node [node]{\textbf{d}}[]
% 			child {
% 			  node [node]{\textbf{e}}[]
% 			}
% 			child {
% 			  node [node]{\textbf{h}}[]
% 			  child {
% 			    node [node]{\textbf{f}}[]
% 			  }
% 			  child {
% 			    node [node]{\textbf{b}}[]
% 			  }
% 			}
% 		      }
% 		    }
%                 }
% 		child {
% 		  node (b) [node, xshift=0.9cm]{\textbf{b}}[]
% 		  child {
% 		    node [node]{\textbf{a}}[]
% % 		    child {
% % 		      node [node]{\textbf{g}}[]
% % 		    }
% 		  }
%  		  child {
% 		    node [node]{\textbf{b}}[]
% % 		    child {
% % 		      node (d) [node]{\textbf{d}}[]
% % 		      child {
% % 			node [node]{\textbf{e}}[]
% % 		      }
% % 		    }
% 		  }
% 		  child {
% 		    node [node]{\textbf{c}}[]
% 		  }
% 		};
% 	      \node[right=3cm of labc]{d)}[];
% \end{tikzpicture}
%   \caption{Feature space representation related to the kernel \nuovotk for an example tree.\label{fig:nuovokernelfeaturespacelllll}}
% \end{figure}

\subsection{A Graph Kernel for Continuous Node Labels and Edges} \label{sec:sstcontinuous}

\nuovo{In many real world problems, node and edge labels may belong to complex domains, such as real numbers and vectorial data \cite{}. 
Kernels for discrete data tend to perform poorly when node labels belong to continuous domains due to sparsity issues \cite{}. 
This section shows a class of novel kernels for graphs able to deal with edge labels and non-discrete node labels. 
Our strategy is again to extend some of the tree kernels described in Section~\ref{sec:kernelsfortrees} to continuous domains and to deal with edge labels. 
We focus on the SST kernel in the following, but similar changes can be easily applied to other kernels. 
First a few definition need to be extended to the continuous domain}{Rev 1 (tutta la sezione e' nuova)}.
Let $L()$ be a function that map nodes to a generic codomain $\cal{X}_L$. 
Similarly, a function $L_E()$, whose codomain is $\cal{X}_E$, returns the label of a specific edge. 
Let us assume a total ordering for $\cal{X}_L$ and $\cal{X}_E$ is defined. 
The ordering in \definizione{\ref{def:leq}} can be extended to include edges by prepending the representation of the edge to the one of the corresponding child node: 	
$\kappa\big(L(\node)\big\lceil \hash{(\node,ch_\node[1])}\#\hash(ch_\node[1])\#\ldots\#\hash{(\node,ch_\node[\rho(\node)])}\#\hash(ch_\node[\rho(\node)])\big\rfloor\big) $
% Note that all the results in Section~\ref{} do not depend on the . 
Let us assume a kernel for labels, $K_L:\cal{X}_L\times\cal{X}_L$, and a kernel for edges, $K_E:\cal{X}_E\times\cal{X}_E$ are available. 
Then the $C()$ definition of SST can be extended as follows: 
\textit{i}) if $\node_1$ or $\node_2$ are leaf nodes or $\rho(\node_1)\neq \rho(\node_2)$ then $C_{SST}(\node_1,\node_2)=K_L(\labelfun(\node_1),\labelfun(\node_2))$;\\
\textit{ii}) if $\node_1$ and $\node_2$ are not leaf nodes and $\rho(\node_1)=\rho(\node_2)$ then
	\begin{equation}
	  \begin{array}{l}
	    \displaystyle C_{SST}(\node_1,\node_2)=K_L(\labelfun(\node_1),\labelfun(\node_2))\displaystyle\prod_{j=1}^{\rho(\node_1)}K_E((\node_1,ch_{\node_1}[j]),\\\hfill(\node_2,ch_{\node_2}[j]))\Big(\sigma + C_{CSST}(ch_{\node_1}[j],ch_{\node_2}[j])\Big). 
	  \end{array}
	  \label{eq:ccsst}
        \end{equation}
%Assuming the complexity of $K_L()$ and $K_E()$ are  
Following the reasoning at the end of Section~\ref{sec:treekernelsfordags}, the complexity of the kernel in \eqref{eq:ccsst} is $O(n^2H^2 Q(K_E) Q(K_L))$, where $Q(K_E)$ and $Q(K_L)$ are the worst case complexities of the kernels $K_L()$ and $K_E()$. 

% 
% \textit{i}) if $\node_1$ or $\node_2$ are leaf nodes or $\rho(\node_1)\neq \rho(\node_2)$, then $K_L(\labelfun(\node_1),\labelfun(\node_2))$; 
% \textit{ii}) if $\labelfun(\node_1)=\labelfun(\node_2)$ and both $\node_1$ and $\node_2$ are preterminal nodes, i.e. parent of a leaf node, then $C_{SST}(\node_1,\node_2)=\lambda$; 
% \textit{iii}) if $\labelfun(\node_1)=\labelfun(\node_2)$ and either $\node_1$ or $\node_2$ is not a  preterminal node, then 
% 
% \begin{equation}
%   K_{CSST}(\node_1, \node_2) = K_L(\labelfun(\node_1),\labelfun(\node_2)) \text{if $\node_1$ is leaf $\vee$ $\node_2$ is leaf $\vee$}
%  \label{eq:CSST}
% \end{equation}
% 
% 
%  \begin{equation}
%   C_{CSST}(\node_1,\node_2) = 
%   \begin{cases}
%     \displaystyle K_L(\labelfun(\node_1),\labelfun(\node_2)) \text{~~~if $\node_1$ or $\node_2$ are leaf}\\ \hfill \text{nodes or $\rho(\node_1)\neq\rho(\node_2)$}\\
%     \displaystyle K_L(\labelfun(\node_1),\labelfun(\node_2))\displaystyle\prod_{j=1}^{\rho(\node_1)} \Big(\sigma + C_{CSST}(ch_{\node_1}[j],ch_{\node_2}[j])\Big)\\K_E((\node_1,ch_{\node_1}[j]),(\node_2,ch_{\node_2}[j])) \text{otherwise}, 
%   \end{cases}
% \label{eq:csst}
%  \end{equation}







==> ordering.tex <==
% \subsection{Ordering DAG vertices} \label{sec:orderingdagvertices}
% 
% The procedure described in section~\ref{sec:odd} yields a multiset of Decompositional DAGs from a graph. However, such DAGs are not ordered. 
% Despite the fact that it has been demonstrated that the computation of any tree kernel for unordered trees with subtrees as their substructures is \mbox{$\sharp P$-complete \cite{Kashima2007}}, some kernels for unordered trees have been defined in literature \cite{Kimura2011, Vishwanathan2003}. 
% Such kernels, in order to be tractable, tend to restrict the type of substructures used as features, thus potentially limiting their expressiveness. Indeed, a set of experiments performed with the kernel in \cite{Kimura2011} on the datasets described in section~\ref{sec:exps} show that the kernel never improves, in terms of classification performances, over the state of the art (for this reason we avoided to report the results in the experimental section). 
% 
% In order to broaden the applicability of our approach, in this section we define a \textit{strict partial order} among vertices of a DAG which  allows us to employ the kernels defined in section~\ref{sec:kernelsfortrees}. 
% %
% The ordering makes use of a unique representation of subtrees. 
% In \cite{Vishwanathan2003} an injective mapping from subtrees to strings is presented. Here we modify such mapping by employing perfect hash functions to encode subtrees. As a consequence we obtain a compressed subtree representation, which will be also used in section~\ref{sec:hash}: 
% \begin{definition}
%  \label{def:leqtree}
%  \textbf{Strict partial order relation $\dot{<}$ between tree vertices} \\
%   Let $\kappa()$ be a perfect hash function defined on strings, and $\hash()$ a function whose purpose is to encode tree vertices: If $\node$ is a leaf node, then $\hash(\node)=\kappa(L(\node))$; otherwise, let $\#,],[\notin \cal{A}$ be symbols never appearing in any node label, then 
% $$\hash(\node)=\kappa\big(L(\node)\big[ \hash(ch_1[\node])\#\hash(ch_2[\node])\ldots\#\hash(ch_{\rho(\node)}[\node])\big]\big),$$
%   where the children of $\node$ are assumed to be ordered according to $\hash()$. \\
% Then $\node_{i} \dot{<} \node_{j}$ if $\hash(\node_i)<\hash(\node_j)$, where $<$ is the relation of order between alphanumeric strings. 
% \end{definition}\\
% The assumption that the children of a node are already ordered according to $\hash()$ can be easily fulfilled by applying $\hash()$ according to a post order visit of the DAG. 
% Since $\kappa()$ is a perfect hash,  %and given the encoding for DAG vertices described in \definizione~\ref{def:leq}, 
% if two tree vertices have different node labels or at least a different child, then they can not have the same $\hash()$ value (a detailed demonstration in the case $\kappa()$ is the identity function can be found in \cite{Vishwanathan2003}). %In other words, $\hash()$, when applied to tree vertices, is an injective function. 
% As a consequence, the ordering between $\hash()$ values is a strict partial order since it is based on the alphanumeric ordering $<$ of strings. Then the ordering $\dot{<}$ between tree vertices described in \definizione~\ref{def:leq} is also a strict partial order. 
% 
% Let a tree visit be a function $T(\node_i)$ that, given a node $\node$ of a $DD^{\node_{i}}_{G}$, returns the tree resulting from the visit of the DAG starting from $\node_{i}$. If the DAG is not ordered, then the tree visit is not ordered. 
% Figure~\ref{fig:treevisit} gives an example of tree visits. Note that different DAGs may yield the same tree visit: for example the trees resulting from the visit starting in node \textbf{s} are identical for the DAGs in Figure~\ref{fig:treevisit}-a and Figure~\ref{fig:treevisit}-b.   
% \begin{definition}
%  \label{def:leq}
%  \textbf{Strict partial order relation $\dot{<}$ between DAG vertices} \\
% Given two DAG nodes, $\node_i$ and $node_j$, then 
% $\node_{i} \dot{<} \node_{j}$ if $\hash(T(\node_i))<\hash(T(\node_j))$. 
% \end{definition}\\ 
% By applying the same reasoning of \definizione~\ref{def:leqtree} it can be shown that the ordering of \definizione~\ref{def:leq} is a strict partial order. 
% 
% The function $T(\node)$, when applied to DAG vertices, 
% % The concept of tree visit is used in the following 
% The following theorem shows that isomorphic DAGs 
% \begin{theorem} \label{teo:visits}
% 	If $\neg(\node_i \dot{<} \node_j) \wedge \neg(\node_j \dot{<} \node_i)$ according to Definition~\ref{def:leq}, then the trees $T(\node_i)$ and $T(\node_j)$, obtained as visits of the subdags rooted at $\node_i$ and $\node_j$, are identical. 
% \end{theorem}
% \begin{proof}
%  If $\neg(\node_i \dot{<} \node_j) \wedge \neg(\node_j \dot{<} \node_i)$ then $\hash(\node_i)\geq \hash(\node_j) \wedge \hash(\node_j)\geq \hash(\node_j) \Leftrightarrow \hash(\node_i)=\hash(\node_j)$. Recalling that $\hash()$ is injective, we prove the thesis by induction. If $\node_i, \node_j$ are leaf nodes, then $\hash(\node_i)=\hash(\node_j)\Leftrightarrow L(\node_i)=L(\node_j)$. If $\node_i, \node_j$ are not leaf nodes, then $\forall 1\leq l\leq \rho(\node_i)$ $T(ch_l[\node_i])$ is identical to $T(ch_l[\node_j])$ for inductive hypothesis, and then it must be $L(\node_i)=L(\node_j)$ since $\hash(\node_i)=\hash(\node_j)$; therefore $T(\node_i)$ is identical to $T(\node_j)$. 
% \end{proof}
% 
% 
% % % It resembles the injective mapping in \cite{Vishwanathan2003}, although we choose to employ perfect hash functions to compactely represent subtrees, since we will also make use of them in section~\ref{sec:hash}: 
% % \begin{definition}
% %  \label{def:mapping}
% % \textbf{SubDAG Encoding} \\
% % let $\#,],[\notin \cal{A}$ be symbols never appearing in any node label. If $\node$ is a leaf node, its encoding is $h(L(\node))$, otherwise $\node$ is encoded as $$h(L(\node))\big[ h(ch_1[\node])\#h(ch_2[\node])\ldots\#h(ch_{\rho(\node)}[\node])\big].$$  
% % \end{definition}
% % \begin{definition}
% %  \label{def:leq}
% %  \textbf{Strict partial order relation $\dot{<}$ between DAG vertices} \\
% %   Let $\kappa()$ be a perfect hash function defined on strings, and $\hash()$ a function whose purpose is to encode DAG vertices: If $\node$ is a leaf node, then $\hash(\node)=\kappa(L(\node))$; otherwise, let $\#,],[\notin \cal{A}$ be symbols never appearing in any node label, then 
% % $$\hash(\node)=\kappa\big(L(\node)\big[ \hash(ch_1[\node])\#\hash(ch_2[\node])\ldots\#\hash(ch_{\rho(\node)}[\node])\big]\big),$$
% %   where the children of $\node$ are assumed to be ordered according to $\hash()$. \\
% % Then $\node_{i} \dot{<} \node_{j}$ if $\hash(\node_i)<\hash(\node_j)$, where $<$ is the relation of order between alphanumeric strings. 
% % \end{definition}\\
% % The assumption that the children of a node are already ordered according to $\hash()$ can be easily fulfilled by applying $\hash()$ according to a post order visit of the DAG. 
% % Since $\kappa()$ is a perfect hash and given the encoding for DAG vertices described in \definizione~\ref{def:leq}, if two vertices have different node labels or at least a different child, then they can not have the same $\hash()$ value (a detailed demonstration in the case $\kappa()$ is the identity function can be found in \cite{Vishwanathan2003}). In other words, $\hash()$ is an injective function. 
% % As a consequence, the ordering between $\hash()$ values is a strict partial order since it is based on the alphanumeric ordering $<$ of strings. Then the ordering $\dot{<}$ between DAG vertices described in \definizione~\ref{def:leq} is also a strict partial order. 
% 
% In the following, we will denote the Decompositional Dag ordered according to \definizione~\ref{def:leq} as $ODD^{\node_{i}}_{G}$. The time complexity of the ordering phase is $O(|V| \rho\log \rho)$ where the term $\rho\log \rho$ accounts for the ordering of the children of each node.
% 
% The reason for defining the ordering according to Definition~\ref{def:leq} is that it must be efficient to compute and must ensure that the swapping of non comparable nodes does not affect the feature space representation of the DAG. After introducing the extension of tree kernels to DAGs in Section~\ref{sec:treekernelsfordags}, we will show that our ordering meets both constraints. The remainder of this section introduces concepts and prove results needed in Section~\ref{sec:treekernelsfordags}. 
%  
% Let a tree visit be a function $T(\node_i)$ that, given a node $\node$ of a $ODD^{\node_{i}}_{G}$, returns the tree resulting from the visit of the DAG starting from $\node_{i}$. Figure~\ref{fig:treevisit} gives an example of tree visits. Note that the trees resulting from the visit starting in node \textbf{s} are identical for the DAGs in Figure~\ref{fig:treevisit}-a) and Figure~\ref{fig:treevisit}-b). However, if we consider the set of trees returned by all the tree visits, the DAGs in Figure~\ref{fig:treevisit}-a) and Figure~\ref{fig:treevisit}-b) can be discriminated since one tree is produced by the visit starting in node \textbf{d} of the DAG in Figure~\ref{fig:treevisit}-a) and two trees are generated by the two visits starting in the nodes labelled with \textbf{d} in Figure~\ref{fig:treevisit}-b). 
% Moreover, note that the set of tree visits would be different even if the nodes labelled with \textbf{d} were not leaves. 
% % The concept of tree visit is used in the following 
% % \begin{theorem} \label{teo:visits}
% % 	If $\neg(\node_i \dot{<} \node_j) \wedge \neg(\node_j \dot{<} \node_i)$ according to Definition~\ref{def:leq}, then the trees $T(\node_i)$ and $T(\node_j)$, obtained as visits of the subdags rooted at $\node_i$ and $\node_j$, are identical. 
% % \end{theorem}
% % \begin{proof}
% %  If $\neg(\node_i \dot{<} \node_j) \wedge \neg(\node_j \dot{<} \node_i)$ then $\hash(\node_i)\geq \hash(\node_j) \wedge \hash(\node_j)\geq \hash(\node_j) \Leftrightarrow \hash(\node_i)=\hash(\node_j)$. Recalling that $\hash()$ is injective, we prove the thesis by induction. If $\node_i, \node_j$ are leaf nodes, then $\hash(\node_i)=\hash(\node_j)\Leftrightarrow L(\node_i)=L(\node_j)$. If $\node_i, \node_j$ are not leaf nodes, then $\forall 1\leq l\leq \rho(\node_i)$ $T(ch_l[\node_i])$ is identical to $T(ch_l[\node_j])$ for inductive hypothesis, and then it must be $L(\node_i)=L(\node_j)$ since $\hash(\node_i)=\hash(\node_j)$; therefore $T(\node_i)$ is identical to $T(\node_j)$. 
% % \end{proof}
% 
% 







\subsection{Ordering DAG vertices} \label{sec:orderingdagvertices}

The procedure described in Section~\ref{sec:odd} yields a multiset of Decompositional DAGs from a graph. However, such DAGs are not ordered. 
Despite the fact that it has been demonstrated that the computation of any tree kernel for unordered trees with subtrees as their substructures is \mbox{$\sharp P$-complete \cite{Kashima2007}}, some kernels for unordered trees have been defined in literature \cite{Kimura2011, Vishwanathan2003}. 
Such kernels, in order to be tractable, tend to restrict the type of substructures used as features, thus potentially limiting their expressiveness. Indeed, a set of experiments performed with the kernel in \cite{Kimura2011} on the datasets described in Section~\ref{sec:exps} show that the kernel never improves, in terms of classification performances, over the state of the art (for this reason we do not report the results in the experimental section). 

In order to broaden the applicability of our approach, in this section we define a \textit{strict partial order} among vertices of a DAG which  allows us to employ the kernels defined in Section~\ref{sec:kernelsfortrees}. 
%
The ordering makes use of a unique representation of subtrees as strings inspired by \cite{Vishwanathan2003}.  
% In \cite{Vishwanathan2003} an injective mapping from subtrees to strings is presented. Here we modify such mapping by employing perfect hash functions to encode subtrees. 
Here we modify such mapping by employing perfect hash functions to encode subtrees. 
As a consequence we obtain a compressed subtree representation, which will be also used in section~\ref{sec:hash} to implement one of the kernels proposed in this paper. 
The compressed representation is here used to define an ordering between DAG vertices:  
% \begin{definition}
%  \label{def:leq}
%  \textbf{Strict partial order relation $\dot{<}$ between DAG vertices} \\
%   Let $\kappa()$ be a perfect hash function defined on strings, and $\hash()$ a function whose purpose is to encode DAG vertices: If $\node$ is a leaf node, then $\hash(\node)=\kappa(L(\node))$; otherwise, let $\#,],[\notin \cal{A}$ be symbols never appearing in any node label, then 
% $$\hash(\node)=\kappa\big(L(\node)\big[ \hash(ch_1[\node])\#\hash(ch_2[\node])\ldots\#\hash(ch_{\rho(\node)}[\node])\big]\big),$$
%   where the children of $\node$ are assumed to be ordered according to $\hash()$. \\
% Then $\node_{i} \dot{<} \node_{j}$ if $\hash(\node_i)<\hash(\node_j)$, where $<$ is the relation of order between alphanumeric strings. 
% \end{definition}\\
% The assumption that the children of a node are already ordered according to $\hash()$ can be easily fulfilled by applying $\hash()$ according to a post order visit of the DAG. 
% Since $\kappa()$ is a perfect hash and given the encoding for DAG vertices described in \definizione~\ref{def:leq}, if two vertices have different node labels or at least a different child, then they can not have the same $\hash()$ value (a detailed demonstration in the case $\kappa()$ is the identity function can be found in \cite{Vishwanathan2003}). In other words, $\hash()$ is an injective function. 
% As a consequence, the ordering between $\hash()$ values is a strict partial order since it is based on the alphanumeric ordering $<$ of strings. Then the ordering $\dot{<}$ between DAG vertices described in \definizione~\ref{def:leq} is also a strict partial order. 
% % It resembles the injective mapping in \cite{Vishwanathan2003}, although we choose to employ perfect hash functions to compactely represent subtrees, since we will also make use of them in section~\ref{sec:hash}: 
% \begin{definition}
%  \label{def:mapping}
% \textbf{SubDAG Encoding} \\
% let $\#,],[\notin \cal{A}$ be symbols never appearing in any node label. If $\node$ is a leaf node, its encoding is $h(L(\node))$, otherwise $\node$ is encoded as $$h(L(\node))\big[ h(ch_1[\node])\#h(ch_2[\node])\ldots\#h(ch_{\rho(\node)}[\node])\big].$$  
% \end{definition}
\begin{definition}[Strict partial order relation $\dot{<}$ between DAG vertices]
 \label{def:leq}
%   Let $\kappa()$ be a perfect hash function defined on strings, and $\hash()$ a function whose purpose is to encode DAG vertices: If $\node$ is a leaf node, then $\hash(\node)=\kappa(L(\node))$; otherwise, let $\#,\lceil,\rfloor\notin \cal{A}$ be symbols never appearing in any node label, then 
% $$\hash(\node)=\kappa\big(L(\node)\big\lceil \hash(ch_1[\node])\#\hash(ch_2[\node])\ldots\#\hash(ch_{\rho(\node)}[\node])\big\rfloor\big),$$
Let $\kappa()$ be a perfect hash function and $\#,\lceil,\rfloor\notin \cal{A}$ be symbols never appearing in any node label, then 
$$\hash(\node)=\begin{cases}
  \kappa(L(\node)) \text{\hspace{3.6cm}if $\node$ is a leaf node}\\
%   \kappa\big(L(\node)\big\lceil \hash(ch_\node[1])\#\hash(ch_\node[2])\ldots\#\hash(ch_\node[\rho(\node)])\big\rfloor\big) \\
%    \text{\hspace{5.8cm}otherwise},\\ 
  \kappa\big(L(\node)\big\lceil \hash(ch_\node[1])\#\ldots\#\hash(ch_\node[\rho(\node)])\big\rfloor\big) \text{\hspace{0.1cm}otherwise},\\ 
  \end{cases}
$$
  where the children of $\node$ are recursively ordered according to their $\hash()$ values. 
Then $\node_{i} \dot{<} \node_{j}$ if $\hash(\node_i)<\hash(\node_j)$, where $<$ is the relation of order between alphanumeric strings. 
\end{definition} 
Notice that $\hash(\node_i)=\hash(\node_j)\Leftrightarrow \neg(\node_i \dot{<} \node_j) \wedge \neg(\node_j \dot{<} \node_i)$, i.e.  $\hash(\node_i)=\hash(\node_j)$ if and only if the nodes $\node_i$ and $\node_j$ are not comparable. 
In such case, many orderings for non comparable children nodes in \definizione~\ref{def:leq} are possible. We will show in Section~\ref{sec:treekernelsfordags} that any of them yields the same representation in terms of features and thus the related kernel functions for graphs are well defined. For this reason we avoid to give a specific ordering between non comparable vertices. 
If two vertices $\node_i$, $\node_j$ have different node labels or at least two children $ch_{\node_i}[l]$, $ch_{\node_j}[m]$ (possibly $l=m$) have a different representation, then the use of the symbols $\#,\lceil,\rfloor$ and the fact that $\kappa()$ is perfect ensures that they can not have the same $\hash()$ value (a detailed demonstration in the case $\kappa()$ is the identity function can be found in \cite{Vishwanathan2003}). 
% Since $\kappa()$ is a perfect hash and given the encoding for DAG vertices described in \definizione~\ref{def:leq}, if two vertices have different node labels or at least a different child, then they can not have the same $\hash()$ value (a detailed demonstration in the case $\kappa()$ is the identity function can be found in \cite{Vishwanathan2003}). 
% In other words, $\hash()$ is an injective function. 
The ordering between $\hash()$ values is a strict partial order, i.e. irreflexive, transitive and asymmetric, since it is based on the alphanumeric \mbox{ordering $<$} of strings. Then the ordering $\dot{<}$ between DAG vertices described in \definizione{\ref{def:leq}} is also a strict partial order. 
%  \begin{theorem}
%   \label{teo:orderingwelldefined}
%  The relation in \definizione~\ref{def:leq} is a strict partial order between DAG vertices.
%  \end{theorem}
%  \begin{proof}	
%  A strict partial order is a relation on a set that is irreflexive, asymmetric and transitive. Since $\kappa()$ is a perfect hash and given the encoding for DAG vertices described in \definizione~\ref{def:leq}, if two vertices differ for their node label or for a children, then they can not have the same $h()$ value. A first consequence is that $\neg(\node_{i} \dot{<} \node_{i})$. 
%  \end{proof}
% 
% By exploiting \definizione~\ref{def:leq}, \definizione~\ref{def:mapping}, and the recursive application of \Lemma~\ref{lemmaeq}, 
% We can now prove the following lemma
%   \begin{lemma} Let $>$ and $=$ be the natural relations of order and equivalence between alphanumeric strings, then the following statements are true
%     \label{lemmamapping}
%     \begin{description}
%     \item i) $\neg(\node_{j} \dot{<} \node_{k}) \wedge \neg(\node_{k} \dot{<} \node_{j})$ if and only if $h(\node_{j}) = h(\node_{k})$.
%     \item ii) $\node_{j} \dot{<} \node_{k}$ if and only if $h(\node_{j}) < h(\node_{k})$;
%     \end{description}     
%     \end{lemma} 
%     \begin{proof}
%     {\it i)} The proof is done by induction. $\Rightarrow)$ Since the mapping in \definizione~\ref{def:mapping} is injective, we need to show that the input of the encoding function is identical. If $\node_j, \node_k$ are leaf nodes, then $h(\node_j)=h(\node_k)$ by \Lemma~\ref{lemmaeq}; otherwise, by inductive hypothesis $\forall 1\leq l\leq \rho(\node_j)=\rho(\node_k). h(ch_l[\node_j])=h(ch_l[\node_k])$, thus the encoding for non leaf nodes in \definizione~\ref{def:mapping} again ensures that $h(\node_j)=h(\node_k)$ (see the proof in \cite{Vishwanathan2003} for details). 
%     $\Leftarrow)$ If the encoding of $\node_j$ and $\node_k$ is identical, then $L(\node_j)=L(\node_k)$ and the thesis follows by \Lemma~\ref{lemmaeq} for leaf nodes; if $\node_j, \node_k$ are not leaf nodes, by inductive hypothesis $\forall 1\leq l\leq \rho(\node_j)=\rho(\node_k). \neg(ch_l[\node_{j}] \dot{<} ch_l[\node_{k}]) \wedge \neg(ch_l[\node_{k}] \dot{<} ch_l[\node_{j}])$ and thus the thesis follows again by \Lemma~\ref{lemmaeq}. \\
%     {\it ii)} $\Rightarrow)$ If $\node_{j} \dot{<} \node_{k}$ for rule 1. or 2. in \definizione~\ref{def:leq} 
% 
% % 
% % the fact that the symbol $\#$ can not be found in any node label ensures that different child sequences can not be the same input to $h()$. Therefore, being $h()$ injective implies that if $\neg(\node_{j} \dot{<} \node_{k}) \wedge \neg(\node_{k} \dot{<} \node_{j})$ then $h(\node_{j}) = h(\node_{k})$ by recursive 
% %      application of L{\scriptsize EMMA}~\ref{lemmaeq} ( 
% % if $S(\node_{j}) = S(\node_{k})$ then neither $\node_{j} \dot{<} \node_{k}$ nor $\node_{k} \dot{<} \node_{j}$ can hold, otherwise
% %      there will exist a position where $S(\node_{j})$ and  $S(\node_{k})$ differ, which is in contradiction with the hypothesis.\\
%     {\it ii)}: Let us assume that $\node_{j} \dot{<} \node_{k}$ then
% if 1. or 2. applies, we have $[L(\node_{j}) < L(\node_{k})] \vee [outdeg(\node_{j}) < outdeg(\node_{k})]$ which, by Definition~\ref{def:mapping}, entails that $S(\node_{j}) < S(\node_{k})$;
% if 3. must be applied, then \mbox{$S(\node_{j})= L \cdot m \cdot \left(\prod_{i=1}^{m}S(ch_{i}[\node_j])\right)$} and \mbox{$S(\node_{k})= L \cdot m \cdot \left(\prod_{i=1}^{m}S(ch_{i}[\node_k])\right),$} where $L=L(\node_j)=L(\node_k)$ and $m = outdeg(\node_{j}) = outdeg(\node_{k})$. Moreover, let $l$ be the value of
%     the index for which 3. applies. Then, by {\it i)}, we have $\prod_{i=1}^{l-1}S(ch_{i}[\node_j]) = \prod_{i=1}^{l-1}S(ch_{i}[\node_k])$ and the above arguments
%     can be recursively applied to
%     $ch_{l}[\node_j] \dot{<} ch_{l}[\node_k]$, eventually till only vertices with $0$ out-degree are reached. For those vertices, only 1. or 2. may apply, which leads 
%     to the desired result.\\
%     Viceversa, if  $S(\node_{j}) < S(\node_{k})$, let $q$ be the first position where the two strings differ, i.e. $pos(q,S(\node_{j})) < pos(q,S(\node_{k}))$, then it is easy to see that that position
%     corresponds to the first application of 1. (i.e. $pos(q,S(\node_{j}))$ and $pos(q,S(\node_{k}))$ are labels) or 2. (i.e. $pos(q,S(\node_{j}))$ and $pos(q,S(\node_{k}))$ are out-degrees) after having only applied 3. (possibly $0$ times if $q<3$), which entails that $\node_{j} \dot{<} \node_{k}$. 
%     \end{proof}
% 
%  \begin{definition}
%   \label{def:leq}
%   \textbf{Strict partial order relation $\dot{<}$ between DAG vertices} \\
%   Let us assume a perfect hash function $h()$ defined on strings is available. Then the relation $\node_{i} \dot{<} \node_{j}$ holds if and only if one of the following conditions is met:
%     \begin{enumerate}
%      \item 
%     \end{enumerate}
% 
%  \end{definition}
% 
% 
% \subsection{Ordering Dag vertices} \label{sec:orderingdagverticesold}
% 
% The procedure described in section~\ref{sec:odd} yields a multiset of Decompositional DAGs from a graph. However, such DAGs are not ordered. 
% Despite the fact that it has been demonstrated that the computation of any tree kernel for unordered trees with subtrees as their substructures is \mbox{$\sharp P$-complete \cite{Kashima2007}}, some kernels for unordered trees have been defined in literature \cite{Kimura2011, Vishwanathan2003}. 
% Such kernels, in order to be tractable, tend to restrict the type of substructures used as features, thus potentially limiting their expressiveness. Indeed, a set of experiments performed with the kernel in \cite{Kimura2011} on the datasets described in section~\ref{sec:exps} show that the kernel never improves, in terms of classification performances, over the state of the art (for this reason we avoided to report the results in the experimental section). 
% 
% In order to broaden the applicability of our approach, in this section we define a \textit{strict partial order} among vertices of a DAG which will allow us to employ the kernels defined in section~\ref{sec:kernelsfortrees}. 
% 
% %In this section we define a \textit{strict partial order} among vertices of a DAG.
%  \begin{definition}
%  \label{def:leqold}
%  \textbf{Strict partial order relation $\dot{<}$ between DAG vertices} \\
%  Let us assume to have a total order between vertex labels (e.g. the lexicographic order). Then the relation $\node_{i} \dot{<} \node_{j}$ holds if and only if one of the following conditions is met:
%  \begin{enumerate}
% \item $\labelfun(\node_{i})<\labelfun(\node_{j})$;
% \item $[\labelfun(\node_{i})=\labelfun(\node_{j})]\ \wedge\ [\rho(\node_{i}) < \rho(\node_{j})];$
% \item Assume $[\labelfun(\node_{i})=\labelfun(\node_{j})] \wedge [\rho(\node_{i}) = \rho(\node_{j})]$ and the sons $ch_l[\node_{i}]$ of $\node_{i}$ and the sons $ch_l[\node_{j}]$ of $\node_{j}$ are partially ordered by the relation we are defining, i.e.
%  they form two partially ordered sets. \\
%  Then we can define two sequences \\
%  $ch_{1}[\node_{i}], ch_{2}[\node_{i}], \ldots , ch_{m}[\node_{i}]$, \\
%  $ch_{1}[\node_{j}], ch_{2}[\node_{j}], \ldots , ch_{m}[\node_{j}]$, \\
%   where $m = \rho(v_i) = \rho(v_j)$, and every $ch_{k}[\node_{i}]$ is a (not necessarily unique) minimal element of the set defined as $\left\{ ch_{l}[\node_{i}] | l\in \{k, \ldots, m\}\right\}$.
% Then the relation holds if:\\
% $[\exists l . ch_{l}[\node_{i}] \dot{<}  ch_{l}[\node_{j}]]\ \wedge $ \\ $[\neg\exists k<l. (ch_{k}[\node_{i}] \dot{<}  ch_{k}[\node_{j}] \vee ch_{k}[\node_{j}] \dot{<}  ch_{k}[\node_{i}])]$;
% \end{enumerate}
% \end{definition}
% \noindent From the above definition it can be shown the following  
%   \begin{lemma}
%     \label{lemmaeq}
%       $\neg(\node_{j} \dot{<} \node_{k}) \wedge \neg(\node_{k} \dot{<} \node_{j})$ if and only if the following conditions are simultaneously verified
%           \begin{description}
%            \item i) $\labelfun(\node_{j})=\labelfun(\node_{k})$ (otherwise 1. applies);
%            \item ii) $\rho(\node_{j}) = \rho(\node_{k})$ (otherwise 2. applies);
%            \item iii) $\forall l, \neg(ch_{l}[\node_{j}] \dot{<} ch_{l}[\node_{k}]) \wedge \neg(ch_{l}[\node_{k}] \dot{<} ch_{l}[\node_{j}])$ (otherwise 3. applies).
%            \end{description}    
%      \end{lemma}  
% \begin{lemma}
%   \label{lemmadue}
%   \begin{description}
%     \item i) If~ $\neg(\node_{i} \dot{<} \node_{j}) \wedge (\node_{j} \dot{<} \node_{k})$ then $(\node_{i} \dot{<} \node_{k})$. 
%     \item ii) If~ $(\node_{i} \dot{<} \node_{j}) \wedge \neg(\node_{j} \dot{<} \node_{k})$ then $(\node_{i} \dot{<} \node_{k})$. 
%   \end{description}
% \end{lemma}
%   \begin{proof}
%   We only prove {\it i)} by induction since the proof for {\it ii)} is analogous. 
%   In the case any $\node_{i}, \node_{j}, \node_{k}$ is a leaf node, the thesis follows from the transitivity of the operator $<$ on strings: $L(\node_i)=L(\node_j)$ for \Lemma~\ref{lemmaeq}, thus $L(\node_i)=L(\node_j)<L(\node_k)$ and $\node_{i} \dot{<} \node_{k}$ by \definizione~\ref{def:leq}. 
%   In the general case if $\node_{i} \dot{<} \node_{j}$ for 1. or 2. in \definizione~\ref{def:leq}, the thesis follows from the same reasoning as above. If $\node_{i} \dot{<} \node_{j}$ for 3. in \definizione~\ref{def:leq}, then $\exists l. ch_l[\node_j] \dot{<} ch_l[\node_k]$ and $\neg(ch_l[\node_i] \dot{<} ch_l[\node_j])$ for \Lemma~\ref{lemmaeq}, and the thesis follows by inductive hypothesis. 
%   \end{proof}
% 
%  \begin{theorem}
%   \label{teo:orderingwelldefinedold}
%  The relation in \definizione~\ref{def:leq} is a strict partial order between DAG vertices.
%  \end{theorem}
%   
%  \begin{proof}
%  A strict partial order is a relation on a set that is irreflexive, asymmetric and transitive. 
%   In the following each property is proven.
% \begin{itemize}
%   \item \textit{Irreflexivity}: the pair $(\node_j, \node_j)$ satisfies conditions i)-iii) of \Lemma~\ref{lemmaeq}, thus $\neg(\node_{j} \dot{<} \node_{j})$ %$\neg(\node_{i} \dot{<} \node_{i})$, i.e. no condition in Definition.~\ref{def:leq} is satisfied by the pair $(\node_i, \node_i)$:
% %   since $\node_{i}$ is mapped into $S(\node_{i})$, L{\scriptsize EMMA}~\ref{lemmamapping}.{\it ii)} applies and thus $\neg(\node_{i} \dot{<} \node_{i})$;
% \item \textit{Asymmetry}: $\node_{i} \dot{<} \node_{j}  \Rightarrow \neg (\node_{j} \dot{<} \node_{i})$. 
%  If $\node_{i} \dot{<} \node_{j}$ for 1. or 2. in \definizione~\ref{def:leq}, then $\neg(\node_{j} \dot{<} \node_{i})$ since conditions 1-3 are not satisfied in the same definition. If $\node_{i} \dot{<} \node_{j}$ for 3. then $\exists l. ch_l[\node_i] \dot{<} ch_l[\node_j]$ and $\forall k<l. \neg(ch_k[\node_j] \dot{<} ch_k[\node_i])$. By applying the inductive hypothesis on the $l$-th children we get $\neg(ch_l[\node_j] \dot{<} ch_l[\node_i])$, therefore we can conclude $\neg(\node_{j} \dot{<} \node_{i})$ because conditions 1-3 in \definizione~\ref{def:leq} are not satisfied. 
% % By L{\scriptsize EMMA}~\ref{lemmamapping}, if $\node_{i} \dot{<} \node_{j}$ then $S(\node_{i}) < S(\node_{j})$, which is not consistent with the condition $S(\node_{j}) < S(\node_{i})$ required by $\node_{j} \dot{<} \node_{i}$.
%  \item \textit{Transitivity} ($\node_{i} \dot{<} \node_{j} \wedge \node_{j} \dot{<} \node_{k} \Rightarrow \node_{i} \dot{<} \node_{k}$). 
% We prove the thesis by induction. The base case and when $\node_{i} \dot{<} \node_{j}$ for 1. or 2. in \definizione~\ref{def:leq}, are analogous to the correspondent cases of \Lemma~\ref{lemmadue}. If $\node_{i} \dot{<} \node_{j}$ for 3. in \definizione~\ref{def:leq}, then $\exists l. ch_l[\node_i] \dot{<} ch_l[\node_j]$ and $\exists m. ch_m[\node_j] \dot{<} ch_m[\node_k]$. If $l=m$ the thesis follows by inductive hypothesis. 
% If $l>m$ then $\neg(ch_m[\node_i] \dot{<}ch_m[\node_j])$; if $l<m$ then $ch_l[\node_j] \dot{<} ch_l[\node_k]$. In both cases we can apply  \Lemma~\ref{lemmadue} to conclude the thesis. 
% % If $l<m$ then $ch_l[\node_j] \dot{<} ch_l[\node_k]$ \Lemma~\ref{lemmadue} can be applied to $ch_l[\node_i]$ . 
% %  
% % If $l<m$ then $ch_l[\node_i] \dot{<} ch_m[\node_j]$ since the sequence of children of $\node_j$ has been formed by repeatedly selecting the minimal element. 
% % 
% % 
% % Let us assume, by contradiction, that $\neg(\node_{i} \dot{<} \node_{k}) \wedge \neg(\node_{k} \dot{<} \node_{i})$. If $\node_{i} \dot{<} \node_{j}$ for 1. in \definizione~\ref{def:leq}, then $L(\node_k)<L(\node_j)$ and $\node_{k} \dot{<} \node_{j}$, which contradicts the hypothesis. If $\node_{i} \dot{<} \node_{j}$ for 2., then $\rho(\node_k)<\rho(\node_j)$ and $\node_{k} \dot{<} \node_{j}$. Finally, if $\node_{i} \dot{<} \node_{j}$ for 3., then $\exists l. ch_l[\node_i] \dot{<} ch_l[\node_j]$. By inductive hypothesis $ch_l[\node_k] \dot{<} ch_l[\node_j]$. 
% % 
% % By L{\scriptsize EMMA}~\ref{lemmamapping}, if $\node_{i} \dot{<} \node_{j} \wedge \node_{j} \dot{<} \node_{k} \Rightarrow S(\node_{i}) < S(\node_{j}) \wedge  S(\node_{j}) < S(\node_{k})$, which implies that $S(\node_{i}) < S(\node_{k}) \Rightarrow \node_{i} \dot{<} \node_{k}$.~\fbox{~\!\!}
% \end{itemize}
%  \end{proof}
% 
% 
% In order to ease the discussion on the properties of the ordering in \definizione~\ref{def:leq}, a unique representation of subtrees is introduced. In \cite{Vishwanathan2003} an injective mapping from subtrees to strings is presented. Here we modify such mapping by employing perfect hash functions. As a consequence we obtain a compressed subtree representation, which will also later be used in section~\ref{sec:hash}: 
% % It resembles the injective mapping in \cite{Vishwanathan2003}, although we choose to employ perfect hash functions to compactely represent subtrees, since we will also make use of them in section~\ref{sec:hash}: 
% \begin{definition}
%  \label{def:mapping}
% let $\#,],[\notin \cal{A}$ be symbols never appearing in any node label and let us assume the vertices of a DAG are ordered according to definition~\ref{def:leq}. If $\node$ is a leaf node, its encoding is $h(L(\node))$, otherwise $\node$ is encoded as $$h(L(\node))\big[ h(ch_1[\node])\#h(ch_2[\node])\ldots\#h(ch_{\rho(\node)}[\node])\big].$$  
% % $h(L(\node))\cdot\big[\prod_{j=1}^{\rho(\node)}\#\cdot h(ch_j[\node])\big]$, where '$\cdot$' is the concatenation operator and '$\prod$' represents the application of '$\cdot$' to an indexed sequence of arguments. 
% \end{definition}
% % By exploiting \definizione~\ref{def:leq}, \definizione~\ref{def:mapping}, and the recursive application of \Lemma~\ref{lemmaeq}, 
% We can now prove the following lemma
%   \begin{lemma} Let $>$ and $=$ be the natural relations of order and equivalence between alphanumeric strings, then the following statements are true
%     \label{lemmamapping}
%     \begin{description}
%     \item i) $\neg(\node_{j} \dot{<} \node_{k}) \wedge \neg(\node_{k} \dot{<} \node_{j})$ if and only if $h(\node_{j}) = h(\node_{k})$.
%     \item ii) $\node_{j} \dot{<} \node_{k}$ if and only if $h(\node_{j}) < h(\node_{k})$;
%     \end{description}     
%     \end{lemma} 
%     \begin{proof}
%     {\it i)} The proof is done by induction. $\Rightarrow)$ Since the mapping in \definizione~\ref{def:mapping} is injective, we need to show that the input of the encoding function is identical. If $\node_j, \node_k$ are leaf nodes, then $h(\node_j)=h(\node_k)$ by \Lemma~\ref{lemmaeq}; otherwise, by inductive hypothesis $\forall 1\leq l\leq \rho(\node_j)=\rho(\node_k). h(ch_l[\node_j])=h(ch_l[\node_k])$, thus the encoding for non leaf nodes in \definizione~\ref{def:mapping} again ensures that $h(\node_j)=h(\node_k)$ (see the proof in \cite{Vishwanathan2003} for details). 
%     $\Leftarrow)$ If the encoding of $\node_j$ and $\node_k$ is identical, then $L(\node_j)=L(\node_k)$ and the thesis follows by \Lemma~\ref{lemmaeq} for leaf nodes; if $\node_j, \node_k$ are not leaf nodes, by inductive hypothesis $\forall 1\leq l\leq \rho(\node_j)=\rho(\node_k). \neg(ch_l[\node_{j}] \dot{<} ch_l[\node_{k}]) \wedge \neg(ch_l[\node_{k}] \dot{<} ch_l[\node_{j}])$ and thus the thesis follows again by \Lemma~\ref{lemmaeq}. \\
%     {\it ii)} $\Rightarrow)$ If $\node_{j} \dot{<} \node_{k}$ for rule 1. or 2. in \definizione~\ref{def:leq} 
% 
% % 
% % the fact that the symbol $\#$ can not be found in any node label ensures that different child sequences can not be the same input to $h()$. Therefore, being $h()$ injective implies that if $\neg(\node_{j} \dot{<} \node_{k}) \wedge \neg(\node_{k} \dot{<} \node_{j})$ then $h(\node_{j}) = h(\node_{k})$ by recursive 
% %      application of L{\scriptsize EMMA}~\ref{lemmaeq} ( 
% % if $S(\node_{j}) = S(\node_{k})$ then neither $\node_{j} \dot{<} \node_{k}$ nor $\node_{k} \dot{<} \node_{j}$ can hold, otherwise
% %      there will exist a position where $S(\node_{j})$ and  $S(\node_{k})$ differ, which is in contradiction with the hypothesis.\\
%     {\it ii)}: Let us assume that $\node_{j} \dot{<} \node_{k}$ then
% if 1. or 2. applies, we have $[L(\node_{j}) < L(\node_{k})] \vee [outdeg(\node_{j}) < outdeg(\node_{k})]$ which, by Definition~\ref{def:mapping}, entails that $S(\node_{j}) < S(\node_{k})$;
% if 3. must be applied, then \mbox{$S(\node_{j})= L \cdot m \cdot \left(\prod_{i=1}^{m}S(ch_{i}[\node_j])\right)$} and \mbox{$S(\node_{k})= L \cdot m \cdot \left(\prod_{i=1}^{m}S(ch_{i}[\node_k])\right),$} where $L=L(\node_j)=L(\node_k)$ and $m = outdeg(\node_{j}) = outdeg(\node_{k})$. Moreover, let $l$ be the value of
%     the index for which 3. applies. Then, by {\it i)}, we have $\prod_{i=1}^{l-1}S(ch_{i}[\node_j]) = \prod_{i=1}^{l-1}S(ch_{i}[\node_k])$ and the above arguments
%     can be recursively applied to
%     $ch_{l}[\node_j] \dot{<} ch_{l}[\node_k]$, eventually till only vertices with $0$ out-degree are reached. For those vertices, only 1. or 2. may apply, which leads 
%     to the desired result.\\
%     Viceversa, if  $S(\node_{j}) < S(\node_{k})$, let $q$ be the first position where the two strings differ, i.e. $pos(q,S(\node_{j})) < pos(q,S(\node_{k}))$, then it is easy to see that that position
%     corresponds to the first application of 1. (i.e. $pos(q,S(\node_{j}))$ and $pos(q,S(\node_{k}))$ are labels) or 2. (i.e. $pos(q,S(\node_{j}))$ and $pos(q,S(\node_{k}))$ are out-degrees) after having only applied 3. (possibly $0$ times if $q<3$), which entails that $\node_{j} \dot{<} \node_{k}$. 
%     \end{proof}
% 
% 
%  \begin{definition}
%  \label{def:mappingold}
%  Given a vertex $\node$, the following alphanumeric string $S(\node)$ is associated to it:
% \[S(\node)=L(\node)\cdot outdeg(\node)\cdot \left(\prod_{i=1}^{outdeg(v)}S(ch_{i}[\node])\right)\]
% where '$\cdot$' is the concatenation operator and '$\prod$' represents the application of
% '$\cdot$' to an indexed sequence of arguments; moreover, the order adopted for the children of a node
% is the same order defined in Definition~\ref{def:leq}.
%  \end{definition}
% By exploiting Definition~\ref{def:leq}, Definition~\ref{def:mapping}, and the recursive application of L{\scriptsize EMMA}~\ref{lemmaeq}, we can now prove the following lemma
%   \begin{lemma} Let $>$ and $=$ be the natural relations of order and equivalence between alphanumeric strings, then the following statements are true
%     \label{lemmamappingold}
%     \begin{description}
%     \item i) $\neg(\node_{j} \dot{<} \node_{k}) \wedge \neg(\node_{k} \dot{<} \node_{j})$ if and only if $S(\node_{j}) = S(\node_{k})$.
%     \item ii) $\node_{j} \dot{<} \node_{k}$ if and only if $S(\node_{j}) < S(\node_{k})$;
%     \end{description}     
%     \end{lemma} 
%     \begin{proof}
%     {\it i)}:
% %     \begin{description}
% %     \item 
% if $\neg(\node_{j} \dot{<} \node_{k}) \wedge \neg(\node_{k} \dot{<} \node_{j})$ then $S(\node_{j}) = S(\node_{k})$ by recursive 
%      application of L{\scriptsize EMMA}~\ref{lemmaeq};
% %     \item 
% if $S(\node_{j}) = S(\node_{k})$ then neither $\node_{j} \dot{<} \node_{k}$ nor $\node_{k} \dot{<} \node_{j}$ can hold, otherwise
%      there will exist a position where $S(\node_{j})$ and  $S(\node_{k})$ differ, which is in contradiction with the hypothesis.\\
% %     \end{description}
%     {\it ii)}: Let us assume that $\node_{j} \dot{<} \node_{k}$ then
% %    \begin{description}
% %    \item 
% if 1. or 2. applies, we have $[L(\node_{j}) < L(\node_{k})] \vee [outdeg(\node_{j}) < outdeg(\node_{k})]$ which, by Definition~\ref{def:mapping}, entails that $S(\node_{j}) < S(\node_{k})$;
% %    \item 
% if 3. must be applied, then \mbox{$S(\node_{j})= L \cdot m \cdot \left(\prod_{i=1}^{m}S(ch_{i}[\node_j])\right)$} and \mbox{$S(\node_{k})= L \cdot m \cdot \left(\prod_{i=1}^{m}S(ch_{i}[\node_k])\right),$} where $L=L(\node_j)=L(\node_k)$ and $m = outdeg(\node_{j}) = outdeg(\node_{k})$. Moreover, let $l$ be the value of
%     the index for which 3. applies. Then, by {\it i)}, we have $\prod_{i=1}^{l-1}S(ch_{i}[\node_j]) = \prod_{i=1}^{l-1}S(ch_{i}[\node_k])$ and the above arguments
%     can be recursively applied to
%     $ch_{l}[\node_j] \dot{<} ch_{l}[\node_k]$, eventually till only vertices with $0$ out-degree are reached. For those vertices, only 1. or 2. may apply, which leads 
%     to the desired result.\\
%     Viceversa, if  $S(\node_{j}) < S(\node_{k})$, let $q$ be the first position where the two strings differ, i.e. $pos(q,S(\node_{j})) < pos(q,S(\node_{k}))$, then it is easy to see that that position
%     corresponds to the first application of 1. (i.e. $pos(q,S(\node_{j}))$ and $pos(q,S(\node_{k}))$ are labels) or 2. (i.e. $pos(q,S(\node_{j}))$ and $pos(q,S(\node_{k}))$ are out-degrees) after having only applied 3. (possibly $0$ times if $q<3$), which entails that $\node_{j} \dot{<} \node_{k}$.~\fbox{~\!\!} 
% %    \end{description}
%     \end{proof}
% %The above lemma can be used to prove the following two lemmas
% %  \begin{lemma}
% %    \label{lemmaordering}
% %     If $\node_{i} \dot{<} \node_{j} \wedge \neg(\node_{j} \dot{<} \node_{k}) \wedge \neg(\node_{k} \dot{<} \node_{j})$ then 
% %     $\node_{i} \dot{<} \node_{k}$. 
% %     \end{lemma}  
% %  \begin{lemma}
% %    \label{corollaryordering}
% %      if $\neg(\node_{i} \dot{<} \node_{j}) \wedge \neg(\node_{j} \dot{<} \node_{i}) \wedge \node_{j} \dot{<} \node_{k}$ then $\node_{i} \dot{<} \node_{k}$.
% %  \end{lemma}
% 
% 
%  \begin{theorem}
%   \label{teo:orderingwelldefinedold}
%  The relation just defined is a strict partial order between DAG vertices.
%  \end{theorem}
%   
%  \begin{proof}
%  A strict partial order is a relation on a set $P$ that is irreflexive, asymmetric and transitive. 
%   In the following each property is proven.
% \begin{itemize}
%   \item \textit{Irreflexivity}: $\neg(\node_{i} \dot{<} \node_{i})$, i.e. no condition in Definition.~\ref{def:leq} is satisfied by the pair $(\node_i, \node_i)$:
%   since $\node_{i}$ is mapped into $S(\node_{i})$, L{\scriptsize EMMA}~\ref{lemmamapping}.{\it ii)} applies and thus $\neg(\node_{i} \dot{<} \node_{i})$;
% \item \textit{Asymmetry}: ($\node_{i} \dot{<} \node_{j}  \Rightarrow \neg \node_{j} \dot{<} \node_{i}$).
% By L{\scriptsize EMMA}~\ref{lemmamapping}, if $\node_{i} \dot{<} \node_{j}$ then $S(\node_{i}) < S(\node_{j})$, which is not consistent with the condition $S(\node_{j}) < S(\node_{i})$ required by $\node_{j} \dot{<} \node_{i}$.
%  \item \textit{Transitivity} ($\node_{i} \dot{<} \node_{j} \wedge \node_{j} \dot{<} \node_{k} \Rightarrow \node_{i} \dot{<} \node_{k}$). 
% By L{\scriptsize EMMA}~\ref{lemmamapping}, if $\node_{i} \dot{<} \node_{j} \wedge \node_{j} \dot{<} \node_{k} \Rightarrow S(\node_{i}) < S(\node_{j}) \wedge  S(\node_{j}) < S(\node_{k})$, which implies that $S(\node_{i}) < S(\node_{k}) \Rightarrow \node_{i} \dot{<} \node_{k}$.~\fbox{~\!\!}
% \end{itemize}
%  \end{proof}

We now show that if two DAGs $DD_{G_1}^{\node_i}$ and $DD_{G_2}^{\node_j}$ are isomorphic, then the root nodes of the DAGs are not comparable with respect to the ordering in \definizione{\ref{def:leq}}: 
\begin{theorem} \label{teo:dagisomorfi}
	if two DAGs $DD_{G_1}^{\node_i}$ and $DD_{G_2}^{\node_j}$ are isomorphic, then $\neg(\node_i \dot{<} \node_j) \wedge \neg(\node_j \dot{<} \node_i)$. 
\end{theorem}
\begin{proof}
  Let \mbox{$f: V_{G_1} \rightarrow V_{G_2}$} be an isomorphism between $DD_1^{\node_i}$ and $DD_2^{\node_j}$. 
%   Since $DD_1^{\node_i}$ and $DD_2^{\node_j}$ are isomorphic, there exists a function \mbox{$f: V_{G_1} \rightarrow V_{G_2}$}. 
  We prove the thesis by induction. Let $f(\node_i)=\node_j$, since the nodes are isomorphic $L(\node_i)=L(\node_j)$. If $\node_i$ and $\node_j$ are leaf nodes, then $\hash(\node_i)=\hash(\node_j)$ and consequently $\neg(\node_i \dot{<} \node_j) \wedge \neg(\node_j \dot{<} \node_i)$. Otherwise, by inductive hypothesis $\forall l. 1\leq l\leq \rho(\node_i).$  $\hash(ch_{\node_i}[l])=\hash(ch_{f(\node_i)}[l])$ and $L(\node_i)=L(f(\node_i))$, thus $\hash(\node_i)=\hash(f(\node_i))=\hash(\node_j)$. 
\end{proof}

In the following, we will denote as $ODD^{\node_{i}}_{G}$ the Decompositional Dag rooted at $\node_i$ and ordered according to \definizione{\ref{def:leq}}. 
If the $\hash()$ values are computed according to a post order visit of the DAG, then the values $\hash(ch_{\node}[l])$ for $1\leq l\leq \rho(\node)$ are already available for computing $\hash(\node)$. Thus the time complexity of the ordering phase of the DAG is $O(|V| \rho\log \rho)$ where the term $\rho\log \rho$ accounts for the ordering of the children of each node. 

The reason for defining the ordering according to \definizione{\ref{def:leq}} is that it must be efficient to compute and must ensure that the swapping of non comparable nodes does not affect the feature space representation of the DAG. After introducing the extension of tree kernels to DAGs in Section~\ref{sec:treekernelsfordags}, we will show that our ordering meets both constraints. 
% The remainder of this section introduces concepts and prove results needed in Section~\ref{sec:treekernelsfordags}. 
 
% More ''standard'' orderings would not meet both constraints. For example, a total order between DAG vertices would require an algorithm with GI-COMPLETE computational complexity \cite{}. On the contrary, simple partial orderings, as the one based on reachability of the nodes, would not allow us to consistently order structurally different subdags, thus making impossible to have a consistent mapping in feature space for any kernel whose features are defined according to such structures (which basically includes most convolution kernels, as we will show in section \ref{sec:treekernelsfordags}).
%
%In the following we prove a result that we will use in section \ref{sec:treekernelsfordags} to show that the ordering of definition \ref{def:leq} allows a consistent application of convolution kernels to the DAG domain.
% % Let a tree visit be a function $T(\node_i)$ that, given a node $\node$ of a $ODD^{\node_{i}}_{G}$, returns the tree resulting from the visit of the DAG starting from $\node_{i}$. 
% % Figure~\ref{fig:treevisit} gives an example of tree visits. Note that the trees resulting from the visit starting in node \textbf{s} are identical for the DAGs in Figure~\ref{fig:treevisit}-a and Figure~\ref{fig:treevisit}-b even if the DAGs are not isomorphic. However, the DAGs in Figure~\ref{fig:treevisit}-a and Figure~\ref{fig:treevisit}-b can be discriminated if we consider the multiset of trees returned by the tree visits starting in all nodes of the DAGs: one tree is produced by the visit starting in node \textbf{d} of the DAG in Figure~\ref{fig:treevisit}-a and two trees are generated by the two visits starting in the nodes labelled with \textbf{d} in Figure~\ref{fig:treevisit}-b. 
% % %  but only  for : the tree resulting from the visit starting in node \textbf{s} has two leaf nodes \textbf{d}, while the $T()$ related to the DAG of Figure~\ref{fig:treevisit}-b) has associated twice the tree composed of only the leaf node \textbf{d}. 
% % Moreover, note that the set of tree visits would be different even if the nodes labelled with \textbf{d} were not leaves. The concept of tree visit is used in the following 
% \begin{theorem} \label{teo:visits}
% 	$\neg(\node_i \dot{<} \node_j) \wedge \neg(\node_j \dot{<} \node_i)$ according to \definizione~\ref{def:leq} if and only if 
% 	 $T(\node_i)$ and $T(\node_j)$, obtained as visits of the subdags rooted at $\node_i$ and $\node_j$, are identical.
% \end{theorem}
% \begin{proof}
%  If $\neg(\node_i \dot{<} \node_j) \wedge \neg(\node_j \dot{<} \node_i)$ then $\hash(\node_i)\geq \hash(\node_j) \wedge \hash(\node_j)\geq \hash(\node_j) \Leftrightarrow \hash(\node_i)=\hash(\node_j)$. Recalling that $\kappa()$, the function on which $\hash()$ is baesd on, is a perfect hash function, we prove the thesis by induction. If $\node_i, \node_j$ are leaf nodes, then $\hash(\node_i)=\hash(\node_j)\Leftrightarrow L(\node_i)=L(\node_j)$. If $\node_i, \node_j$ are not leaf nodes, then $\forall 1\leq l\leq \rho(\node_i)$ $T(ch_l[\node_i])$ is identical to $T(ch_l[\node_j])$ for inductive hypothesis, and then it must be $L(\node_i)=L(\node_j)$ since $\hash(\node_i)=\hash(\node_j)$; therefore $T(\node_i)$ is identical to $T(\node_j)$. 
% %  We prove the thesis by induction. If $\node_i, \node_j$ are leaf nodes, then $L(\node_i)=L(\node_j)$ for \Lemma~\ref{lemmaeq}. If $\node_i, \node_j$ are not leaf nodes, then $L(\node_i)=L(\node_j)$, $\rho(\node_i)=\rho(\node_j)$ for \Lemma~\ref{lemmaeq} and $\forall 1\leq l\leq \rho(\node_i)$ $ch_l[\node_i]$ is identical to $ch_l[\node_j]$ for inductive hypothesis; therefore $\node_i$ is identical to $\node_j$. 
% \end{proof}

% 
% \begin{theorem} \label{teo:visitsold}
% 	If $\neg(\node_i \dot{<} \node_j) \wedge \neg(\node_j \dot{<} \node_i)$ according to Definition~\ref{def:leq}, then the trees $T(\node_i)$ and $T(\node_j)$, obtained as visits of the subdags rooted at $\node_i$ and $\node_j$, are identical. 
% \end{theorem}
% \begin{proof}
% if $\neg(\node_i \dot{<} \node_j) \wedge \neg(\node_j \dot{<} \node_i)$, by L{\scriptsize EMMA}~\ref{lemmamapping} $S(\node_i)=S(\node_j)$. Moreover, it is not difficult to
% see that for any vertex $\node$, $S(\node)$ is an unambiguous representation of $T(\node)$ where the labels of the visited vertices are presented according to a depth
% visit of $T(\node)$ (remember that vertices are ordered according to the same relation $\dot{<}$) along with the out-degree of each vertex, which allows the
% correct reconstruction of $T(\node)$. Because of that, and since $S(\node_i)=S(\node_j)$, we deduce that $T(\node_i)$ and $T(\node_j)$ are identical.~\fbox{~\!\!}
% \end{proof}



==> speedingupthekernel.tex <==
% \subsection{Speeding up the kernel} \label{sec:bigdag}
\subsection{Speeding up the single kernel evaluation} \label{sec:bigdag}
%As we saw in the previous section, the computational complexity of the ODD kernels depends hardly on the DAG kernel we decide to use. In the instantiations we take into consideration, the complexity is around $O(n^{4})$ .
%
%We can apply various techniques to reduce the computational time required in practice, and to limit the theoretical complexity.
%
%We used various approaches, obtaining good practical results.
%
%
We now show how to speed up the computation of eq.~\eqref{eq:convolutiondagkernel} when $K_T$ is a convolution kernel where the input tree is decomposed into proper subtrees. All the kernels described in Section~\ref{sec:kernelsfortrees} and the vast majority of tree kernels defined in literature meet this constraint. 
The strategy for speeding up kernel computation is based on avoiding to recompute $C()$ values for identical proper subtrees appearing in different DAGs. 
The $|V_G|$ Decompositional DAGs generated according to the procedure described in Section~\ref{sec:odd} can be represented by a single Annotated DAG, named $BigDAG$, where each node is annotated with the frequency of appearance of the proper subtree rooted at $\node$, i.e. $T(\node)$, in all the ODDs of the graph. An example of $BigDAG$ construction is shown in Figure~\ref{fig:bigdag}. In the figure, the subtree rooted in $\textbf{b}$ in the two graphs are merged together in the $BigDAG$ since all of their descendant nodes, i.e. $\textbf{c}$, are identical. Note that, on the contrary, the nodes labelled with $\textbf{a}$ are not merged together because, in one case the second child of $\textbf{a}$ is $\textbf{d}$ and in the other the second child is the subtree rooted at $\textbf{c}$. 
\begin{figure}[ht]
\centering
\begin{tikzpicture}[auto,thick,scale=.5]
\tikzstyle{label} = [rectangle, fill=white!100, ultra thick, draw=black!80,
            minimum height=60mm, minimum width=4cm,outer sep=0pt]
   \tikzstyle{node}=[minimum size=12pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
  \small
	 \draw [red,->,line width=5pt] (-15cm,-1.5)--(-13.5cm,-1.5);
    \node [node, xshift=-8.4cm] {\textbf{a}} [->] %[->, ultra thick]
                child {
                    node [node] {\textbf{b}}[] 
                    child {node (d2)[node, xshift=0.35cm]{\textbf{c}}[]}
                }
                child {
                    node (b2) [node]{\textbf{d}}[]
                };
%  	 \node [yshift=-0cm, xshift=-10.4cm] {a)};
       \node [node, xshift=-10.4cm, yshift=-0cm] (A2) {\textbf{a}} [->] %[->, ultra thick]
                child {
                    node [node] {\textbf{b}}[] 
                    child {node (d2)[node, xshift=0.0cm]{\textbf{c}}[]}
                }
                child {
                    node (b2) [node]{\textbf{c}}[]
                    child {node (d3)[node, xshift=0.0cm]{\textbf{d}}[]}
                };
        ;     
    \node [node, xshift=-5.4cm](ABIG) {\textbf{a}} [->] %[->, ultra thick]
                child {
                    node [node] (B1BIG){\textbf{b}}[] 
                    child {node (C1BIG)[node, xshift=0.35cm]{\textbf{c}}[]}
                }
                child {
                    node (DBIG) [node, right, xshift=0.6cm] at (C1BIG){\textbf{d}}[]
                }
				;

\node [node, xshift=-4.5cm] (aBIG){\textbf{a}} [->] %[->, ultra thick]
                child {
                    node [node](CBIG) {\textbf{c}}[] 
	      };

         \draw [->]
        (CBIG) to (DBIG)
        ;
   \draw [->]
        (aBIG) to (B1BIG)
        ;
	    \node [above, right, xshift=0.2cm] at (ABIG) {1};
	    \node [above, right, xshift=0.2cm] at (aBIG) {1};
	    \node [above, right, xshift=0.2cm] at (B1BIG) {2};
	    \node [above, right, xshift=0.2cm] at (C1BIG) {2};
	    \node [above, right, xshift=0.2cm] at (DBIG) {2};
	    \node [above, right, xshift=0.2cm] at (CBIG) {1};
\end{tikzpicture}
\caption{Two DAGs (left) and their associated $BigDAG$. Numbers on the right of the nodes represent their frequencies.\label{fig:bigdag}}
\end{figure}
The algorithm for computing the $BigDAG$ can be found in~\cite{Aiolli2006}. Its complexity is $O(|V_G|^2\log |V_G|)$, thus it does not affect the worst-case complexity of any of the kernels considered in the paper. 
The kernel of eq.~\eqref{eq:convolutiondagkernel} can be rewritten as 
\begin{equation} \label{eq:bigdag}
K_{K_T}(G_1,G_2) = \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\sum_{\substack{u_1 \in V(BigDAG(G_1)) \\u_2 \in V(BigDAG(G_2))}}\!\!\!\!\!\!\!\!\!\!\!\!\!\! f_{u_1} f_{u_2} C(u_1,u_2),
\end{equation}
where $f_u$ is the frequency of the ordered DAG rooted at $u$ in $ODD(G)$. 
We want to stress the fact that the $BigDAG$ does not loose any information about the ODDs, thus eq.~\eqref{eq:bigdag} and eq.~\eqref{eq:convolutiondagkernel} are equivalent. 
The speed up due to the $BigDAG$ depends on the number of identical substructures found in the ODDs. 
We now derive an upper bound on the number of nodes of the $BigDAG$ in terms of the in-degree of the nodes and the size of the cycles in the original graph $G$. 
We first derive the bound for a specific class of graphs and then extend it to general graphs. 

Without loss of generality, we will assume in the following to deal with connected and undirected graphs.  
Let's consider a polytree $P$, i.e. a graph for which at most one undirected path exists between any two nodes. 
Let us consider any node $\node_i \in P$ with degree $\rho(\node_i)$. The procedure for obtaining a Decompositional DAG, when applied to all the nodes of
$P$, generates exactly $\rho(\node_i)+1$ different patterns of connectivity for $\node_i$. In fact, since $P$ is a polytree,
only $1$ edge at a time can be entering $\node_i$ while all the remaining edges are outgoing. Moreover, we have to consider the case
where $\node_i$ is the starting node for the visit and all the edges are outgoing. 
These considerations are valid for all nodes belonging to
$P$, thus $BigDAG$ will exactly have $\sum_{i=1}^{|P|}(\rho(\node_i)+1)$ nodes.

Let's now turn our attention to general graphs. Given a graph $G$ we can represent it as a polytree $P(G)$ by iteratively grouping the nodes forming local cycles into a single node $\upsilon\in P(G)$ until no more cycles can be grouped (see Figure~\ref{fig:polytree} for an example). Let us define $n_{\upsilon_i}$ as the number of nodes of $G$ represented by $\upsilon_i$ in $P(G)$ and $q=|P|$. The values $\rho(\upsilon_i)$ represent now the sum of the incoming edges of all the nodes represented by $\upsilon_i$. 
Then, the bound can be computed by applying the same reasoning for polytrees, the only difference being that $\upsilon_i$ contains $n_{\upsilon_i}$ choices for starting the visit from a node ``inside'' $\upsilon_i$, thus generating $n_{\upsilon_i}$ different substructures with, in the worst case of a single cycle involving all the nodes of $G$ represented by $\upsilon_i$, a total of $n_i^2$ nodes added to the $BigDAG$. 
The number of nodes added to the $BigDAG$ is thus bounded by:
\begin{equation}
	|BigDAG(G)| \leq \sum_{i=1}^{q} (\rho(\upsilon_i) + n_{\upsilon_i}^{2}).
	\label{eq:bigdagnodes}
\end{equation}
Note that $|BigDAG(G)| \leq |V_G|^2$, being the worst case when there's only one cycle of length $|V_G|$. 
Let us define the length of the longest cycle in $G$ to be $o$. The bound then becomes $o|V_G|+\sum_i \rho(\upsilon_i)$, since $\sum_i n_{\upsilon_i}=|V_G|$. Note that $\sum_i \rho(\upsilon_i)\leq 2q$ otherwise $P(G)$ wouldn't be a polytree. Just to give an example, if $o=|V_G|^{\frac{1}{2}}$, then $|BigDAG(G)| \leq 2q+\sum_i n_{\upsilon_i} n_{\upsilon_i}\leq 2q+|V_G|^{\frac{1}{2}}\sum_i n_{\upsilon_i}=2q+|V_G|^{\frac{3}{2}}$. 

Note that if the number of nodes in the $BigDAG$ is $O(|V_G|^{\frac{3}{2}}$), then the complexity of the kernels reduces significantly, for example the application of the subset tree kernel would have a complexity of $O(|V_G|^3)$, thus reducing the complexity of a factor $|V_G|$. Section~\ref{sec:exps} will discuss the actual reduction of the computational burden due to the $BigDAG$ on benchmark datasets. 

%Due to the specific process generating the ODDs, a bound on the number of nodes in the BigDAG can be given according to the following 
%\begin{theorem}
%Given a set $ODD_G$ generated from graph $G$, the nodes of the BigDAG are $\sum_{i=1}^{n} (p_{i}+n_{i}^{2})$, where $p_i$ is the in-degree of $\node_i\in G$ and 
%\end{theorem}
%in terms of the in-degree of the nodes and on the size of the cycles. 

%The first technique we applied modify the formulation of the kernel, maintaining the same informations. Instead of generate $n$ DAGs for each graph, each with $n$ nodes, we can maintain the same information in one single annotated DAGs. In this big DAG, every node is associated with a frequency label, that represents the number of times the proper subtree rooted at $\node$ appears in the various ODDs of the graph.
%So with this method, at the end of the decomposition each graph is associated with a single DAG, with at most $n^{2}$ nodes (in the worst case the number of nodes is the same as the sum over all the ODDs). However In the average case, much nodes repeats in more than one DAG and in practical terms we see a high performance improvement.
%
%Following this scheme we have one Big DAG representation for each graph, so we apply the DAG kernel only one time per pair of graphs.
%
%The new formulation of the kernel is the following:
%\[
%K_{BigODD}(G,G') = \sum_{\substack{d \in BigODD(G) \\d' \in BigODD(G')}} frequency_{d}^{G} * frequency_{d'}^{G'} * K_{T}(d,d')
%\]
%where $BigODD(G)$ is the DAG generated for the graph $G$, and $frequency_{d}^{G}$ is the function returning the frequency label associated to the vertex d in the big dag $BigODD(G)$.
%
%This kernel is positive semidefinite because it is equivalent to the kernel $K_{AllODD}$.
%
%In particular there are some classes of graphs for which we can give a closer bound on the number of nodes resulting in the BigDAG.
%
%%\subsection{Bound on the number of vertices for graphs with limited simple cycles length}
%
%Let's consider a particular family of graphs. We will then notice that we will not lose in generality, because every graph can be viewed as a particular instantiation of this family of graphs.
%
%%TODO definition simple cycles
%Let's first define a simple cycle in a graph.
%A \textbf{simple cycle} is a closed (simple) path, with no other repeated vertices or edges other than the starting and ending vertices. 
%
%
%For our bound, let's consider the graphs that can be generated from a particular type of undirected polytree, where each node can be 
%\begin{itemize}
%\item a \textit{single polytree node}, thar represene a vertex of the graph that is not involved in any simple cycle, or 
%\item a \textit{complex polytree node}, that is, a node that represent a set of vertex in the original graph included in one or more simple cycle.
%\end{itemize}
%
%If a node does not appear in any simple cycle, it must be a simple node in our representation.
%If two simple cycles shares some nodes, they will be merged in a single complex node.
%
%With this definition, we will have exactly one (minimal) representation of a graph in this form.
%
%An example that clarify this notation is in figure \ref{fig:poly}.
%
%This polytree structure have $m \leq n$ nodes. Let's associate a multiplicity to every polytree node, indicating the number of vertices of the original graph that are contained in every node (simple or complex). We will call this number $n_{i}$ with $i \in \{ 1 \ldots m \} $. The simple polytree nodes will have $n_{i}=1$.
%
%Every one of these polytree nodes have a degree (the number of edges incident to the vertex) that we will call $p_{i}$.
%
%We now can observe that the structure of the polytree does not permit cycles by definition, so the execution of the visit for the generation of the ODDs can generate a limited number of versions for each node (simple or complex). In particular, for the node $i$, we will have $p_{i}$ versions, one for each selection of the incoming edge, plus the versions starting from a vertex inside the polytree node itself.
%
%For a simple node, there is trivially one version of the node starting from the single vertex in the node.
%For the complex nodes, in the worst case we will have $n_{i}^{2}$ possible versions: in fact, for each of the $n_{i}$ nodes, we can generate $|n_{i}|$ different vertices.
%
%So we will have exactly
%
%\[
%\sum_{i=1}^{m} (p_{i}+n_{i}^{2})
%\] 
%
%vertices in the BigDAG.
%
%We can notice that in the worst case, all vertices of the original graph are collapsed in one single complex node, so the bound on the number of nodes returns to $n^{2}$.
%We can show a better bound, for the class of graphs in which the dimension of the simple cycles of the graph is at most $n^{\frac{1}{2}}$.
%
%In this case the bound is:
%\[
%\sum_{i=1}^{m} (p_{i}+n_{i}^{2}) = \sum_{i=1}^{m} (p_{i}+ \sum_{i=1}^{m} n_{i}^{2}) 
%\]
%
%we can now notice that $\sum_{i=1}^{m} (p_{i}$ can not be greater than $2m$, otherwise we should have cycles, and this is not permitted by the definition of the polytree. So:
%
%\[
% \sum_{i=1}^{m} (p_{i}+ \sum_{i=1}^{m} n_{i}^{2}) \leq  2m + \sum_{i=1}^{m} n_{i}^{2})  = 2m + \sum_{i=1}^{m} n_{i} n_{i}
%\]
%
%now we can use the assumption that $n_{i} \leq n^{\frac{1}{2}}$
%
%\[
%2m + \sum_{i=1}^{m} n_{i} n_{i} \leq 2m + \sum_{i=1}^{m} n^{\frac{1}{2}} n_{i} = 2m+ n^{\frac{1}{2}} \sum_{i=1}^{m} n_{i}
%\]
%
%but $\sum_{i=1}^{m} n_{i}$ is for construction equals to $n$, so
%\[
%2m+ n^{\frac{1}{2}} \sum_{i=1}^{m} n_{i} = 2m+ n^{\frac{1}{2}} n = 2m +n ^{\frac{3}{2}} 
%\]
% where $m \leq n$.
% 
% So the bound on the number of nodes of the BigDAG in this case is $O(n^{\frac{3}{2}} )$.
%
%
%\begin{theorem}
%The \textit{BigDAG ODD} kernel can be calculated on a pair of graphs $G$ and $G'$ where the dimension of the simple cycles of the graphs is at most $n^{\frac{1}{2}}$  in  $O(n^{\frac{3}{2}} \log n^{\frac{3}{2}})$ using the subtree kernel, in $O(n^{3})$ using subset tree kernel and in \textbf{$O(p^{3}n^{3})$} using the partial tree kernel, where $p$ is the maximum out-degree of the vertices of the generated DAGs.
%\end{theorem}
%
%\begin{proof}
%The first step for the kernel computation is to calculate the multistes  $ODDS(G)$ and $ODDs(G')$ using the algorithm  \ref{Algo:ODDs}. To generate a single ODD, we must visit every edge of the original graph, that are at most $m=n^{2}$, so the complexity of this step is $O(n^{2})$. \\
%For the sorting step, we observe that in the worst case we have to sort n sons for each vertex, so the cost is $n \log n$ comparations, and each 
%
%%TODO ordinamento costo
%comparisons cost at most $n$ because we may have to compare all node descendants. So the total cost of the sorting step for a single DAG is $O(n^{}{2} \log n)$. The number of generated DAGs is $n$, so the cost of the entire sorting step is $O(n p^{h+2} \log p)$.\\
%
%At this point we have to calculate the DAG kernel $K_{T}$ for each pair of DAG that we generated starting from $G$ and $G'$. All the possible pairs are $n^{2}$, and every DAG have at most $p^{h+1}$ vertices.
%
%The complexity of this step depends from the complexity of the kernel we use:
%\begin{itemize}
%\item The Subtree kernel has complexity $O(n \log n)$, so the complexity of the step is $O(n^{\frac{3}{2}} \log n^{\frac{3}{2}})$.
%\item The Subset tree kernel has complexity $O(n^{2})$, so the complexity of the step is  $O(n^{3})$.
%\item The Partial tree kernel has complexity $O(p^{3} n^{2})$, so the complexity of the step is  $O(p^{3} n^{3})$.
%
%
%\end{itemize}
%
%So the total complexity of the kernel is bounded from the calculation of the kernel $k_{T}$.
%\end{proof}
%
%
%
\begin{figure}
\centering	
\vspace{0.1in}
\label{fig:poly}
\begin{tikzpicture}[scale=0.6]
   	\tikzstyle{every node}=[minimum size=18pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
          \tikzstyle{node}=[minimum size=18pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
          
           \node (0,0)(s) {s}
        child {
            node (b) {b}
            child{
			node (i) {i}
				child { node (l) {l}
					}	
		}
		child {
		node (m) {m}
		}
        }
        child {
        	node (c)[right =2 of b ] {c}
		child{
			node (e) {e}
				child { node (d) {d}
					}	
		}
		child {
		node (h) {h}
		}
        };
	      \draw [black, dashed] (e)+(0.85,0) circle (2.4cm){}; %%%%%%
	      \draw [black, dashed] (i)+(0.2,0) circle (2.3cm){}; %%%%%%
               	\tikzstyle{every node}=[]
              \node[](label1)[right=0.3 of c] {\small \textit{$\upsilon_{1}$}};
              \node[](label2)[left=0.4 of b] {\small \textit{$\upsilon_{2}$}};
{sec:odd}
    \draw 
    (c) to (h)
    (h) to (d)
    (m) to (l)
    (b) to (l)
    ;
   \node [draw, node,xshift=4.7cm] (s2) {s}[-]
        child {node [node, minimum size=20pt] (v2) {$v_2$}}
	child {node [node, minimum size=20pt, xshift=1cm,yshift=-0.2cm] (v1) {$v_1$}};
  \draw [dashed,->, bend right] (e)+(3.4,0) to (v1);
  \draw [dashed,->, bend left] (i)+(1.8,1.6) to (v2);
% 	};
	
  %  \draw [->]
    %(b) to (d)
    %;
%              \node[] (label1)[copy shadow, right=1 of s,fill=yellow,rotate=10,draw] {\small \textit{level 1}}

%     \node(label0)[right=1.5 of s] {\small \textit{level 0}};
%          \node (label1)[right=1 of e] {\small \textit{level 1}};
%     \node (label2)[ right=1 of d] {\small \textit{level 2}};

\end{tikzpicture}
\caption{Example of a polytree representing a graph with two ``complex'' polytree nodes $\upsilon_{1}$ and $\upsilon_{2}$
representing local cycles.\label{fig:polytree}}
\end{figure}

%\subsection{Limited Ordered Decompositional DAG Kernel for bounded degree graphs}
%
%This kernel is an approximated version of the previous one. Informally, the depth first visit that is performed to create the Decompositional DAGs starting from the graphs in input, is limited to a fixed depth level $h$. This results in a minor complexity of the resulting kernel, that can be expressed in terms of this (constant) factor $h$.
%if we call p the maximum degree of the graph, every Decompositional DAG obtained by this limited decomposition have at most $h$ levels, with at most   $p^{l}$ vertex for each level $l$.
%The maximum number of vertices of each ODD is then $p^{h+1}-1$.
%
%%TODO disegno
%\begin{figure}
%\begin{tikzpicture}[scale=0.7]
%   	\tikzstyle{every node}=[minimum size=18pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
%	   	\tikzstyle{red}=[minimum size=18pt, inner sep=0pt, outer sep=0pt,ball color=red,circle, text=white]
%
%    \node [red](s) {s}
%        child {
%            node [red](b) {b}
%        };
%        
%         \node [red](e) at (0:2){e}   
%         		child { node [red](d) {d}}		
%    ;
%    \draw 
%    (s) to (e)
%    (b) to (e)
%    (b) to (d)
%    (e) to (d)
%    ;
%\end{tikzpicture}
%
%\begin{tikzpicture}[scale=0.7]
%   %	\tikzstyle{every node}=[minimum size=18pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
%    \node[minimum size=18pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white] (s) {d}
%     child[->] {
%            node[minimum size=18pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white] (b) {e}}
%	child[->]{
%	node[minimum size=18pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white] (e) {b}
%		child[->] { node [minimum size=18pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white](d) {s}}
%        };
%        
%    \draw [->]
%    (b) to (d)
%    ;
%%              \node[] (label1)[copy shadow, right=1 of s,fill=yellow,rotate=10,draw] {\small \textit{level 1}}
%
%     \node(label0)[right=1.5 of s] {\small \textit{level 0}};
%          \node (label1)[right=1 of e] {\small \textit{level 1}};
%     \node (label2)[ right=1 of d] {\small \textit{level 2}};
%
%\end{tikzpicture}
%\caption{Example of a graph with $p=2$, and the number of nodes of the limited DAG that that we obtain}
%\end{figure}
%
%The computational complexity of this approximated version of the ODD kernel, that we will call \textit{Limited ODD kernel} is faster than the original kernel.


\subsection{Speeding up the kernel matrix computation} \label{sec:bigbigdag}

When using a kernel method, such as the SVM, the tuning of the hyperparameters through a validation set or through cross-validation is common practice. If the kernel function depends on multiple parameters, 
then it is often more efficient to precompute the kernel matrix of the dataset\footnote{The $i,j$ element of the kernel matrix corresponds to the evaluation of the kernel function on the $i$-th and $j$-th examples of the dataset} than computing the kernel values on demand. Other kernel methods, e.g. KPCA, require the full kernel matrix to be computed.

In this section, we discuss how the computation of the full kernel matrix can be optimized. 
The $BigDAG$ has been used to avoid multiple calculations of kernel values for the same structures in different ODDs. The same idea can be extended to the whole training set avoiding multiple calculations of the kernel values for the same structures in different examples. 
Note that substructures shared by different graphs \textit{should} exist, otherwise the kernel would be extremely sparse for the considered training set, and not worth to be used for learning. 
% In this section, we discuss how the computation of the full kernel matrix, especially when using the \textit{subtree kernel}, can be optimized.
% Specifically, we observe that:
% \begin{enumerate}
% \item the BigDAG idea used to avoid multiple calculations of kernel values for the same structures in different ODDs, can be extended to the whole training set avoiding multiple calculations of the kernel values for the same structures in different examples.
% \item If the \textit{subtree kernel} is used, the method we propose yields an explicit (and compact) feature space representation of the kernel; this fact leads to a very efficient implementation.
% \end{enumerate}
% 
Let's assume that the training set contains $M$ graphs. Then, we can obtain a compact representation of all the $BigDAGs$ coming from the $M$ graphs by applying the same algorithm for building the $BigDAG$ starting from a multiset of ODDs, the only difference being that, while a sub-DAG   in a $BigDAG$ may have a frequency greater than one. 
% Following the same idea introduced in Section~\ref{sec:bigdag}, %where we have shown how a $BigDAG$ constitutes a compact representation of the various $ODDs$ generated from a single graph, we can apply the same idea to 
% we can get a compact representation of all the $BigDAGs$ coming from the $M$ graphs. 
% This way, we can avoid to compute multiple times the contribution to the kernel of substructures shared by several graphs. 
The idea is implemented as follows. An annotated DAG, we call it $Big^{2}DAG$, is created starting from all the $BigDAGs$ generated by the training set, where each different structure is represented only once. A (sparse) vector $F_{v_{i}}$, representing the frequency of the structure rooted at that node in all graphs, is associated to each node of the $Big^{2}DAG$. For example, $F_{v_{i}}[j]$ represents the frequency of the structure rooted at node $v_{i}$ in $BigDAG(G_{j})$. Figure~\ref{fig:big2dag} shows an example of $Big^{2}DAG$ construction.
% As mentioned above, the $Big^{2}DAG$ is an explicit representation of the feature space of the \textit{subtree kernel} described in Section~\ref{sec:kernelsfortrees}. In fact, we can notice that 
While the frequency associated to each node in $BigDAG(G_i)$ is the frequency of the proper subtree rooted at that node in all the ODDs related to the graph $G_i$, in the same way, the vector $F_{u_{i}}$ represents the frequencies of the proper subtree rooted in node $u_i$ in the various training graphs. 
When the graphs $G_i$ and $G_j$ have been used to construct the $Big^{2}DAG$, eq.~(\ref{eq:bigdag}) can be rewritten as: 
\begin{equation}\label{eq:big2dag}
K_{Big^{2}DAG}(G_i,G_j)=\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\sum_{u_1,u_2 \in V(Big^{2}DAG)}\!\!\!\!\!\!\!\!\!\!\!\!\!\! F_{u_1}[i]*F_{u_2}[j]* C(u_1,u_2). 
\end{equation}
Since eq.~(\ref{eq:bigdag}) corresponds to the entry $i,j$ of the kernel matrix, in order to compute the whole kernel matrix efficiently it is sufficient to construct the $Big^{2}DAG$ from all the graphs in the training set and then apply eq.~(\ref{eq:bigdag}) to any pair of graphs in the training set. 

% If the \textit{subtree kernel} is used, there is a match only between identical subtrees, that is $ C(u_1,u_2) \neq 0 \iff T(u_1) = T(u_2) $, and eq.~(\ref{eq:big2dag}) can be rewritten as:
% \begin{equation}\label{eq:bigbigdagsubtree}
%  K_{Big^{2}DAG}(G_i,G_j)=\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\sum_{u\in V(Big^{2}DAG)}\!\!\!\!\!\!\!\!\!\!\!\!\!\! F_{u}[i]*F_{u}[j] C(u,u)
% \end{equation}
% 
% Exploiting eq.~\eqref{eq:bigbigdagsubtree} leads to a very efficient implementation. In fact, the whole kernel matrix can be computed with a single scan of the $Big^{2}DAG$ nodes. 
%Exploiting this new formula, we can calculate the whole kernel matrix with a single scan of the $Big^{2}DAG$ nodes, leading to a very efficient implementation of the kernel computation.

\begin{figure}
\centering
\begin{tikzpicture}[auto,thick,scale=.5]
\tikzstyle{label} = [rectangle, fill=white!100, ultra thick, draw=black!80,
            minimum height=60mm, minimum width=4cm,outer sep=0pt]
   \tikzstyle{node}=[minimum size=12pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
  \small
	 \draw [red,->,line width=4pt] (-14cm,-1.5)--(-13.2cm,-1.5);
    \node [node, xshift=-10.4cm](ABIG) {\textbf{a}} [->] %[->, ultra thick]
                child {
                    node [node] (B1BIG){\textbf{b}}[] 
                    child {node (C1BIG)[node, xshift=0.35cm]{\textbf{c}}[]}
                }
                child {
                    node (DBIG) [node, right, xshift=0.6cm] at (C1BIG){\textbf{d}}[]
                };
\node [node, xshift=-9.5cm] (aBIG){\textbf{a}} [->] %[->, ultra thick]
                child {
                    node [node](CBIG) {\textbf{c}}[] 
	      };

         \draw [->]
        (CBIG) to (DBIG)
        ;
   \draw [->]
        (aBIG) to (B1BIG)
        ;
         
	    \node [above, right, xshift=0.2cm] at (ABIG) {1};
	    \node [above, right, xshift=0.2cm] at (aBIG) {1};
	    \node [above, right, xshift=0.2cm] at (B1BIG) {2};
	    \node [above, right, xshift=0.2cm] at (C1BIG) {2};
	    \node [above, right, xshift=0.2cm] at (DBIG) {2};
	    \node [above, right, xshift=0.2cm] at (CBIG) {1};
        
 \node [node, xshift=-8.4cm](BBIG2) {\textbf{b}} [->] %[->, ultra thick]
                child {
                    node [node] (C1BIG2){\textbf{c}}[] 
                    child {node (D1BIG2)[node, xshift=0.35cm]{\textbf{d}}[]}
                }
                child {
                    node (CBIG2) [node, right, xshift=0.6cm] at (D1BIG2){\textbf{c}}[]
                }
				;

\node [node, xshift=-7.5cm] (EBIG2){\textbf{e}} [->] %[->, ultra thick]
                child {
                    node [node](B1BIG2) {\textbf{b}}[] 
	      };

         \draw [->]
        (EBIG2) to (C1BIG2)
        ;
   \draw [->]
        (B1BIG2) to (CBIG2)
        ;
         
	    \node [above, right, xshift=0.2cm] at (BBIG2) {1};
	    \node [above, right, xshift=0.2cm] at (C1BIG2) {2};
	    \node [above, right, xshift=0.2cm] at (D1BIG2) {2};
	    \node [above, right, xshift=0.2cm] at (CBIG2) {2};
	    \node [above, right, xshift=0.2cm] at (EBIG2) {1};
	    \node [above, right, xshift=0.2cm] at (B1BIG2) {1};
        
    \node [node, xshift=-6.0cm](ABIGBIG) {\textbf{a}} [->] %[->, ultra thick]
                child {
                    node [node] (B1BIGBIG){\textbf{b}}[] 
                    child {node (C1BIGBIG)[node, xshift=0.35cm]{\textbf{c}}[]}
                }
                child {
                    node (DBIGBIG) [node, right, xshift=1.2cm, yshift=-0.2cm] at (C1BIGBIG){\textbf{d}}[]
                }
				;

\node [node, xshift=-4.7cm] (aBIGBIG){\textbf{a}} [->] %[->, ultra thick]
                child {
                    node [node, yshift=-0.35cm](C2BIGBIG) {\textbf{c}}[] 
	      };
\node [node, xshift=-3.5cm] (BBIGBIG){\textbf{b}} [->] ;%[->, ultra thick]
\node [node, xshift=-3.5cm, yshift=-0.5cm] (EBIGBIG){\textbf{e}} [->] ;%[->, ultra thick]


         \draw [->]
        (C2BIGBIG) to (DBIGBIG)
        ;
   \draw [->]
        (aBIGBIG) to (B1BIGBIG)
        ;
  \draw [->]
        (BBIGBIG) to (C2BIGBIG)
        ;
  \draw [->]
        (EBIGBIG) to (C2BIGBIG)
        ;
         \draw [->]
        (EBIGBIG) to (B1BIGBIG)
        ;  
  \draw [->] (BBIGBIG) to (C1BIGBIG);
	    \node [above, right, xshift=0.2cm] at (ABIGBIG) {[1,0]};
	    \node [above, right, xshift=0.2cm] at (aBIGBIG) {[1,0]};
	    \node [above, right, xshift=0.2cm] at (BBIGBIG) {[0,1]};
	    \node [above, right, xshift=0.2cm] at (EBIGBIG) {[0,1]};
	    \node [above, right, yshift=-0.2cm,xshift=0.2cm] at (C2BIGBIG) {[1,2]};
	    \node [above, right, yshift=-0.2cm,xshift=0.2cm] at (B1BIGBIG) {[2,1]};
	    \node [above, right, xshift=0.2cm] at (C1BIGBIG) {[2,2]};
	    \node [above, right, xshift=0.2cm] at (DBIGBIG) {[2,2]};
\end{tikzpicture}
\caption{Two $BigDAGs$ (left) and their associated $Big^{2}DAG$. Arrays on the right of nodes represent the frequencies associated to each example.\label{fig:big2dag}}
\end{figure}

% \begin{figure}
% \centering
% \begin{tikzpicture}[auto,thick,scale=.5]
% \tikzstyle{label} = [rectangle, fill=white!100, ultra thick, draw=black!80,
%             minimum height=60mm, minimum width=4cm,outer sep=0pt]
%    \tikzstyle{node}=[minimum size=12pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
%   \small
% 	 \draw [red,->,line width=4pt] (-14cm,-1.5)--(-13.2cm,-1.5);
%     \node [node, xshift=-10.4cm](ABIG) {\textbf{a}} [->] %[->, ultra thick]
%                 child {
%                     node [node] (B1BIG){\textbf{b}}[] 
%                     child {node (C1BIG)[node, xshift=0.35cm]{\textbf{c}}[]}
%                 }
%                 child {
%                     node (DBIG) [node, right, xshift=0.6cm] at (C1BIG){\textbf{d}}[]
%                 };
% \node [node, xshift=-9.5cm] (aBIG){\textbf{a}} [->] %[->, ultra thick]
%                 child {
%                     node [node](CBIG) {\textbf{c}}[] 
% 	      };
% 
%          \draw [->]
%         (CBIG) to (DBIG)
%         ;
%    \draw [->]
%         (aBIG) to (B1BIG)
%         ;
%          
% 	    \node [above, right, xshift=0.2cm] at (ABIG) {1};
% 	    \node [above, right, xshift=0.2cm] at (aBIG) {1};
% 	    \node [above, right, xshift=0.2cm] at (B1BIG) {2};
% 	    \node [above, right, xshift=0.2cm] at (C1BIG) {2};
% 	    \node [above, right, xshift=0.2cm] at (DBIG) {2};
% 	    \node [above, right, xshift=0.2cm] at (CBIG) {1};
%         
%  \node [node, xshift=-8.4cm](BBIG2) {\textbf{b}} [->] %[->, ultra thick]
%                 child {
%                     node [node] (C1BIG2){\textbf{c}}[] 
%                     child {node (D1BIG2)[node, xshift=0.35cm]{\textbf{d}}[]}
%                 }
%                 child {
%                     node (CBIG2) [node, right, xshift=0.6cm] at (D1BIG2){\textbf{c}}[]
%                 }
% 				;
% 
% \node [node, xshift=-7.5cm] (EBIG2){\textbf{e}} [->] %[->, ultra thick]
%                 child {
%                     node [node](B1BIG2) {\textbf{b}}[] 
% 	      };
% 
%          \draw [->]
%         (EBIG2) to (C1BIG2)
%         ;
%    \draw [->]
%         (B1BIG2) to (CBIG2)
%         ;
%          
% 	    \node [above, right, xshift=0.2cm] at (BBIG2) {1};
% 	    \node [above, right, xshift=0.2cm] at (C1BIG2) {2};
% 	    \node [above, right, xshift=0.2cm] at (D1BIG2) {2};
% 	    \node [above, right, xshift=0.2cm] at (CBIG2) {2};
% 	    \node [above, right, xshift=0.2cm] at (EBIG2) {1};
% 	    \node [above, right, xshift=0.2cm] at (B1BIG2) {1};
%         
%     \node [node, xshift=-6.0cm](ABIGBIG) {\textbf{a}} [->] %[->, ultra thick]
%                 child {
%                     node [node] (B1BIGBIG){\textbf{b}}[] 
%                     child {node (C1BIGBIG)[node, xshift=0.35cm]{\textbf{c}}[]}
%                 }
%                 child {
%                     node (DBIGBIG) [node, right, xshift=1.2cm] at (C1BIGBIG){\textbf{d}}[]
%                 }
% 				;
% 
% \node [node, xshift=-4.7cm] (aBIGBIG){\textbf{a}} [->] %[->, ultra thick]
%                 child {
%                     node [node](C2BIGBIG) {\textbf{c}}[] 
% 	      };
% \node [node, xshift=-3.5cm] (BBIGBIG){\textbf{b}} [->] ;%[->, ultra thick]
% \node [node, xshift=-3.5cm, yshift=-0.5cm] (EBIGBIG){\textbf{e}} [->] ;%[->, ultra thick]
% 
% 
%          \draw [->]
%         (C2BIGBIG) to (DBIGBIG)
%         ;
%    \draw [->]
%         (aBIGBIG) to (B1BIGBIG)
%         ;
%   \draw [->]
%         (BBIGBIG) to (C2BIGBIG)
%         ;
%   \draw [->]
%         (EBIGBIG) to (C2BIGBIG)
%         ;
%          \draw [->]
%         (EBIGBIG) to (B1BIGBIG)
%         ;  
% 	    \node [above, right, xshift=0.2cm] at (ABIGBIG) {[1,0]};
% 	    \node [above, right, xshift=0.2cm] at (aBIGBIG) {[1,0]};
% 	    \node [above, right, xshift=0.2cm] at (BBIGBIG) {[0,1]};
% 	    \node [above, right, xshift=0.2cm] at (EBIGBIG) {[0,1]};
% 	    \node [above, right, yshift=-0.2cm,xshift=0.2cm] at (C2BIGBIG) {[1,2]};
% 	    \node [above, right, yshift=-0.2cm,xshift=0.2cm] at (B1BIGBIG) {[2,1]};
% 	    \node [above, right, xshift=0.2cm] at (C1BIGBIG) {[2,2]};
% 	    \node [above, right, xshift=0.2cm] at (DBIGBIG) {[2,2]};
% \end{tikzpicture}
% \caption{Two $BigDAGs$ (left) and their associated $Big^{2}DAG$. Arrays on the right of nodes represent the frequencies associated to each example.\label{fig:big2dag}}
% \end{figure}


\subsection{Limiting the depth of the visits} \label{sec:h}
%It is a common practice in many graph kernels (see Section~\ref{sec:relatedwork} and the references therein) to limit in some way, depending on the kernel definition, the features that are generated. Usually this practice is used to limit the computational complexity of the method. It is worth to notice that the computational complexity of our method is very similar to the complexity of other kernels using this kind of limitation (see \cite{Shervashidze2009a}).

It is a common practice in many graph kernels (see Section~\ref{sec:relatedwork} and the references therein) to limit the features that are generated in order to reduce the computational burden when evaluating the kernel. 
 We apply this approach by limiting the depth of the visits during the generation of the multiset of DAGs. % when the tree kernel employed is the \textit{subtree kernel}. 
Our aim is 
\begin{enumerate}
 \item to further reduce the computational complexity of the kernel when large graphs are involved; 
 \item moreover, for some tree kernels, to add features that otherwise would be discarded if only unlimited visits were performed. Examples of such kernels are the \textit{subtree kernel} and the one presented in Section~\ref{sec:noveltk}. 
\end{enumerate}
The above idea is implemented as follows. Given a graph $G$, for any $j \in \{0..h\}$ and for any  $\node_{i} \in V_{G}$, an ODD is generated with the additional constraint that the maximum depth is at most $j$ (we will refer to it as $ODD_{G}^{\node_{i},j}$). All the $ODD_{G}^{\node_{i},j}$ are merged together and form the $BigDAG(G)$ as described in Section~\ref{sec:bigdag}.  
%The method of limiting the depth of the visits consists in fixing an a-priori value $h$ that will be the maximum depth of the visit that is performed to generate the ODDs (see Section~\ref{sec:odd}). That is, given a graph $G$ for any $j \in \{0..h\}$ and for any  $\node_{i} \in V_{G}$, a different ODD is generated (we will refer to it as $ODD_{G}^{\node_{i},h}$), and all these ODDs are merged in the creation of the $BigDAG(G)$ (see Section~\ref{sec:bigdag}).
The kernel definition is the same as in eq.~(\ref{eq:convolutiondagkernel}), the only difference being that $ODD(G)$ is now replaced by $\{ODD_{G}^{\node_{i},j} |  \node_{i} \in V_{G}, j \in \{0\ldots h\} \}$. This kernel is referred to as $K_{ODD-ST_h}$ in the following. 
Notice that, while new features are introduced when kernels such as ST are employed and the visits are limited, all DAGs generated by visits of depth $j>h$ are lost (see Figure~\ref{fig:dd_with_h}). 
% While new features are introduced when the \textit{subtree kernel} is employed and the visits are limited, all DAGs generated by visits of depth $j>h$ are lost (see Figure~\ref{fig:dd_with_h}).
%It is worth to notice that, if the \textit{subtree kernel} is used, this approach introduces new features. In fact, the DAGs generated by visits of depth up to $h$ may not necessarily be included in the set of DAGs generated when performing a complete visit of the graph. On the other hand, all DAGs generated by visits of depth $j>h$ are lost (see Figure~\ref{fig:dd_with_h}).
%TODO figura con le feature mancanti
\begin{figure}
\centering
\begin{tikzpicture}[auto,thick,scale=.5]
   \tikzstyle{graph}=[scale=1.0,minimum size=12pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
		\node (s) [xshift=0.75cm,graph] {s};   
		\node (b) [xshift=0.75cm,yshift=-0.75cm,graph] {b};
    \node (e) [xshift=1.5cm,graph] {e};   
    \node (d) [xshift=1.5cm,yshift=-0.75cm,graph] {d};		
    ;    	
  \small
	 \node [yshift= -0.375cm] {h=0};
	 \node [xshift= 3cm,yshift= -0.375cm] {h=1};
   \tikzstyle{node}=[minimum size=12pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
        \node [node,xshift=4.2cm, yshift=0.75cm] {\textbf{s}} [->] %[->, ultra thick]
                child {
                    node [node] {\textbf{e}}[] 
                }
                child {
                    node (b2) [node]{\textbf{b}}[]
                }
				;
       \node (e) [node,xshift=4.2cm,yshift=-0.75cm] {e}
        		child[->] {
            			node (s) [node] {s}
            			}
						child[->]{
									node (b) [node] {b}
									}
	   				child[->] {
            			node (d) [node] {d}
            			}
        ;
        \node [node,xshift=6.8cm,yshift=0.75cm] {b}
        		child[->] {
            			node [node] {s}
            			}
						child[->]{
									node [node] {e}
									}
	   				child[->] {
            			node [node] {d}
            			}
        ;    
        \node [node,xshift=6.8cm, yshift=-0.75cm] {\textbf{d}} [->] 
                child {
                    node [node] {\textbf{b}}[] 
                }
                child {
                    node (e2) [node]{\textbf{e}}[]
                }
				;
\end{tikzpicture}
\caption{Example of decomposition of the graph shown in Figure~\ref{fig:dagconstruction}-a)  into its DDs with visits up to depth $h=1$.\label{fig:dd_with_h}}
\end{figure}

Given a node, in the worst case no more than $O(\rho^h)$ nodes
are generated by all the visits up to depth $h$. In fact, the total number of generated nodes is 
$$H = \sum_{j=0}^{h}(h+1-j)\rho^j = \frac{(h+1)-(h+2)\rho +\rho^{h+2}}{(1-\rho)^2}.$$ 
Therefore the $BigDAG$ of a graph cannot have more than $nH$ nodes\footnote{It is worth to notice that 
the bound is not tight, since the same leaf nodes are generated in turn by visits of neighbours nodes with depth $0$ and $1$.}. The time complexity of $BigDAG$ creation is thus dominated by a $O(nH\log(nH))$ term. 
If $\rho$ is constant, then $H$ is constant as well and the complexity reduces to $O(n\log n)$. 
Note that limiting the visits allows us to apply the kernel for graphs in eq.~\eqref{eq:convolutiondagkernel} with any tree kernel in Section~\ref{sec:treekernelsfordags} having the same worst case complexity of the corresponding tree kernel: for example, when computing eq.\eqref{eq:convolutiondagkernel} with the \textit{subtree kernel} the total worst case complexity is $O(n\log n)$. 
% 
% Note that, even if we consider the fastest tree kernel among the ones in Section~\ref{sec:treekernelsfordags}, i.e. the \textit{subtree kernel}, which matches the complexity of the
% kernel when using the \textit{subtree kernel}.
% 


==> speedingupthekernelmatrix.tex <==



\begin{figure}
\centering
\begin{tikzpicture}[auto,thick,scale=.5]
\tikzstyle{label} = [rectangle, fill=white!100, ultra thick, draw=black!80,
            minimum height=60mm, minimum width=4cm,outer sep=0pt]
   \tikzstyle{node}=[minimum size=12pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
  \small
	 \draw [red,->,line width=4pt] (-14cm,-1.5)--(-13.2cm,-1.5);
 	% \draw [red,->,line width=5pt] (-14.8,-6.0)--(-12.6,-6.0);
    \node [node, xshift=-10.4cm](ABIG) {\textbf{a}} [->] %[->, ultra thick]
                child {
                    node [node] (B1BIG){\textbf{b}}[] 
                    child {node (C1BIG)[node, xshift=0.35cm]{\textbf{c}}[]}
                }
                child {
                    node (DBIG) [node, right, xshift=0.6cm] at (C1BIG){\textbf{d}}[]
                }
				;

\node [node, xshift=-9.5cm] (aBIG){\textbf{a}} [->] %[->, ultra thick]
                child {
                    node [node](CBIG) {\textbf{c}}[] 
	      };

         \draw [->]
        (CBIG) to (DBIG)
        ;
   \draw [->]
        (aBIG) to (B1BIG)
        ;
         
	    \node [above, right, xshift=0.2cm] at (ABIG) {1};
	    \node [above, right, xshift=0.2cm] at (aBIG) {1};
	    \node [above, right, xshift=0.2cm] at (B1BIG) {2};
	    \node [above, right, xshift=0.2cm] at (C1BIG) {2};
	    \node [above, right, xshift=0.2cm] at (DBIG) {2};
	    \node [above, right, xshift=0.2cm] at (CBIG) {1};

        
 \node [node, xshift=-8.4cm](BBIG2) {\textbf{b}} [->] %[->, ultra thick]
                child {
                    node [node] (C1BIG2){\textbf{c}}[] 
                    child {node (D1BIG2)[node, xshift=0.35cm]{\textbf{d}}[]}
                }
                child {
                    node (CBIG2) [node, right, xshift=0.6cm] at (D1BIG2){\textbf{c}}[]
                }
				;

\node [node, xshift=-7.5cm] (EBIG2){\textbf{e}} [->] %[->, ultra thick]
                child {
                    node [node](B1BIG2) {\textbf{b}}[] 
	      };

         \draw [->]
        (EBIG2) to (C1BIG2)
        ;
   \draw [->]
        (B1BIG2) to (CBIG2)
        ;
         
	    \node [above, right, xshift=0.2cm] at (BBIG2) {1};
	    \node [above, right, xshift=0.2cm] at (C1BIG2) {2};
	    \node [above, right, xshift=0.2cm] at (D1BIG2) {2};
	    \node [above, right, xshift=0.2cm] at (CBIG2) {2};
	    \node [above, right, xshift=0.2cm] at (EBIG2) {1};
	    \node [above, right, xshift=0.2cm] at (B1BIG2) {1};
        





    \node [node, xshift=-6.0cm](ABIGBIG) {\textbf{a}} [->] %[->, ultra thick]
                child {
                    node [node] (B1BIGBIG){\textbf{b}}[] 
                    child {node (C1BIGBIG)[node, xshift=0.35cm]{\textbf{c}}[]}
                }
                child {
                    node (DBIGBIG) [node, right, xshift=1.2cm] at (C1BIGBIG){\textbf{d}}[]
                }
				;

\node [node, xshift=-4.7cm] (aBIGBIG){\textbf{a}} [->] %[->, ultra thick]
                child {
                    node [node](C2BIGBIG) {\textbf{c}}[] 
	      };
\node [node, xshift=-3.5cm] (BBIGBIG){\textbf{b}} [->] ;%[->, ultra thick]
\node [node, xshift=-3.5cm, yshift=-0.5cm] (EBIGBIG){\textbf{e}} [->] ;%[->, ultra thick]


         \draw [->]
        (C2BIGBIG) to (DBIGBIG)
        ;
   \draw [->]
        (aBIGBIG) to (B1BIGBIG)
        ;
  \draw [->]
        (BBIGBIG) to (C2BIGBIG)
        ;
  \draw [->]
        (EBIGBIG) to (C2BIGBIG)
        ;
         \draw [->]
        (EBIGBIG) to (B1BIGBIG)
        ;  

	    \node [above, right, xshift=0.2cm] at (ABIGBIG) {[1,0]};
	    \node [above, right, xshift=0.2cm] at (aBIGBIG) {[1,0]};
	    \node [above, right, xshift=0.2cm] at (BBIGBIG) {[0,1]};
	    \node [above, right, xshift=0.2cm] at (EBIGBIG) {[0,1]};
	    \node [above, right, yshift=-0.2cm,xshift=0.2cm] at (C2BIGBIG) {[1,2]};
	    \node [above, right, yshift=-0.2cm,xshift=0.2cm] at (B1BIGBIG) {[2,1]};
	    \node [above, right, xshift=0.2cm] at (C1BIGBIG) {[2,2]};
	    \node [above, right, xshift=0.2cm] at (DBIGBIG) {[2,2]};
\end{tikzpicture}
\caption{Two $BigDAGs$ (left) and their associated $Big^{2}DAG$. Arrays on the right of nodes represent the frequencies associated to each example.\label{fig:big2dag}}
\end{figure}






\subsection{Speeding up the kernel matrix computation} \label{sec:bigbigdag}

When using a kernel method, such as the SVM, the tuning of the hyperparameters through a validation set or through cross-validation is common practice. If the kernel function depends on multiple parameters,
then it is often more efficient to precompute the kernel matrix of the dataset than computing
the kernel values on demand. Other kernel methods, e.g. KPCA, 
require the full kernel matrix to be computed.

In this section, we discuss how the computation of the full kernel matrix, especially when using the \textit{subtree kernel}, can be optimized.
Specifically, we observe that:
\begin{enumerate}
\item the BigDAG idea used to avoid multiple calculations of kernel values for the same structures in different ODDs, can be extended to the whole training set avoiding multiple calculations of the kernel values for the same structures in different examples.
\item If the \textit{subtree kernel} is used, the method we propose yields an explicit (and compact) feature space representation of the kernel; this fact leads to a very efficient implementation.
\end{enumerate}

Let's assume that the training set contains $M$ graphs. 
Following the same idea introduced in Section~\ref{sec:bigdag}, %where we have shown how a $BigDAG$ constitutes a compact representation of the various $ODDs$ generated from a single graph, we can apply the same idea to 
we can get a compact representation of all the $BigDAGs$ coming from the $M$ graphs. 
This way, we can avoid to compute multiple times the contribution to the kernel of substructures shared by several graphs. Note that these substructures \textit{should} exist, otherwise the kernel
would be extremely sparse for the considered training set, and not worth to be used for learning.

The idea is implemented as follows. An annotated DAG, we call it $Big^{2}DAG$, is created starting from all the $BigDAGs$ generated by the training set, where each different structure is represented only once. A (sparse) vector $F_{v_{i}}$, representing the frequency of the structure rooted in that node in all graphs, is associated to each node of the $Big^{2}DAG$. For example, $F_{v_{i}}[j]$ represents the frequency of structure rooted in node $v_{i}$ in $BigDAG(G_{j})$. Figure \ref{fig:big2dag} shows an example of $Big^{2}DAG$ construction.

As mentioned above, the $Big^{2}DAG$ is an explicit representation of the feature space of the \textit{subtree kernel} described in Section~\ref{sec:kernelsfortrees}. In fact, we can notice that the frequency associated to each node in $BigDag(G_i)$ is the frequency of the proper subtree rooted at that node in all the ODDs related to the graph $G_i$.
In the same way, the vector $F_{u_{i}}$ represents the frequencies of the proper subtree rooted in node $u_i$ in the various training graphs.
So with this new representation,  eq.~(\ref{eq:bigdag}) can be rewritten as:
\begin{equation}\label{eq:big2dag}
K_{Big^{2}DAG}(G_i,G_j)=\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\sum_{u_1,u_2 \in V(Big^{2}DAG)}\!\!\!\!\!\!\!\!\!\!\!\!\!\! F_{u_1}[i]*F_{u_2}[j] C(u_1,u_2)
\end{equation}
If the \textit{subtree kernel} is used, there is a match only between identical subtrees, that is $ C(u_1,u_2) \neq 0 \iff T(u_1) = T(u_2) $, and eq.~(\ref{eq:big2dag}) can be rewritten as:
\begin{equation}\label{eq:bigbigdagsubtree}
 K_{Big^{2}DAG}(G_i,G_j)=\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\sum_{u\in V(Big^{2}DAG)}\!\!\!\!\!\!\!\!\!\!\!\!\!\! F_{u}[i]*F_{u}[j] C(u,u)
\end{equation}

Exploiting eq.~\eqref{eq:bigbigdagsubtree} leads to a very efficient implementation. In fact, the whole kernel matrix can be computed with a single scan of the $Big^{2}DAG$ nodes. 
%Exploiting this new formula, we can calculate the whole kernel matrix with a single scan of the $Big^{2}DAG$ nodes, leading to a very efficient implementation of the kernel computation.






==> treekernels.tex <==
\textcolor{red}{
\section{Kernels for trees} \label{sec:kernelsfortrees}}

\textcolor{red}{This section introduces the convolution tree kernels. As it will be shown in the following sections, they can naturally be extended to be used as kernels for DAGs. The focus of this section is on those kernels employed in the remainder of the paper. 
The convolution kernel framework, as introduced by Haussler \cite{Haussler1999}, describes a general methodology for computing kernels on complex discrete objects. The idea is to split the original object into parts. Assuming that a positive semidefinite kernel on the parts is available, Haussler describes a methodology for combining the local kernels that preserves positive semidefiniteness. In the case of tree structured data most convolution kernels are instances of the following formula: 
$$K(T_1, T_2)=\sum_{\node_1\in T_1}\sum_{\node_2\in T_2}C(\node_1,\node_2),$$ 
where $\node\in T$ is a shorthand for $\node\in V_T$ and $C()$ is the kernel on the parts. In all kernels considered in this section, the parts are composed by proper subtrees, thus $C(\node_1, \node_2)$ is a function counting the number of matching substructures in the proper subtrees rooted at nodes $\node_1$ and $\node_2$. 
By changing the definition of $C()$ many tree kernels can be obtained. %, for example the Subset tree (SST) kernel \cite{Collins2002} and the Subtree (ST) kernel \cite{Vishwanathan2003}. 
% The Partial tree (PT) kernel \cite{Moschitti2006a} counts the number of matching subtrees. 
%  The $C()$ function computing the PT kernel has three cases: \textit{i}) if $\labelfun(\node_1) \neq \labelfun(\node_2)$ then $C_{PT}(\node_1,\node_2)=0$; \textit{ii}) if $\labelfun(\node_1)=\labelfun(\node_2)$ and both $\node_1$ and $\node_2$ are preterminal nodes, i.e. parent of a leaf node, then $C_{PT}(\node_1,\node_2)=\lambda$; \textit{iii}) if $\labelfun(\node_1)=\labelfun(\node_2)$ and either $\node_1$ or $\node_2$ is not a  preterminal node, then 
%  \begin{equation} 
%   \begin{array}{ll}
%  C_{PT}(\node_1,\node_2) = &  \lambda\Big(\mu^2+\displaystyle \sum_{J_1,J_2,|J_1|=|J_2|} \mu^{d(J_1)+d(J_2)}  \\
% & \displaystyle \prod_{i=1}^{|J_1|} \big(1 + C_{PT}(chs_{\node_1}[J_{1i}],chs_{\node_2}[J_{2i}])\big)\Big),
%   \end{array}
%  \end{equation}
% where $J_{11},J_{12},J_{13},\ldots$ $J_{21},J_{22},J_{23},\ldots$ are sequences of indexes associated with the ordered sequences of children $chs_{\node_1}$ and $chs_{\node_2}$ respectively, $J_{1i}$ and $J_{2i}$ point to the $i$-th child in the two sequences and $|J_1|$ denotes the length of the sequence $J_1$. Finally, $d(J_1) = J_{1|J_1|}-J_{11}$ and $d(J_2) = J_{2|J_2|}-J_{21}$. 
% The parameter $\lambda$ penalizes matchings between large trees (if a large tree has a match, then all its subtrees have a match) and $\mu$ penalizes subtrees built on subsequences of children that contain gaps. 
% Its worst-case complexity is $O(\rho^3 |T|^2)$, where $\rho$ is the maximum out-degree of the two trees. 
% 
% Other popular kernels for trees are the Subset tree (SST) kernel \cite{Collins2002} and the Subtree (ST) kernel \cite{Vishwanathan2003}. 
% The feature spaces associated to the kernels are both subsets of the feature space of the PT kernel. 
The SST kernel counts the number of matching subset trees \cite{Collins2002}. The $C()$ function computing the SST kernel has three cases: \textit{i}) if $\labelfun(\node_1) \neq \labelfun(\node_2)$ then $C_{SST}(\node_1,\node_2)=0$; \textit{ii}) if $\labelfun(\node_1)=\labelfun(\node_2)$ and both $\node_1$ and $\node_2$ are preterminal nodes, i.e. parent of a leaf node, then $C_{SST}(\node_1,\node_2)=\lambda$; \textit{iii}) if $\labelfun(\node_1)=\labelfun(\node_2)$ and either $\node_1$ or $\node_2$ is not a  preterminal node, then 
% The only difference with respect to the definition of  $C_{PT}()$ is in case \textit{iii}): 
 \begin{equation}
 C_{SST}(\node_1,\node_2) = \lambda\displaystyle \prod_{j=1}^{\rho(\node_1)} \Big(\sigma + C_{SST}(ch_{\node_1}[j],ch_{\node_2}[j])\Big), 
\label{eq:csst}
 \end{equation}
where $\sigma$ determines the type of kernel (SST is obtained with $\sigma=1$). The complexity of SST is $O(|T|^2)$. 
The ST kernel counts the number of matching proper subtrees between the input trees $T_1$ and $T_2$ \cite{Vishwanathan2003}. The weight of a match of a feature $f$, i.e. a proper subtree rooted at a node $\node$, is $C(\node, \node)=\lambda^{|f|}$, where $|f|$ is the number of nodes of $f$. Although the ST kernel can be obtained from eq.~\eqref{eq:csst} by setting $\sigma=0$ \cite{Collins2002}, a $O(|T|\log |T|)$ algorithm has been presented in \cite{Vishwanathan2003}. 
\nuovo{The Partial Tree (PT) kernel \cite{Moschitti2006a} counts the number of matching subtrees. Its worst-case complexity is $O(\rho^3 |T|^2)$, where $\rho$ is the maximum out-degree of the two trees}{nostra scelta ridurre la descrizione di PT}. 
The Elastic Tree kernel extends PT by allowing matches between nodes with different labels and allowing matchings between substructures built by
combining subtrees with their descendants (the difference with respect to PT is that a subtree feature can be built from a subset of non connected nodes of the original tree) \cite{Kashima2002}. 
Altough its worst case complexity is $O(|T|^2)$, the evaluation of the kernel practically introduces a significant overhead with respect to SST and PT. 
More kernels which extend the feature space of PT are described in \cite{Bloehdorn2007, Shin2010, Zhang2007}.}

\textcolor{red}{All the kernels described in this section share two characteristics: 
\begin{itemize}
 \item in order to compute any of the $C(\node_1, \node_2)$ functions described in this section, it is only required to access the children of a node. As a consequence, the corresponding tree kernels can, in principle, be applied to DAGs with no modification; 
 \item the kernels described in this section require the children of a node to be ordered. Since the DAGs resulting from the decomposition described in Section~\ref{sec:odd} do not meet this requirement, in the next section we show how to define a canonical ordering for DAG nodes. 
\end{itemize}
}

